Network-level Safety Metrics for Overall Traffic Safety Assessment: A Case Study

Driving safety analysis has recently experienced unprecedented improvements thanks to technological advances in precise positioning sensors, artificial intelligence (AI)-based safety features, autonomous driving systems, connected vehicles, high-throughput computing, and edge computing servers. Particularly, deep learning (DL) methods empowered volume video processing to extract safety-related features from massive videos captured by roadside units (RSU). Safety metrics are commonly used measures to investigate crashes and near-conflict events. However, these metrics provide limited insight into the overall network-level traffic management. On the other hand, some safety assessment efforts are devoted to processing crash reports and identifying spatial and temporal patterns of crashes that correlate with road geometry, traffic volume, and weather conditions. This approach relies merely on crash reports and ignores the rich information of traffic videos that can help identify the role of safety violations in crashes. To bridge these two perspectives, we define a new set of network-level safety metrics (NSM) to assess the overall safety profile of traffic flow by processing imagery taken by RSU cameras. Our analysis suggests that NSMs show significant statistical associations with crash rates. This approach is different than simply generalizing the results of individual crash analyses, since all vehicles contribute to calculating NSMs, not only the ones involved in crash incidents. This perspective considers the traffic flow as a complex dynamic system where actions of some nodes can propagate through the network and influence the crash risk for other nodes. We also provide a comprehensive review of surrogate safety metrics (SSM) in the Appendix A.

==> Adot_DATASET.tex <==
\section{ADOT Dataset}
\subsection{Trajectory Data}
The Arizona Department of Transportation (ADOT) collected total xx videos from xx cameras crossing I-1O from $3^rd$ Street to SR-51. Each camera record 10 hours video varying from 9 am to 6 pm. Fig.R\ref{} show the xx scenes of the video data with the regions of interest (RoIs). The RoIs are adopted to gurantee the accuracy and simplixty for the processing. 

We employ YOLOv5+DeepSort to extract the trajectories. YOLOv5 is ......... DeepSort is based on.  algorithm, and requires a well-performed detector. The center of the 

Then we translate the trajectories from the camera perspective to the top-view perspective by .....

The data specification is shown on Table.\ref{}.

% Video Processing

%% Filtering
\subsection{Crash Data}
Crash data is .....

ADOT also provides the corresponding crash data collected from 2015-2019. The data provides xx, xx, xx, ....
Fig.\ref{} shown the heatmap of the incidents in the recorded data.



The data specification is shown on Table.\ref{}

\section{Experiment}

==> TableDataset-2.tex <==

\begin{comment}


%wang2011automatic,morris2011trajectory,hospedales2012video,
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline\rowcolor{gray}
\textbf{Category} &
  \textbf{Dataset} &
  \textbf{Size} &
  \textbf{Features} \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Trajectory\\ analysis\end{tabular}} &
  MIT traffic dataset(2011)\cite{wang2011automatic} &
  \begin{tabular}[c]{@{}l@{}}around 162, 000 frames\\ from a 90 minutes long video sequence (30 fps)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Both pedestrian and vehicle movements;\\ with occlusions and varying illumination conditions\end{tabular} \\ \cline{2-4} 
 &
  MIT trajectory dataset(2008)\cite{grimson2008trajectory} &
  577 radar tracks, 45 453 video tracks &
  Multiple single camera view \\ \cline{2-4} 
 &
  CVRR trajectory analysis datasets (2011) \cite{morris2011trajectory}  &
  \begin{tabular}[c]{@{}l@{}}4 scenes: a simulated intersection (19 activities),\\ a real highway (8 activities)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Units are pixels;\\ only contain spatial information\end{tabular} \\ \cline{2-4} 
 &
  i-Lids–advanced vehicle detection challenge\cite{ilidsadvanced_2007} &
  35000 images. 7 sequences with 25 fps. &
  \begin{tabular}[c]{@{}l@{}}Consider daytime;\\ various locations in the UK\end{tabular} \\ \cline{2-4} 
 &
  NGSIM(2007)\cite{NGSIM}  &
  45 mins+45 mins+ 30 mins&
  \begin{tabular}[c]{@{}l@{}}Three sub-datasets;\\ US-101 and I-80 for freeway scenario;\\ Lankershim Boulevard Dataset for arterial corridors scenario;\\ each dataset is segmented with different congestion conditions \end{tabular} \\ \cline{2-4} 
 
  &
  QMUL junction dataset(2012) \cite{hospedales2012video} &
  1 hour video &
  Busy traffic at a junction \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Auto-driving\\ tasks\end{tabular}} &
  CamVid(2009) \cite{brostow2009semantic} &
  700 images, 32 classes, 10 min HD video with 30fps &
  \begin{tabular}[c]{@{}l@{}}Support pixel-wise segmentation tasks;\\ provide 3D camera pose\end{tabular} \\ \cline{2-4} 
 &
  Cityscapes (2016)\cite{cordts2016cityscapes} &
  \begin{tabular}[c]{@{}l@{}}5000 pixel-level annotated images\\  and 20000 coarse annotated images (weak-label)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}complex urban street scenes;\\  record from 50 cities;\end{tabular} \\ \cline{2-4} 
 &
  Mapillary Vistas Dataset(2017)\cite{neuhold2017mapillary} &
  \begin{tabular}[c]{@{}l@{}}25 000 high-resolution images; \\ 66 classes for objection\\ 37 instance-specific labels\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Various conditions regarding weather, \\ season and daytime\end{tabular} \\ \cline{2-4} 
 &
  SYNTHIA(2016) \cite{ros2016synthia} &
  \begin{tabular}[c]{@{}l@{}}13,400 frames of the city (real);\\ \\ four video sequences of  ~50,000 frames (simulated);\\ 13 classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Scene diversity;\\ multiple seasons;\\ lighting conditions and weather\end{tabular} \\ \cline{2-4} 
 &
  KITTI Vision Benchmark Suite (2012)\cite{Geiger2012CVPR}&
  7481 training images and 7518 test images; &
  \begin{tabular}[c]{@{}l@{}}Up to 15 cars and 30 pedestrians per image;\\ tasks of interest are stereo, optical flow, \\ visual odometry, 3D object detection, and 3D tracking\end{tabular} \\ \cline{2-4} 
 &
  Berkeley Deep Drive (2018)\cite{yu2018bdd100k}  &
  over 100K videos &
  \begin{tabular}[c]{@{}l@{}}Diversity of annotations;\\ diversity of geography, environment, and weather\end{tabular} \\ \cline{2-4} 
 &
  IDD (2019) \cite{varma2019idd}&
  10,004 images; 34 classes; 182 drive sequences &
  \begin{tabular}[c]{@{}l@{}}Unstructured environments;\\ four-level label hierarchy; possibility for new tasks: \\ domain adaptation, \\ few-shot learning and behavior prediction\end{tabular} \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Traffic sign\\ detection\end{tabular}} &
  TLR (2009)\cite{de2009real} &
  \begin{tabular}[c]{@{}l@{}}11 179 frames (8min 49sec, @25FPS);\\ 9 168 instances of traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Hand-labeled;\\ tasks for traffic light detection and traffic sign detection\end{tabular} \\ \cline{2-4} 
 &
  LISA (2012)\cite{mogelmose2012vision}&
  \begin{tabular}[c]{@{}l@{}}6600 frames with ~7800 annotated objects;\\ 49 classes of signs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Recorded in the US;\\ Images from various camera types\end{tabular} \\ \cline{2-4} 
 &
  GTSDB(2013)\cite{houben2013detection} &
  \begin{tabular}[c]{@{}l@{}}900 images \\ divided into 600 training images (846 traffic signs) \\ and 300 evaluation images (360 traffic signs)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Signs are divided into prohibitory, danger, mandatory, \\ and other signs\end{tabular} \\ \cline{2-4} 
 &
  BelgianTS(2014)\cite{timofte2014multi} &
  \begin{tabular}[c]{@{}l@{}}13,444 traffic sign annotations in 9,006 still images \\ corresponding to 4,565\\ physically distinct traffic signs.\end{tabular} &
  Available for 2D and 3D testing \\ \cline{2-4} 
 &
  TT100K (2016)\cite{zhu2016traffic}&
  \begin{tabular}[c]{@{}l@{}}100000 images containing 30000 traffic-sign instances;\\  128 sign classes\end{tabular} &
  Diversity of annotation \\ \cline{2-4} 
 &
  BSTL (2017)\cite{behrendt2017deep}&
  \begin{tabular}[c]{@{}l@{}}13427 images (5093training+8334test~15fps);\\ 24000 annotated traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Cover a decent variety of road scenes and\\  typical difficulties\end{tabular} \\ \hline
\multirow{Plate detection} &
  ReId (2017)\cite{ReId} &
  9.5hours from 8 locations &
  \begin{tabular}[c]{@{}l@{}}Varied daytime;\\ multi-plates on a frame;\\ cameras placed on bridges above highways;\\ relatively small objects\end{tabular} \\ \cline{2-4} 
 &
  UCSD car dataset(2007) \cite{UCSDCARS} &
  \begin{tabular}[c]{@{}l@{}}10 hours video;\\ 878 cars tracked from the moment;\\ 291 still cars recorded in parking lot\end{tabular} &
  Label with make, model, license plate location, plate texts \\ \cline{2-4} 
 &
  UFPR-ALPR Dataset(2018)\cite{laroca2018robust_UFPR} &
  \begin{tabular}[c]{@{}l@{}}4,500 fully annotated images from 150 vehicles;\\ 30 fps\\ >30,000 license characters;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Different license color;\\ both vehicle and camera are moving\end{tabular} \\ \cline{2-4} 
 &
  SSIG Dataset(2016)\cite{gonccalves2016benchmark_SSIG} &
  \begin{tabular}[c]{@{}l@{}}2000 Brazilian license plates; \\ 14,000 alphanumeric symbols\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Static camera view;\\ character are segmented\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Some popular traffic-related datasets.}
\label{tab:trafficdataset}
\end{table*}








\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline\rowcolor{gray}
\textbf{Category} &
  \textbf{Dataset} &
  \textbf{Size} &
  \textbf{Features} \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Naturalistic\\ Study\end{tabular}} &
  The 100-Car Naturalistic Driving Study(2006)\cite{dingus2006100} &
  \begin{tabular}[c]{@{}l@{}}~2,000,000 vehicle miles;\\ ~43,000 hours of data\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Contains extreme cases of driving behavior;\\ Event-based database\end{tabular} \\ \cline{2-4} 
 &
  SHRP 2 NDS dataset(2012)\cite{the_shrp_2_2012}  &
  more than 2 PB of continuous naturalistic driving data &
  \begin{tabular}[c]{@{}l@{}}Multi-view video outputs;\\ collected during a 3-y period from \\ more than 3,500 participants, aged 16–98\end{tabular} \\ \hline

\multirow{UAV} &
  MOR-UAV(2020)\cite{MOR-UAV} &
  \begin{tabular}[c]{@{}l@{}}89,783 moving object instances;\\  10,948 various scenarios;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Tasks for moving and non-moving objects;\\ varied conditions of the environment;\\ labeled by aixs-aligned bounding boxes\end{tabular} \\ \cline{2-4} 
 &
  Stanford Drone Dataset(2016)\cite{robicquet2016learning} &
  \begin{tabular}[c]{@{}l@{}}>100 top-view scenes;\\ 20,000 targets\\ annotated trajectories and id\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Real-world scenario-based;\\ varied types of targets\end{tabular} \\ \cline{2-4} 
 &
  The highD dataset(2018)\cite{krajewski2018highd} &
  \begin{tabular}[c]{@{}l@{}}16.5hous of measurements for 110,000 vehicles from 6\\ locations.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Real-world scenario-based;\\ focus on highways\\ contain naturalistic behavior of road users\end{tabular} \\ \cline{2-4} 
 &
  The inD dataset(2019)\cite{bock2019ind} &
  \begin{tabular}[c]{@{}l@{}}contains more than 11500 road users;\\ 10 hours measurement\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Successor of highD,\\ focus on intersections\end{tabular} \\ \hline
  \multirow{}{}{\begin{tabular}[c]{@{}l@{}}Video-based \\ Traffic events\\ (Crash)\end{tabular}} &
  UCF-Crimes(2018) \cite{sultani2018real} &
  1900 sequences, 128hours &
  \begin{tabular}[c]{@{}l@{}}Includes realistic anomalies such as fighting, road crash;\\ No spatial annotation\end{tabular} \\ \cline{2-4} 
 &
  DAD(2016) \cite{chan2016anticipating} &
  1730 sequences, 2.4 hours &
  \begin{tabular}[c]{@{}l@{}}Spatio-temporal annotation\\ Video captured by dashcam\end{tabular} \\ \cline{2-4} 
 &
  CADP(2018)\cite{shah2018cadp} &
  1416 sequences, 5.2 hours &
  \begin{tabular}[c]{@{}l@{}}Include multi-crash sequences\\ Captured by CCTV; Include varied environment\end{tabular} \\
  \cline{2-4}
  &
  NVIDIA AI CITY challenge\cite{ai_city_challenge} &
  \begin{tabular}[c]{@{}l@{}}Track 1: 31 videos (about 9 hours in total)\\ Track 2: 56,277 images,\\ 36,935 come from 333 object identities\\ Track 3: 215.03 minutes videos \\ 300K bounding boxes\\ Track 4: 200 15mins videos 30fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Track 1: vehicle counting\\ Track 2: vehicle Re-id\\ Track 3: vehicle tracking\\ Track 4: Abnormal detection\\ Anomalies can be due to \\ car crashes or stalled vehicles\end{tabular} \\ \hline
  
\multirow{\begin{tabular}[c]{@{}l@{}}Fine-grained\\ Vehicle\\ Classification\end{tabular}} &
  Standford Cars\cite{krause20133d} &
  16,185 images of 196 classes of cars &
  \begin{tabular}[c]{@{}l@{}}The cars images are taken from many angles;\\ classes typically based on Make, Model, Year\end{tabular} \\ \cline{2-4} 
 &
  COMPCARS\cite{yang2015large} &
  \begin{tabular}[c]{@{}l@{}}Web-nature: 136,726 (entire car)+27,618 (car parts),\\ 163 car makes with 1,716 car models;\\ Surveillance-nature: 5000 car images\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Web-nature data are labeled with \\ bounding boxes and viewpoints;\\ the surveillance-nature images are in the \\ front view\end{tabular} \\ \hline

\end{tabular}%
}
\caption{Some popular traffic-related datasets [Continue].}
\label{tab:trafficdataset-continue}
\end{table*}
\end{comment}





%wang2011automatic,morris2011trajectory,hospedales2012video,
\begin{table*}[!h]
\centering\caption{Some popular traffic-related datasets.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
%\hline\rowcolor{gray}
\toprule
\textbf{Category} &
  \textbf{Dataset} &
  \textbf{Size} &
  \textbf{Features} \\ \midrule

\multirow{\begin{tabular}[c]{@{}l@{}}Trajectory\\ analysis\end{tabular}} &
  MIT traffic dataset(2011)\cite{wang2011automatic} &
  \begin{tabular}[c]{@{}l@{}}around 162, 000 frames\\ from a 90 minutes long video sequence (30 fps)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Both pedestrian and vehicle movements;\\ with occlusions and varying illumination conditions\end{tabular} \\ \cmidrule{2-4} 
 &
  MIT trajectory dataset(2008)\cite{grimson2008trajectory} &
  577 radar tracks, 45 453 video tracks &
  Multiple single camera view \\ \cmidrule{2-4} 
 &
  CVRR trajectory analysis datasets (2011) \cite{morris2011trajectory}  &
  \begin{tabular}[c]{@{}l@{}}4 scenes: a simulated intersection (19 activities),\\ a real highway (8 activities)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Units are pixels;\\ only contain spatial information\end{tabular} \\ \cmidrule{2-4} 
 &
  i-Lids–advanced vehicle detection challenge\cite{ilidsadvanced_2007} &
  35000 images. 7 sequences with 25 fps. &
  \begin{tabular}[c]{@{}l@{}}Consider daytime;\\ various locations in the UK\end{tabular} \\ \cmidrule{2-4} 
 &
  NGSIM(2007)\cite{NGSIM}  &
  45 mins+45 mins+ 30 mins&
  \begin{tabular}[c]{@{}l@{}}Three sub-datasets;\\ US-101 and I-80 for freeway scenario;\\ Lankershim Boulevard Dataset for arterial corridors scenario;\\ each dataset is segmented with different congestion conditions \end{tabular} \\ \cmidrule{2-4} 
 
  &
  QMUL junction dataset(2012) \cite{hospedales2012video} &
  1 hour video &
  Busy traffic at a junction \\ \midrule
\multirow{\begin{tabular}[c]{@{}l@{}}Auto-driving\\ tasks\end{tabular}} &
  CamVid(2009) \cite{brostow2009semantic} &
  700 images, 32 classes, 10 min HD video with 30fps &
  \begin{tabular}[c]{@{}l@{}}Support pixel-wise segmentation tasks;\\ provide 3D camera pose\end{tabular} \\ \cmidrule{2-4} 
 &
  Cityscapes (2016)\cite{cordts2016cityscapes} &
  \begin{tabular}[c]{@{}l@{}}5000 pixel-level annotated images\\  and 20000 coarse annotated images (weak-label)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}complex urban street scenes;\\  record from 50 cities;\end{tabular} \\ \cmidrule{2-4} 
 &
  Mapillary Vistas Dataset(2017)\cite{neuhold2017mapillary} &
  \begin{tabular}[c]{@{}l@{}}25 000 high-resolution images; \\ 66 classes for objection\\ 37 instance-specific labels\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Various conditions regarding weather, \\ season and daytime\end{tabular} \\ \cmidrule{2-4} 
 &
  SYNTHIA(2016) \cite{ros2016synthia} &
  \begin{tabular}[c]{@{}l@{}}13,400 frames of the city (real);\\ \\ four video sequences of  ~50,000 frames (simulated);\\ 13 classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Scene diversity;\\ multiple seasons;\\ lighting conditions and weather\end{tabular} \\ \cmidrule{2-4} 
 &
  KITTI Vision Benchmark Suite (2012)\cite{Geiger2012CVPR}&
  7481 training images and 7518 test images; &
  \begin{tabular}[c]{@{}l@{}}Up to 15 cars and 30 pedestrians per image;\\ tasks of interest are stereo, optical flow, \\ visual odometry, 3D object detection, and 3D tracking\end{tabular} \\ \cmidrule{2-4} 
 &
  Berkeley Deep Drive (2018)\cite{yu2018bdd100k}  &
  over 100K videos &
  \begin{tabular}[c]{@{}l@{}}Diversity of annotations;\\ diversity of geography, environment, and weather\end{tabular} \\ \cmidrule{2-4} 
 &
  IDD (2019) \cite{varma2019idd}&
  10,004 images; 34 classes; 182 drive sequences &
  \begin{tabular}[c]{@{}l@{}}Unstructured environments;\\ four-level label hierarchy; possibility for new tasks: \\ domain adaptation, \\ few-shot learning and behavior prediction\end{tabular} \\ \midrule
\multirow{\begin{tabular}[c]{@{}l@{}}Traffic sign\\ detection\end{tabular}} &
  TLR (2009)\cite{de2009real} &
  \begin{tabular}[c]{@{}l@{}}11 179 frames (8min 49sec, @25FPS);\\ 9 168 instances of traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Hand-labeled;\\ tasks for traffic light detection and traffic sign detection\end{tabular} \\ \cmidrule{2-4} 
 &
  LISA (2012)\cite{mogelmose2012vision}&
  \begin{tabular}[c]{@{}l@{}}6600 frames with ~7800 annotated objects;\\ 49 classes of signs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Recorded in the US;\\ Images from various camera types\end{tabular} \\ \cmidrule{2-4} 
 &
  GTSDB(2013)\cite{houben2013detection} &
  \begin{tabular}[c]{@{}l@{}}900 images \\ divided into 600 training images (846 traffic signs) \\ and 300 evaluation images (360 traffic signs)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Signs are divided into prohibitory, danger, mandatory, \\ and other signs\end{tabular} \\ \cmidrule{2-4} 
 &
  BelgianTS(2014)\cite{timofte2014multi} &
  \begin{tabular}[c]{@{}l@{}}13,444 traffic sign annotations in 9,006 still images \\ corresponding to 4,565\\ physically distinct traffic signs.\end{tabular} &
  Available for 2D and 3D testing \\ \cmidrule{2-4} 
 &
  TT100K (2016)\cite{zhu2016traffic}&
  \begin{tabular}[c]{@{}l@{}}100000 images containing 30000 traffic-sign instances;\\  128 sign classes\end{tabular} &
  Diversity of annotation \\ \cmidrule{2-4} 
 &
  BSTL (2017)\cite{behrendt2017deep}&
  \begin{tabular}[c]{@{}l@{}}13427 images (5093training+8334test~15fps);\\ 24000 annotated traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Cover a decent variety of road scenes and\\  typical difficulties\end{tabular} \\ \midrule
\multirow{Plate detection} &
  ReId (2017)\cite{ReId} &
  9.5hours from 8 locations &
  \begin{tabular}[c]{@{}l@{}}Varied daytime;\\ multi-plates on a frame;\\ cameras placed on bridges above highways;\\ relatively small objects\end{tabular} \\ \cmidrule{2-4} 
 &
  UCSD car dataset(2007) \cite{UCSDCARS} &
  \begin{tabular}[c]{@{}l@{}}10 hours video;\\ 878 cars tracked from the moment;\\ 291 still cars recorded in parking lot\end{tabular} &
  Label with make, model, license plate location, plate texts \\ \cmidrule{2-4} 
 &
  UFPR-ALPR Dataset(2018)\cite{laroca2018robust_UFPR} &
  \begin{tabular}[c]{@{}l@{}}4,500 fully annotated images from 150 vehicles;\\ 30 fps\\ >30,000 license characters;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Different license color;\\ both vehicle and camera are moving\end{tabular} \\ \cmidrule{2-4} 
 &
  SSIG Dataset(2016)\cite{gonccalves2016benchmark_SSIG} &
  \begin{tabular}[c]{@{}l@{}}2000 Brazilian license plates; \\ 14,000 alphanumeric symbols\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Static camera view;\\ character are segmented\end{tabular} \\  \bottomrule
\end{tabular}%
}

\label{tab:trafficdataset}
\end{table*}








\begin{table*}[h]
\centering\caption{Some popular traffic-related datasets [Continue].}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\textbf{Category} &
  \textbf{Dataset} &
  \textbf{Size} &
  \textbf{Features} \\ \midrule
\multirow{\begin{tabular}[c]{@{}l@{}}Naturalistic\\ Study\end{tabular}} &
  The 100-Car Naturalistic Driving Study(2006)\cite{dingus2006100} &
  \begin{tabular}[c]{@{}l@{}}~2,000,000 vehicle miles;\\ ~43,000 hours of data\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Contains extreme cases of driving behavior;\\ Event-based database\end{tabular} \\ \cmidrule{2-4} 
 &
  SHRP 2 NDS dataset(2012)\cite{the_shrp_2_2012}  &
  more than 2 PB of continuous naturalistic driving data &
  \begin{tabular}[c]{@{}l@{}}Multi-view video outputs;\\ collected during a 3-y period from \\ more than 3,500 participants, aged 16–98\end{tabular} \\ \midrule

\multirow{UAV} &
  MOR-UAV(2020)\cite{MOR-UAV} &
  \begin{tabular}[c]{@{}l@{}}89,783 moving object instances;\\  10,948 various scenarios;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Tasks for moving and non-moving objects;\\ varied conditions of the environment;\\ labeled by aixs-aligned bounding boxes\end{tabular} \\ \cmidrule{2-4} 
 &
  Stanford Drone Dataset(2016)\cite{robicquet2016learning} &
  \begin{tabular}[c]{@{}l@{}}>100 top-view scenes;\\ 20,000 targets\\ annotated trajectories and id\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Real-world scenario-based;\\ varied types of targets\end{tabular} \\ \cmidrule{2-4} 
 &
  The highD dataset(2018)\cite{krajewski2018highd} &
  \begin{tabular}[c]{@{}l@{}}16.5hous of measurements for 110,000 vehicles from 6\\ locations.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Real-world scenario-based;\\ focus on highways\\ contain naturalistic behavior of road users\end{tabular} \\ \cmidrule{2-4} 
 &
  The inD dataset(2019)\cite{bock2019ind} &
  \begin{tabular}[c]{@{}l@{}}contains more than 11500 road users;\\ 10 hours measurement\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Successor of highD,\\ focus on intersections\end{tabular} \\ \midrule
  \multirow{\begin{tabular}[c]{@{}l@{}}Video-based \\ Traffic events\\ (Crash)\end{tabular}} &
  UCF-Crimes(2018) \cite{sultani2018real} &
  1900 sequences, 128hours &
  \begin{tabular}[c]{@{}l@{}}Includes realistic anomalies such as fighting, road crash;\\ No spatial annotation\end{tabular} \\ \cmidrule{2-4} 
 &
  DAD(2016) \cite{chan2016anticipating} &
  1730 sequences, 2.4 hours &
  \begin{tabular}[c]{@{}l@{}}Spatio-temporal annotation\\ Video captured by dashcam\end{tabular} \\ \cmidrule{2-4} 
 &
  CADP(2018)\cite{shah2018cadp} &
  1416 sequences, 5.2 hours &
  \begin{tabular}[c]{@{}l@{}}Include multi-crash sequences\\ Captured by CCTV; Include varied environment\end{tabular} \\
  \cmidrule{2-4}
  &
  NVIDIA AI CITY challenge\cite{ai_city_challenge} &
  \begin{tabular}[c]{@{}l@{}}Track 1: 31 videos (about 9 hours in total)\\ Track 2: 56,277 images,\\ 36,935 come from 333 object identities\\ Track 3: 215.03 minutes videos \\ 300K bounding boxes\\ Track 4: 200 15mins videos 30fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Track 1: vehicle counting\\ Track 2: vehicle Re-id\\ Track 3: vehicle tracking\\ Track 4: Abnormal detection\\ Anomalies can be due to \\ car crashes or stalled vehicles\end{tabular} \\ \midrule
  
\multirow{\begin{tabular}[c]{@{}l@{}}Fine-grained\\ Vehicle\\ Classification\end{tabular}} &
  Standford Cars\cite{krause20133d} &
  16,185 images of 196 classes of cars &
  \begin{tabular}[c]{@{}l@{}}The cars images are taken from many angles;\\ classes typically based on Make, Model, Year\end{tabular} \\ \cmidrule{2-4} 
 &
  COMPCARS\cite{yang2015large} &
  \begin{tabular}[c]{@{}l@{}}Web-nature: 136,726 (entire car)+27,618 (car parts),\\ 163 car makes with 1,716 car models;\\ Surveillance-nature: 5000 car images\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Web-nature data are labeled with \\ bounding boxes and viewpoints;\\ the surveillance-nature images are in the \\ front view\end{tabular} \\  \bottomrule

\end{tabular}%
}

\label{tab:trafficdataset-continue}
\end{table*}




==> draft.tex <==
vehicle detection:
pure CNN: 
\cite{sang2018improved}:YOLOv2,vehicle detection
\cite{espinosa2017vehicle} Faster R-cnn,vehicle detection
\cite{wang2019comparative} Faster R-cnn,R-FCN,SSD,YOLOv3,RetinaNet
\cite{kim2019multi} YOLOv3, vehicle detection
\cite{wang2017evolving} Faster RCNN, vehicle detection
\cite{soin2017moving} RCNN, vehicle detection
\cite{zhang2019vehicle} SSD, vehicle detection
\cite{zhang2017application} Faster R-cnn, vehicle detection, traffic monitoring
\cite{peppa2018urban} Faster RCNN
ssd: chen2020inception cao2020front
plate detection:
pure CNN:\cite{kim2017deep}\cite{selmi2017deep}\cite{masood2017license}
\cite{hsu2017robust} YOLO/YOLOv2
\cite{kessentini2019two} YOLOv2
\cite{lee2016real} Faster RCNN
\cite{khazaee2020real} YOLOv3
\cite{xie2018new} YOLO
\cite{chen2019automatic} YOLO
ssd
ren2020implementation,hu2020mobilenet,danilenko2020license

traffic sign:
pure CNN: \cite{zhu2016traffic,wu2013traffic,shustanov2017cnn}
\cite{qian2016road} Fast R-cnn
\cite{shao2019improved} Faster RCNN
\cite{zhang2020cascaded} r-cnn
\cite{zuo2017traffic} Faster rcnn
\cite{zhang2017real} YOLOv2 \cite{Tai_2020} v3
\cite{wu2019traffic} Faster rcnn
\cite{peng2016traffic} Faster rcnn

gao2019traffic ssd
you2020traffic SSD


zhang2019vehicle e UA-DETRAC s 77.94 mAP  UA-DETRAC
,chen2020inception 86.2 KITTI 87.4 UA-DETRAC
,cao2020front 92.18 kitti

6778050,  99.7\%
8019461:repeated 

espinosa2017vehicle: 0.7 author dataset
,wang2019comparative
,wang2017evolving,  84.43     DETRAC dataset others
soin2017moving, 100 author dataset
zhang2017application, 96.5 uav 
,peppa2018urban, 97 R-CNN 98.2 SSD  author dataset

lee2016real: 99.94

 \cite{hsu2017robust,kessentini2019two,khazaee2020real,xie2018new,chen2019automatic}
hsu2017robust:
kessentini2019two: a full LP recognition rate of 97.67\% in the GAP-LP dataset, and of 91.46\% in Radar dataset
khazaee2020real:0.979 0.972 on dateset gnerated by the authors 
xie2018new: 98.32 UCSD PKU
chen2019automatic:98.22 AOLP



ren2020implementation,hu2020mobilenet,danilenko2020license
ren2020implementation： 0.92
hu2020mobilenet 90.12 
danilenko2020license 94+ 


kim2017deep, 98.39\% and a recall of 96.83\% on Caltech
selmi2017deep 94.8 Caltech
,masood2017license 99.09\%  US 99.64\% EU

qian2016road  85.58\%.
,shao2019improved 69.56\% gtsdb+ctsd
,zhang2020cascaded The accuracy and recall rate of our method are 98.7\% and 90.5\% in GTSDB, 99.7\% and 83.62\% in CCTSDB and 98.9\% and 85.6\% in Lisa dataset respectively.
,zuo2017traffic 0.3449 traffic sign detection competition in 2016 by CCF
and UISEE company.
,wu2019traffic mAP  91.75\%  GTSDB
,peng2016traffic mAP ~90 GTSDB

zhang2017real 96.69 @0.017   CCTSDB and GTSDB
,Tai_2020  99.1 mAP  


gao2019traffic, The precision and recall on the test data set are 91.0\%, and 88.06\%  GTSDB
you2020traffic 0.75 0.82recall  TT100K traffic sign datase

zhu2016traffic  a recall 0.91 and accuracy 0.88 TT100K
,wu2013traffic,  AUC of 99.73\% in the category “danger”, and an AUC of 97.62\% in the category “mandatory  GTSDB
shustanov2017cnn 99.94 GTSRB


\subsection{Speed Estimation}
Speed Estimation aims to estimate the movement speed of an object by exploiting the interaction between the object and the environment in a video clip. The speed of the vehicle is one of most significant factor of driving safety. If the video is in the perspective of external observers, the speed of vehicles can be estimated based on visual tracker by:
\begin{align}
    V_t = \sqrt{\delta x^2_t+\delta y^2_t}
\end{align}
where,$x_t$ and $y_t$ are the instantaneous displacement of two dimensions. Consider the minimum time interval (depends on the video source quality and algorithm speed) is existed between two tracking, $\delta x_t$ and $\delta y_t$ can be written as:
\begin{align}
    \delta x_t& = x_t-x_{t-\delta t}\\
    \delta y_t& = y_t-y_{t-\delta t}\\
\end{align}
where, $\delta t$ is the minimum measurable time interval of a tracker.
If want to estimate the speed based on the drivers' view, the question would be relatively difficult. The solutions involve employ Binocular camera to collect data and deploy SLAM technique.



Accuracy  $\frac{Correct predictions}{Total predictions}$
Recall  $\frac{True Positive}{True Positive+False Negative}$
Precision $\frac{True positive}{True positive+False Positive}$
F1 score $2\times\frac{Precision\times Recall}{Precision+ Recall}$
**(Area Under ROC Curve) $AUC=\frac{\sum_{i\in Positive}rank_i-\frac{M(1+M)}{2}}{MN}$
sort the score (low to high) The rank of highest score is $n$
Pixel Accuracy (PA) $\frac{TP+TN}{TP+TN+FP+FN}$


Disparity accuracy 
stixel-wise percentage accuracy .similar to PA

Normalized error (mean)\cite{huang2018measuring} $normalized error=\frac{|d-d_{gt}|}{d_{gt}}$.  $d$ is the calculated distance and $d_{gt}$ is the ground truth of distance.


Average Precision (AP)  $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class)
mean Average Precision (mAP) $mean(AP_i)$
Intersection over Union (IoU) $\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$
$B_{gt}$: ground truth bounding box
$B_{p}$: predicted bounding box






2~\cite{xu2015learning}, unsupervised representation learning, trained SVM
119~\cite{medel2016anomaly}, self-supervised 
%216
205~\cite{xu2017detecting}, unsupervised representation learning
108~\cite{liu2018future}, supervised adversarial learning 

Accident detection: %211 \cite{} : 

gan-based: nguyen2020anomaly  F1 score 0.9412   AI City Challenge 2019 semi-supervised

yao2019unsupervised  60.1 AUC  A3D Dataset 

tian2019automatic 90.02 average precision (AP) CAD-CVIS
%rajesh2020deep successfully 
kim2020pre 0.82 3D conv GTA 

ijjina2019computer Detection Ratio 71 superivsed Youtube+GTA
 shah2018cadp    47.25 CADP
  srinivasan2020novel   78.2 CADP\cite{shah2018cadp}
suzuki2018anticipating 99.1 mean average precision (mAP)


52~\cite{giannakeris2018speed}, unsupervised clustering  NVDIA CITY. nF1-score of 0.33 and our detection time RMSE was 227 (also for spped evaluate)

arceda2018fast 89 

biradar2019challenges achieved 0.3838 F1-score and 93.61 RMSE respectively  Track 3  NVIDIA AI city challenge

xu2018dual  0.8649 3.6152 Track 2 NVIDIA AI CITY CHALLENGE
doshi2020fast 0.5926 8.2386   Track 4 NVIDIA AI CITY CHALLENGE UNSPER

car behaviour 

220~\cite{zhou2016spatial}, supervise 95.2 U-turn dataset\cite{benezeth2009abnormal}
franklin2020traffic  100 and 95.34 input video 1 video 2

traffic incident




%pedestrians 
%34
%2~\cite{xu2015learning}, unsupervised representation learning, trained SVM
%119~\cite{medel2016anomaly}, self-supervised 
%216
%205~\cite{xu2017detecting}, unsupervised representation learning
%108~\cite{liu2018future}, supervised adversarial learning 

12/11 9:33pm
metrif
IDF1



-multiple object tracking accuracy MOTA, $MOTA=1-\frac{FN+FP+\Phi}{T}$,$\Phi$ denotes the number of fragmentations 

-Identification F1-Score $IDF1=\frac{2IDTP}{2IDTP+IDFP+IDFN}$

Multi-camera Tracking Accuracy
$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$
$M^w$: within-camera identity mismatches 
$T^w$:  true within-camera detections
$M^h$:  handover mismatches
$T^h$:  true handover detections

dinh2017development: Kalman filter, GMM
ngel2016low: the Approximated Median Filter
 liu2011multi:a Multi-Modal Particle Filter(MMPF)
jazayeri2011vehicle HMM
xia2013automatic   CAMShift
kaur2016vehicle kalman flter
o2010rear kalman flter
   graph-based

teoh2012reliability Kalman-filter

khalkhali2020vehicle Kalman-filter

luvizon2016video  SIFT+KLT speed

mei2011robust sparse representation

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works               & Performance                  & Methods                                 \\ \hline
qiu2018kestrel      & 75.9 Recall 88.6 Accuracy    & YOLO+KLT                                \\ \hline
lopez2019boosting &
  \begin{tabular}[c]{@{}l@{}}0.305AP subset:M-30 0.662AP subset:M-30-HD \\ 0.381AP subset:Urban1 of  GRAM-RTM\end{tabular} &
  Faster R-CNN \\ \hline
xu2017car           & 98.43                        & Faster R-CNN                            \\ \hline
scheidegger2018mono & 80.04 MOTA on KITTI          & CNN+PMBM filter\cite{garcia2018poisson} \\ \hline
zou2019multi &
  \begin{tabular}[c]{@{}l@{}}75.29MOTA campus \\ 76.06MOTAurban \\ 78.14MOTA highway \\ on KITTI\end{tabular} &
  Siamese network+SPP+MDP \\ \hline
li2019spatio        & 83.2IDF1 nivida AI city      & FPN+tracking loss                       \\ \hline
nikodem2020multi &
  \begin{tabular}[c]{@{}l@{}}single-camera tracking accuracy 97+\\ multi-camera tracking accuracy 91+\end{tabular} &
  hourglass \\ \hline
zhao2018autonomous  & Shown in the form of figures & SSD+dual Kalman filters                 \\ \hline
wang2019orientation & 81.3                         & YOLOv3+SIFT                             \\ \hline
usmankhujaev2020real &
  \begin{tabular}[c]{@{}l@{}}100 Daytime \\ 89.83 Daytime(flipped) \\ 86.11 Nighttime(flipped)\end{tabular} &
  yoloV3+kalman filter \\ \hline
kwan2018compressiv  & For compressive measurements & ResNet                                  \\ \hline
fernandez2019real &
  86.96 MOTA on MOT 15\cite{leal2015motchallenge} &
  CNN detector+DCF+Kalman filter \\ \hline
\end{tabular}%
}
\caption{Some traffic-related works using deep learning. The default dataset is generated by the author of each work. The default metric is accuracy.}
\label{tab:trackingontraffic}
\end{table}

-traffic monitoring:
tracking by detecting

DL detect+ extact spatio-temporal features:
                    \cite{fernandez2019real}ehicles are identified through a deep learning based detector. Second, tracking is performed with a combination of a Discriminative Correlation Filter and a Kalman Filter.
                 86.96  CNN detector+DCF+Kalman filter MOT 15\cite{}
                    

-qiu2018kestrel      YOLO+KLT     75.9 RECALL 88.6P TKI and Desktop   


-lopez2019boosting Faster R-CNN   0.305AP subset:M-30 0.662 subset:M-30-HD 0.381 subset:Urban1          GRAM-RTM
-xu2017car    Faster R-CNN 98.43     

-scheidegger2018mono         CNN+Poisson multi-Bernoulli mixture tracking filter(PMBM)\cite{garcia2018poisson} 80.04 mota kitti
   
-zou2019multi Siamese network+SPP+Markov Decision Process(MDP)
multiple-object tracking accuracy (MOTA) 75.29 campus 76.06 urban 78.14 highway on KITTI

-li2019spatio FPN+tracking loss 83.2IDF1 nivida AI city

-nikodem2020multi  hourglass single-camera tracing accuracy of at least 97 multi-camera east 91

-zhao2018autonomous  SSD+dual Kalman filters Performance shown in form of figures

- wang2019orientation  YOLOv3+SIFT 81.3
- usmankhujaev2020real yoloV3+kalman filter 100 Daytime 89.83 Daytime(flipped) Nighttime(flipped) 86.11

DL: 
-kwan2018compressiv  ResNet compressive measurements
%\cite{wang2018learning}

%but deep learning is relatively time-consumi


$RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$
$p_i$ and $a_i$ represent the predicted and actual outcome.


NVIDIA AI CITY challenge\cite{ai_city_challenge}
Track 1: 31 video clips (about 9 hours in total) captured from 20 unique camera views



Vehicle Counting 9 hours of videos captured from 20 different vantage points
covering various lighting and weather conditions most 10fps

Track 2:Re-ID
56,277 images, of which 36,935 come from 333 object identities 

track 3:Vehicle Tracking

215.03 minutes of videos collected from 46 cameras spanning 16 intersections
 300K bounding boxes for 880 distinct annotated vehicle identities.
 
track 4: Traffic Anomaly Detection 
200 15mins videos 30fps
Anomalies can be due to car crashes or stalled vehicles


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Task & Models \\ \hline
scene understanding &
  \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet} pixel accuracy>95 Cityscapes\\ \cite{lyu2019esnet} 63.2 mIoU Cityscapes\\ \cite{deng2017cnn} 54.5 mIoU Cityscapes\\ \cite{saez2018cnn} 59.3  mIoU Cityscapes\\ \cite{kendall2015bayesian} 63.1 mIoU  CamVid\end{tabular} \\ \hline
Free space estimation &
  \begin{tabular}[c]{@{}l@{}}\cite{ohgushi2020road} 21.9 mIoU\\ \cite{hua2019small} Path planning accuracy\\  0.15m Indoor and 0.27m Outdoor\\ \cite{levi2015stixelnet} 0.87 AUC \\ 89.12\% maxF SEGMENTATION on KITTI\\ \cite{deepika2017obstacle} 0.9667 IoU\end{tabular} \\ \hline
Stixel representation &
  \begin{tabular}[c]{@{}l@{}}\cite{cordts2017stixel} 83.1 exact Disparity accuracy \\ \cite{schneider2016semantic} 7.8 Disparity accuracy\\ \cite{erbs2012stixmentation}88.64 Stixel-wise percentage accuracy\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Some semantic segmentation works In the traffic field. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:semanticwork}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Works &
  Methods \\ \hline
scene understanding &
  \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet} pixel accuracy$>$95 Cityscapes\\ \cite{lyu2019esnet} 63.2 mIoU Cityscapes\\ \cite{deng2017cnn} 54.5 mIoU Cityscapes\\ \cite{saez2018cnn} 59.3  mIoU Cityscapes\\ \cite{kendall2015bayesian} 63.1 mIoU  CamVid\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Edge Detection Network+Fusion\\ CNN+pyramid pooling module\\ Autoencoder\\ Bayesian Autoencoder\end{tabular} \\ \hline
Free space estimation &
  \begin{tabular}[c]{@{}l@{}}\cite{ohgushi2020road} 21.9 mIoU\\ \cite{hua2019small} Path planning accuracy\\  0.15m Indoor and 0.27m Outdoor\\ \cite{levi2015stixelnet} 0.87 AUC \\ 89.12\% maxF SEGMENTATION on KITTI\\ \cite{deepika2017obstacle} 0.9667 IoU\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Autoencoder+fusion+optical flow\\ \\ CNN\\ \\ SegNet\end{tabular} \\ \hline
Stixel representation &
  \begin{tabular}[c]{@{}l@{}}\cite{schneider2016semantic} \\ 7.8 Disparity Error on KITTI 15.2 on Ladicky\cite{ladicky2014pulling}\\ \cite{cordts2017stixel} 83.1 exact Disparity accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}FCN+SGM\\ \\ FCN+SGM+graphical model\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Some semantic segmentation works In the traffic field.}
\label{tab:semanticwork}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Works &
  Methods \\ \hline
\begin{tabular}[c]{@{}l@{}}obtain comprehensive\\  vehicle information\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2015monocular} 59.0 object recall,\\ 83.1\% of the randomly sampled foreground pixel pairs ordered on KITTI \\ \cite{mou2018vehicle} 95.87 F1 score on ISPRS\\ \cite{zhang2020traffic} 97\%  vehicle types accuracy\\ \cite{huang2018measuring} 1.333 front 4.698 side-way KITTI\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CNN+MRF\\ 11\\ ResFCN\\ Mask R-CNN\\ Mask R-CNN\end{tabular} \\ \hline
Lane detection &
  \begin{tabular}[c]{@{}l@{}}\cite{neven2018towards} 96.4\% accruacy\\ \cite{roberts2018dataset}IoU Mapillary 82.9  CityScapes 85.2\\  KITTI 83.8 author's dataset 95\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}multi-task CNN\\ SegNet\end{tabular} \\ \hline
3D reconstruction &
  \begin{tabular}[c]{@{}l@{}}\cite{hadi2020semantic} AP@50\% 8.862 CityScapes 43.949\\ IDD\cite{varma2019idd} 5.643WildDash\cite{zendel2018wilddash}\end{tabular} &
  Mask R-CNN \\ \hline
\end{tabular}%
}
\caption{Some instance segmentation works In the traffic field. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:instancework}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works                  & Performance                                        & Methods                                   \\ \hline
\cite{nguyen2020anomaly}      & F1 score 0.9412   AI City Challenge 2019           & GAN                                       \\ \hline
\cite{yao2019unsupervised}    & 60.1 AUC on A3D Dataset & \begin{tabular}[c]{@{}l@{}}Auto Encoder-Decoder\\ with GRU\end{tabular}                   \\ \hline
\cite{tian2019automatic}      & 90.02 AP  CAD-CVIS                                 & YOLO-CA                                   \\ \hline
\cite{kim2020pre}            & 0.82                                               & 3D conv                                   \\ \hline
\cite{ijjina2019computer}     & 71                                                 & 3D conv                                   \\ \hline
\cite{shah2018cadp}           & 47.25 on CADP           & \begin{tabular}[c]{@{}l@{}}DSA-RNN\cite{chan2016anticipating}\\ Faster R-CNN\end{tabular} \\ \hline
\cite{srinivasan2020novel}    & 78.2 on CADP                                       & Detection Transformer\cite{carion2020end} \\ \hline
\cite{suzuki2018anticipating} & 99.1 mAP                & QRNN\cite{bradbury2016quasi}+DeCAF\cite{donahue2014decaf}                                 \\ \hline
\cite{giannakeris2018speed}   & F1-score 0.33 RMSE 227   on NVIDIA CITY Track 2    & Faster RCNN                               \\ \hline
\cite{arceda2018fast}         & 89                                                 & YOLO+ViF\cite{hassner2012violent}+SVM     \\ \hline
\cite{biradar2019challenges}  & F1-score 0.3838 RMSE 93.61 on NVDIA CITY Track 3   & YOLOv2+ CNN                               \\ \hline
\cite{xu2018dual}             & F1-score 0.8649 RMSE 3.6152 on NVIDIA CITY Track 2 & Mask-RCNN+ ResCNN                         \\ \hline
\cite{doshi2020fast}          & F1-score 0.5926 RMSE 8.2386 on NVIDIA CITY track 4 & YOLO+KNN+K-means                          \\ \hline
\cite{zhou2016spatial} & 95.2 on U-turn dataset \cite{benezeth2009abnormal} & 3D CNN                                    \\ \hline
\cite{franklin2020traffic}    & 100 and 95.34 for input video 1 and video 2            & YOLOv3                                  \\ \hline
\end{tabular}%
}
\caption{Some recent deep learning works for video-based traffic abnormal detection. Unless otherwise specified, the non-indicated numbers is the accuracy}
\label{tab:abnormaldetect}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works               & Performance                  & Methods                                 \\ \hline
\cite{qiu2018kestrel}      & 75.9 Recall 88.6 Accuracy    & YOLO+KLT                                \\ \hline
\cite{lopez2019boosting} &
  \begin{tabular}[c]{@{}l@{}}0.305AP subset:M-30 0.662AP subset:M-30-HD \\ 0.381AP subset:Urban1 of  GRAM-RTM\end{tabular} &
  Faster R-CNN \\ \hline
\cite{xu2017car}           & 98.43                        & Faster R-CNN                            \\ \hline
\cite{scheidegger2018mono} & 80.04 MOTA on KITTI          & CNN+PMBM filter\cite{garcia2018poisson} \\ \hline
\cite{zou2019multi} &
  \begin{tabular}[c]{@{}l@{}}75.29MOTA campus \\ 76.06MOTAurban \\ 78.14MOTA highway \\ on KITTI\end{tabular} &
  Siamese network+SPP+MDP \\ \hline
\cite{li2019spatio}        & 83.2IDF1 nivida AI city      & FPN+tracking loss                       \\ \hline
\cite{nikodem2020multi} &
  \begin{tabular}[c]{@{}l@{}}MOTA 97+\\ MCTA 91+\end{tabular} &
  hourglass \\ \hline
\cite{zhao2018autonomous}  & Shown in the form of figures & SSD+dual Kalman filters                 \\ \hline
\cite{wang2019orientation} & 81.3                         & YOLOv3+SIFT                             \\ \hline
\cite{usmankhujaev2020real} &
  \begin{tabular}[c]{@{}l@{}}100 Daytime \\ 89.83 Daytime(flipped) \\ 86.11 Nighttime(flipped)\end{tabular} &
  yoloV3+kalman filter \\ \hline
\cite{kwan2018compressive}  & For compressive measurements & ResNet                                  \\ \hline
\cite{fernandez2019real} &
  86.96 MOTA on MOT 15\cite{leal2015motchallenge} &
  CNN detector+DCF+Kalman filter \\ \hline
\end{tabular}%
}
\caption{Some traffic-related tracking works using deep learning. The default dataset is generated by the author of each work. The default metric is accuracy.}
\label{tab:trackingontraffic}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Methods &
  Methods \\ \hline
\multirow{}{}{Vehicle Detection} &
  R-CNN family &
  \begin{tabular}[c]{@{}l@{}}\cite{espinosa2017vehicle} 70\\ \cite{wang2019comparative} \\ \cite{wang2017evolving}84.43 DETRAC dataset\\ \cite{soin2017moving}  100\\ \cite{zhang2017application} 96.5\\ \cite{peppa2018urban} 97\end{tabular} \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{sang2018improved} 99.51  BIT-Vehicle\\ \cite{kim2019multi}85.29 UA-DETRAC\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2019vehicle} 77.94 mAP  UA-DETRAC\\ \cite{chen2020inception} 86.2 KITTI 87.4UVD\\ \cite{cao2020front} 92.18 KITTI\\ \cite{peppa2018urban} 98.2\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \cite{6778050} 99.7 \\ \hline
\multirow{}{}{Plate Detection} &
  R-CNN family &
  \cite{lee2016real} 99.94 \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{hsu2017robust} \\ \cite{kessentini2019two} 97.67\% on GAP-LP dataset  91.46 on Radar\\ \cite{khazaee2020real} 97.9\\ \cite{xie2018new} 98.32 UCSD PKU\\ \cite{chen2019automatic} 98.22 AOLP\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{ren2020implementation} 92\\ \cite{hu2020mobilenet} 90.12\\ \cite{danilenko2020license} 94+\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \begin{tabular}[c]{@{}l@{}}\cite{kim2017deep} 98.39 on Caltech\\ \cite{selmi2017deep} 94.8 on Caltech\\ \cite{masood2017license} 99.09 US 99.64 EU\end{tabular} \\ \hline
\multirow{}{}{\begin{tabular}[c]{@{}l@{}}Traffic Sign \\ Detection\end{tabular}} &
  R-CNN family &
  \begin{tabular}[c]{@{}l@{}}\cite{qian2016road} 85.58\\ \cite{shao2019improved} 69.56 gtsdb+ctsd\\ \cite{zhang2020cascaded} 98.7 GTSDB\\ \cite{zuo2017traffic} 0.3449 on CCF2016\\ \cite{wu2019traffic} mAP  91.75  GTSDB\\ \cite{peng2016traffic} mAP ~90 GTSDB\end{tabular} \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2017real} 96.69 on CCTSDB and GTSDB\\ \cite{Tai_2020} 99.1 mAP\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{gao2019traffic} 91.0 GTSDB\\ \cite{you2020traffic}0.75 TT100K\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \begin{tabular}[c]{@{}l@{}}\cite{zhu2016traffic}91 TT100K\\ \cite{wu2013traffic}AUC 99.73 “danger” , 97.62 "mandatory" on GTSDB\\ \cite{shustanov2017cnn} 99.94 GTSDB\end{tabular} \\ \hline
\end{tabular}%
}
\caption{some object detection tasks of traffic works. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:objectdetection}
\end{table}


LP: AOLP\cite{hsu2012application}
caltech\cite{}

\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Accuracy &
  $\frac{Correct predictions}{Total predictions}$ \\ \hline
Recall (R) &
  $\frac{TP}{TP+FN}$ \\ \hline
Precision (P) &
  $\frac{TP}{TP+FP}$ \\ \hline
F1 score &
  $2\times\frac{P\times R}{P+ R}$ \\ \hline
Pixel Accuracy (PA) &
  $\frac{TP+TN}{TP+TN+FP+FN}$ \\ \hline
Normalized error (mean)\cite{huang2018measuring} &
  \begin{tabular}[c]{@{}l@{}}$normalized error=\frac{|d-d_{gt}|}{d_{gt}}$. \\ $d$ is the calculated distance and \\ $d_{gt}$ is the ground truth of distance.\end{tabular} \\ \hline
Average Precision (AP) &
  $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class) \\ \hline
mean Average Precision (mAP) &
  $mean(AP_i)$ \\ \hline
Intersection over Union (IoU) &
  \begin{tabular}[c]{@{}l@{}}$\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$\\ $B_{gt}$: ground truth bounding box\\ $B_{p}$: predicted bounding box\end{tabular} \\ \hline
Disparity accuracy &
   \\ \hline
Stixel-wise percentage accuracy &
  Similar to PA \\ \hline
Identification F1-Score (IDF1) &
  $IDF1=\frac{2IDTP}{2IDTP+IDFP+IDFN}$ \\ \hline
multiple object tracking accuracy (MOTA) &
  \begin{tabular}[c]{@{}l@{}}$MOTA=1-\frac{FN+FP+\Phi}{T}$\\ $\Phi$ denotes the number of fragmentations\end{tabular} \\ \hline
Multi-camera Tracking Accuracy (MCTA) &
  \begin{tabular}[c]{@{}l@{}}$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$\\ $M^w$: within-camera identity mismatches \\ $T^w$:  true within-camera detections\\ $M^h$:  handover mismatches\\ $T^h$:  true handover detections\end{tabular} \\ \hline

RMSE & $RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$ \\ \hline
\end{tabular}%
}
\caption{Some metrics to evaluate traffic works.TP:True Positive TN: True Negative FP:False Positive FN:False Negative}
\label{tab:somemetrics }
\end{table}
UCF-Crimes\cite{sultani2018real}: 1900 sequences 128hours. 151 events
13 realistic anomalies such as fighting, road accident, burglary, robbery, etc
No spatial annotation

DAD\cite{chan2016anticipating}: 1730 sequences 2.4 hours 620 events
spatio-temporal annotation 
dashcam accident videos.

CADP\cite{shah2018cadp}: 1416 sequences 5.2 hours 1416 events
include multi-accident sequences
varied environment
captured by CCTV
\begin{table*}[]
\centering
%\begin{adjustbox}{angle=90}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Paper:  [REF](year)                   & \cite{shirazi2016looking}(2016) & \cite{sivaraman2013looking}(2013) &\cite{khan2017uav} (2017) & \cite{zheng2014traffic}(2014) & \cite{wali2015comparative}(2015) &\cite{morris2013understanding}(2013) & \cite{mukhtar2015vehicle}(2015)  & \cite{janai2017computer}(2017) & \cite{nguyen2018deep}(2018)& \cite{badue2020self}(2020) &\cite{yurtsever2020survey} (2020) & \textbf{Ours}\\ \hline
Human-driven Vehicle       & H    & H    & H    & H    & H    & H    & H       & L  & H & L    & L    & H    \\ \hline
Safety Assessment Analysis & H    & L    & L    & H    & L    & M    & L        & L & L  & L    & L    & M    \\ \hline
Video-based Method         & H    & H    & H    & L    & H    & H    & H        & H & L  & M    & M    & H    \\ \hline
Deep Learning Method       & L    & M    & M    & L    & L    & L    & L        & H & H & M    & H    & H    \\ \hline
Perspective                & E    & E    & E    & E    & I    & E    & I        & I & E  & I    & I    & E    \\ \hline

relations to AVs       & L    & L    & L    & L    & L    & L    & L        & H & L & H   & H    & H    \\ \hline
relations to insurance       & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & L    \\ \hline
relations to  psychology        & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & M    \\ \hline
relations to  Crowd-sourcing        & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & L    \\ \hline
Network Analysis        & X    &H   & M    & M    & X    & H    & X       & H & H &M    & M    & H    \\ \hline
\end{tabular}%
}
%\end{adjustbox}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective.}  
\label{tab:surveys}
\end{table*}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline \rowcolor{gray}
\textbf{Paper: [REF](year)} &
  \cite{shirazi2016looking}(2016) &
  \cite{sivaraman2013looking}(2013) &
  \cite{khan2017uav} (2017) &
  \cite{zheng2014traffic}(2014) &
  \cite{wali2015comparative}(2015) &
  \cite{morris2013understanding}(2013) &
  \cite{mukhtar2015vehicle}(2015) &
  \cite{janai2017computer}(2017) &
  \cite{nguyen2018deep}(2018) &
  \cite{badue2020self}(2020) &
  \cite{yurtsever2020survey} (2020) &
  \cite{wang2019enhancing}(2019) &
  \cite{grigorescu2020survey}(2020) &
  \cite{mozaffari2020deep}2020 &
  \textbf{Ours} \\ \hline
\begin{tabular}[c]{@{}c@{}}Human-driven \\ Vehicle\end{tabular}         & H & H & H & H & H & H & H & L & H & L & L & H & L & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Safety Assessment\\  Analysis\end{tabular}   & H & L & L & H & L & M & L & L & L & L & L & L & M & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Video-based\\  Method\end{tabular}           & H & H & H & L & H & H & H & H & L & M & M & M & H & M & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Deep Learning \\ Method\end{tabular}         & X & X& X & X & L & X & L & H & H & H & H & H & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Perspective\\ ~\end{tabular}                 & E & E & E & E & I & E & I & I & E & I & I & E & I & E & E \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\  AVs\end{tabular}             & L & L & L & L & L & L & L & H & L & H & H & M & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ insurance\end{tabular}       & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ psychology\end{tabular}      & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to  \\ Crowd-sourcing\end{tabular} & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\ Edge Computing\end{tabular}   & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Network\\ Analysis\end{tabular}                                                        & X & H & M & M & X & H & X & H & H & M & M & H & X& M & H \\ \hline
\end{tabular}%
}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}}
\label{tab:surveys}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline \rowcolor{gray}
\textbf{Paper: [REF](year)} &
  \cite{shirazi2016looking}(2016) &
  \cite{sivaraman2013looking}(2013) &
  \cite{khan2017uav} (2017) &
  \cite{zheng2014traffic}(2014) &
  \cite{wali2015comparative}(2015) &
  \cite{morris2013understanding}(2013) &
  \cite{mukhtar2015vehicle}(2015) &
  \cite{janai2017computer}(2017) &
  \cite{nguyen2018deep}(2018) &
  \cite{badue2020self}(2020) &
  \cite{yurtsever2020survey} (2020) &
  \cite{wang2019enhancing}(2019) &
  \cite{grigorescu2020survey}(2020) &
  \cite{mozaffari2020deep}2020 &
  \textbf{Ours} \\ \hline
\begin{tabular}[c]{@{}c@{}}Human-driven \\ Vehicle\end{tabular}         & H & H & H & H & H & H & H & L & H & L & L & H & L & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Safety Assessment\\  Analysis\end{tabular}   & H & L & L & H & L & M & L & L & L & L & L & L & M & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Video-based\\  Method\end{tabular}           & H & H & H & L & H & H & H & H & L & M & M & M & H & M & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Deep Learning \\ Method\end{tabular}         & X & X& X & X & L & X & L & H & H & H & H & H & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Perspective\\ ~\end{tabular}                 & E & E & E & E & I & E & I & I & E & I & I & E & I & E & E \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\  AVs\end{tabular}             & L & L & L & L & L & L & L & H & L & H & H & M & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ insurance\end{tabular}       & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ psychology\end{tabular}      & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to  \\ Crowd-sourcing\end{tabular} & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\ Edge Computing\end{tabular}   & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Network\\ Analysis\end{tabular}                                                        & X & H & M & M & X & H & X & H & H & M & M & H & X& M & H \\ \hline
\end{tabular}%
}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}}
\label{tab:surveys}
\end{table*}
\begin{table*}[]
\centering
\caption{Summary of related review papers. 
%'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}\xc{Updated for the latest chose surveys. The text content still needs to update. Additionally, it seems we removed edge computing in this version, which means we need to remove the row for edge computing.}
\arr{Good job. I like this Table, and it can be the instrumental in getting this paper accepted if we convince the reviewer that it is accurate and complete. A few more comments: a) it should be consistent with text, b) it is ok to include some older References and if we need we can include 2 tables one on top of another, c) if we include more review papers we can have "o" with note that this topic is covered but is outdated, d) it might be questionable that for many topics like "Related to Insurance", "crowd-sourcing", and "Edge computing", is not covered by any of the previous papers, it might be better for only 2 of these unique aspects (not all of them) you include a paper focused only on this matter, like finding a paper that reviews edge computing from traffic data. e) Bring back the Edge computing from the Access, if it is removed it must be a mistake, f) you can also include some new aspects: like "sensors", "data collection methods", "public tools and datasets", "roadside infrastructures", g) if you include Human-driven vehicles, better to add another row for "Autonomous vehicles" right after it (perhaps you can just move relation to AVs to 2nd row".}
}
\label{tab:surveys}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline\rowcolor{gray}
\textbf{Paper:   {[}REF{]}} &
  REF: \cite{hu2020review} &  
  REF: \cite{mozaffari2020deep} &  
  REF: \cite{grigorescu2020survey} & 
  REF: \cite{yurtsever2020survey} &   
  REF: \cite{janai2017computer} &
  REF: \cite{badue2020self} &
  REF: \cite{kumaran2019anomaly} &
  REF: \cite{wang2019enhancing} &
  REF: \cite{nguyen2018deep} &
  REF: \textbf{Ours} \\ 
\textbf{(year)} &
  (2020) &  
  (2020) &  
  (2020) &
  (2020) &   
  (2020) &
  (2020) &
  (2019) &
  (2019) &
  (2018) &
  \textbf{ } \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Human-driven\\      Vehicle\end{tabular}}          & $\surd$ & $\surd$ &    &    &    &    & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Safety   Assessment\\      Analysis\end{tabular}}  & $\surd$ & $\surd$ & $\surd$ &    &    &    & $\surd$   &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Video-based\\      Method\end{tabular}}            & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Deep   Learning\\      Method\end{tabular}}        & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Avs\end{tabular}}            & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      insurance\end{tabular}}      &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      psychology\end{tabular}}     &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Crowd-sourcing\end{tabular}} &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Edge Computing\end{tabular}} &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Network\\      Analysis\end{tabular}}              & $\surd$ & $\surd$ &    &    &    &    & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\end{tabular}%
}
\end{table*}


\begin{table*}[]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray}
\textbf{Task}                                                         & \textbf{DataSet}            & \textbf{Description }              \\ \hline Object Classification
                                     & Cifar-10/100       & Natural image             \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & MNIST              & Hand-writen digits        \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & ImageNet           & Natural image             \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & Fasion-MNIST       & Fasion items              \\ \hline
Scene Classification                      & UIUC-Sports        & Sports events             \\ \cline{2-3} 
                                                             & Place365           & Indoor and outdoor scenes \\ \cline{2-3} 
                                                             & ADE20k             & Indoor and outdoor scenes \\ \hline
Fine-grained Classification                 & CUB200             & Birds                     \\ \cline{2-3} 
                                                             & Stanford dogs/cats & Dogs/Cats                 \\ \cline{2-3} 
                                                             & Oxford flowers     & Flowers                   \\ \hline
\end{tabular}
\end{center}
\caption{Differences datasets for classification tasks, which can be used for initial performance analysis of DL-based classification methods, even in the context of traffic analysis.} 
%\arr{This is good but not relevant to our paper. Develop tables for datasets or methods relevant to classification tasks in traffic analysis. In general our goal is not reviewing DL methods but reviewing their use, applicability, and role in Traffic [safety] analysis. A table with a header like "method[REF]  - DL Method -  application  accuracy", and in DL method you put the method name like GoogleNet and in the application you put something like vehicle type classification}\xc{I think we can remove the table. Traffic-related scene classification is often solved by segmentation methods. And most of the works(On Table.\ref{tab:objectdetection}, except\cite{soin2017moving,peppa2018urban,6778050} ) we mentioned on the object detection section also do car type classification. We can mention it on this section.}}
\label{tab:Classifaction Datasets}
\end{table*}

\begin{table*}[]
\centering
\caption{Summary of related review papers. 
%\arr{Good job. I like this Table, and it can be the instrumental in getting this paper accepted if we convince the reviewer that it is accurate and complete. A few more comments: a) it should be consistent with text, b) it is ok to include some older References and if we need we can include 2 tables one on top of another, c) if we include more review papers we can have "o" with note that this topic is covered but is outdated, d) it might be questionable that for many topics like "Related to Insurance", "crowd-sourcing", and "Edge computing", is not covered by any of the previous papers, it might be better for only 2 of these unique aspects (not all of them) you include a paper focused only on this matter, like finding a paper that reviews edge computing from traffic data. e) Bring back the Edge computing from the Access, if it is removed it must be a mistake, f) you can also include some new aspects: like "sensors", "data collection methods", "public tools and datasets", "roadside infrastructures", g) if you include Human-driven vehicles, better to add another row for "Autonomous vehicles" right after it (perhaps you can just move relation to AVs to 2nd row".}
\xc{Updated. The paper with '*' means although this paper is related but outdated.} \arr{This new table is good. Split miscellaneous points as we discussed, 2) use \checkmark and L\checkmark if a topic is covered in less details. I means instead of using "*" for limited content per paper it is better to use it per topic and you already have this information from the previous TABLe!!!. }}
\label{tab:surveys}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline\rowcolor{gray}
\textbf{Paper}                                                                                                                                                      & \cite{hu2020review}Hu et al.& \cite{mozaffari2020deep}Mozaffari et al. & \cite{grigorescu2020survey}Grigorescu et al. & \cite{yurtsever2020survey}Yurtsever et al. & \cite{janai2017computer}Janai et al. & \cite{badue2020self}Badue et al. & \cite{kumaran2019anomaly}kumaran et al. & \cite{wang2019enhancing}Wang et al. & \cite{nguyen2018deep}Nguyen et al.& *\cite{shirazi2016looking}shirazi et al.& *\cite{mukhtar2015vehicle}Mukhtar et al. & *\cite{morris2013understanding} Morris et al.& Ours \\ \hline
\textbf{Year}                                                                                                                                                       & 2020                      & 2020                           & 2020                              & 2020                             & 2020                           & 2020                       & 2019                            & 2019                           & 2018                        & 2016                            & 2015                      & 2013                           &      \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Human-driven\\      Vehicle\end{tabular}}                                                                                        & $\surd$                        & $\surd$                             &                                   &                                  &                                &                            & $\surd$                              & $\surd$                             & $\surd$                          & $\surd$                              & $\surd$                        & $\surd$                             & $\surd$   \\ \hline
\textbf{Avs}                                                                                                                                                        & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              &                                &                             &                                 &                           &                                & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Safety   Assessment\\      Analysis\end{tabular}}                                                                                & $\surd$                        & $\surd$                             & $\surd$                                &                                  &                                &                            & $\surd$                              &                                &                             & $\surd$                              &                           & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Video-based\\      Method\end{tabular}}                                                                                          & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              & $\surd$                             & $\surd$                          & $\surd$                              & $\surd$                        & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Deep   Learning\\      Method\end{tabular}}                                                                                      & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              & $\surd$                             & $\surd$                          &                                 &                           &                                & $\surd$   \\ \hline
\textbf{Sensors}                                                                                                                                                    & $\surd$                        &                                & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         &                                 &                                &                             & $\surd$                              & $\surd$                        &                                &      \\ \hline
\textbf{Datasets}                                                                                                                                                   &                           &                                & $\surd$                                & $\surd$                               & $\surd$                             &                            & $\surd$                              &                                &                             & $\surd$                              &                           & $\surd$                             &      \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Network\\      Analysis\end{tabular}}                                                                                            & $\surd$                        & $\surd$                             &                                   &                                  &                                &                            & $\surd$                              & $\surd$                             & $\surd$                          &                                 &                           & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Miscellaneous\\       Points\\      (Insurance, Psychology, \\      Crowd-sourcing,\\ Vehicular Edge Computing, \\      etc.,)\end{tabular}} &                           &                                &                                   &                                  &                                &                            &                                 &                                &                             &                                 &                           &                                & $\surd$   \\ \hline
\end{tabular}%
}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{List of sample problems to assess the overall safety of a highway segment. The short codes include MOT: multi-object tracking, OD: object detection, IS: instance segmentation, TE: trajectory extraction, SS: semantic segmentation, EP: environment prior, C: classification. The tasks with '*' meaning that these tasks can be solved by obtaining the relationships (distance, velocity) among vehicles and determining a threshold from the relationships. \arr{use consistent format like "Traffic Blocked--> Traffic blocked".} \arr{Good job, as we dicussed you can add more detailed steps and use '*' for steps that can be included or can be useful but is not necessary like denoising, video stabilization, super resolution, trajectory smoothing,etc. }}
\label{tab:problem}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{|l|l|c|}
\hline\rowcolor{gray}
\textbf{Task}                                & \textbf{Processing Steps} & \textbf{Examples}                         \\ \hline
Vehicle Stopped on Shoulder            & EP-OD/MOT                   & \cite{xu2018dual}                                       \\ \hline
Car Accident                           & OD/MOT                      & \cite{tian2019automatic,nguyen2020anomaly}              \\ \hline
Emergency Vehicle on The Road          & Fine-grained OD             & \cite{nayak2019vision}                                  \\ \hline
Careless/evasive Lane Change           & MOT-TE-C                    & \cite{chen2017dangerous,ramyar2016identification}       \\ \hline
Debris in Roadway                      & EP-OT/SS                    & \cite{ohgushi2020road,hua2019small,deepika2017obstacle} \\ \hline
Traffic Blocked (Slowed-down)          & MOT-TE-(SE)                 & \cite{kaltsa2018multiple,wang2019abnormal}              \\ \hline
Sharp Braking                                 & MOT-TE                    & \cite{jiang2015analysis} \\ \hline
Passing Red Traffic Light              & OD(for sign may needed)-MOT & \cite{wonghabut2018traffic}                             \\ \hline
Traffic Composition                           & OD/MOT                    & \cite{dai2019video}      \\ \hline
*Vehicle Driving Obviously Excessively   Slow & MOT-TE                    &   -                                        \\ \hline
*Vehicle Driving Obviously Excessively   Fast & MOT-TE                    &   -                                        \\ \hline
Vehicle Driving in The Prohibited Area & EP-MOT-TE                   & \cite{nowosielski2016automatic}                         \\ \hline
Invalid Car in HOV                            & EP-OD/MOT                 &  -                                         \\ \hline
Improper (Careless) Entering the Road  & EP-MOT-C                    & \cite{datondji2016survey}                               \\ \hline
Improper (Careless) Exiting the Road   & EP-MOT-C                    & \cite{datondji2016survey}                               \\ \hline
Zigzag Driving                                & MOT-TE-C                  & \cite{chen2017dangerous} \\ \hline
*Distance Violation to Front Vehicle          & MOT-C                     &  -                                         \\ \hline
*Distance Violation to Side Vehicle           & MOT-C                     &  -                                         \\ \hline
Violation of the Lines                 & ET-MOT-TE                   & \cite{nowosielski2016automatic}                         \\ \hline
Pedestrian on The Road                        & OD/MOT                    &  -                                         \\ \hline
Bike/Motorcycle on The Road                   & OD/MOT                    &  -                                         \\ \hline
Trailer {[}Oversized Car{]} on The Road       & OD/MOT                    &  -                                         \\ \hline
\end{tabular}%
}
\end{table*}

\begin{table*}
\centering
\caption{Summary of related review papers. The paper with '*' means although this paper is related but outdated. $L\surd$ denotes a topic is covered in fewer details. }
\label{tab:surveys}\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule 
 \textbf{Paper}                                                                                                     & \cite{hu2020review}Hu et al.& \cite{mozaffari2020deep}Mozaffari et al. & \cite{grigorescu2020survey}Grigorescu et al. & \cite{yurtsever2020survey}Yurtsever et al. & \cite{janai2017computer}Janai et al. & \cite{badue2020self}Badue et al. & \cite{kumaran2019anomaly}kumaran et al. & \cite{wang2019enhancing}Wang et al. & \cite{nguyen2018deep}Nguyen et al.& *\cite{shirazi2016looking}shirazi et al.& *\cite{mukhtar2015vehicle}Mukhtar et al. & *\cite{morris2013understanding} Morris et al.& Ours         \\ 
\midrule 
\textbf{Year}                                                                          & 2020                  & 2020                  & 2020                  & 2020                  & 2020                  & 2020                  & 2019                  & 2019                  & 2018                  & 2016                  & 2015                  & 2013                  &                              \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Human-driven}\\\textbf{ Vehicle}\end{tabular}       & $\surd$               & $\surd$               &                       & $\surd$               &                       &                       & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$                      \\ 

\textbf{Avs}                                                                           & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       & $L\surd$              &                       &                       &                       & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Safety Assessment}\\\textbf{ Analysis}\end{tabular} & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       &                       & $\surd$               &                       &                       & $\surd$               &                       & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{CV-based}\\\textbf{ Method}\end{tabular}            & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Deep Learning}\\\textbf{ Method}\end{tabular}       & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $L\surd$              &                       &                       &                       & $\surd$                      \\ 

\textbf{Sensors}                                                                       & $\surd$               &                       & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       &                       &                       & $\surd$               & $\surd$               &                       &         $\surd$                     \\ 

\textbf{Datasets}                                                                      &                       &                       & $\surd$               & $\surd$               & $\surd$               &                       & $\surd$               &                       &                       & $\surd$               &                       & $\surd$               &  $\surd$                            \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Network}\\\textbf{ Analysis}\end{tabular}           & $\surd$               & $\surd$               &                       &                       &                       &                       & $\surd$               & $\surd$               & $\surd$               &                       &                       & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Vehicular }\\\textbf{Edge Computing}\end{tabular}   &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       & $\surd$                      \\ 

%\textbf{\textbf{Psychology}} %              
\begin{tabular}[c]{@{}c@{}}\textbf{Behavioral \&}\\\textbf{Driver Cognition}\end{tabular}
& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & {$\surd$}  \\
\bottomrule
\end{tabular}}
\end{table*}

==> excluded.tex <==


\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric}     & \textbf{Definition} & \textbf{Features}                                                                                                                         \\ \hline
MaxS*       & $\max v$         & A simple but effective measure of the severity of a collision.                                                                   \\ \hline
$\Delta v$*    & $\Delta v$          & An effective indicator of the severity of a collision.                                                                           \\ \hline
TTC &
  $TTC =\frac{X_L-X_F}{v_F-v_L}$ &
  \begin{tabular}[c]{@{}l@{}}Provides more information than PET; assumes that involved vehicles are at a constant speed;\\ cannot reflect the severity.\end{tabular} \\ \hline
PET &
  $PET =t_2-t_1$ &
  \begin{tabular}[c]{@{}l@{}}Can be easily captured and computed; suitable for assessing intersecting conflicts; \\ only suitable for the cases of transversal trajectories;\\ cannot reflect the severity.\end{tabular} \\ \hline
Initial DR & $DR_{t=0}$          & A basic indicator; cannot consider the following vehicle's acceleration/deceleration.                                                        \\ \hline
DRAC       &$TTC =\frac{(v_F-v_L)^2}{X_L-X_F}$         & \begin{tabular}[c]{@{}l@{}}No need to directly observe the deceleration rate; \\ does not work for lateral movement\end{tabular}      \\ \hline
CPI*       & $CPI_i=\frac{\sum_{t=t_i}^{tf_i}P(DRAC_{i,t})\geq MADR\Delta t\cdot b}{T_i}$          & Considers more factors such as traffic and road conditions compared to DRAC;                                                         \\ \hline
PSD*        &\begin{tabular}[c]{@{}l@{}}$PSD =\frac{RD}{MSD}$;\\ $ PSD =\frac{v^2}{2MADR} $ \end{tabular}      & \begin{tabular}[c]{@{}l@{}}Works for a conflict with a single vehicle involved; \\ \rarely used for specific safety problems.\end{tabular} \\ \hline
UD &
  $UD=\frac{\sum_{S=1}^{S_t}\sum_{V=1}^{V_t}unsafety_{V,S}\cdot d}{TL}$ &
  \begin{tabular}[c]{@{}l@{}} Delivers more accurate information than typical micro-simulation outputs;\\ allows comparison between simulation scenarios or links;\\ some parameters are difficult to capture automatically;\\ only applicable to identical trajectories.\end{tabular} \\ \hline
  
  MSE &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle violate safety boundary of another.\\ Safety boundary: $d_{min}^{long,same}$(Eq.\ref{eq:d_long_same}) $d_{min}^{long,opp}$(Eq.\ref{eq:d_long_opp}) and $d_{min}^{lat}$(Eq.\ref{eq:d_lat})\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Provides how to calculate the quantified risky distances;\\ a basis of many assessment methods.\end{tabular} \\ \hline
PR&
  \begin{tabular}[c]{@{}l@{}}An action to recover when\\ $d_{min}^{long},d_{min}^{lat}$ and the safe range of $a^{lat}$,$a^{long}$ are violated\end{tabular} &
  Adds more information beyond MSDV. \\ \hline
MSDF &
  \begin{tabular}[c]{@{}l@{}}$MSDF^{lat} = \frac{d^{lat}}{d^{lat}_{min}}$\\ $MSDF^{long} = \frac{d^{long}}{d^{long}_{min}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Can indicate the degree of defensive driving style;\\ a higher $MSDF$ may not means higher safety.\end{tabular} \\ \hline
MSDCE &
  $MSDCE = \sqrt{\frac{\vert d^{long}_{gt,min} - d^{long}_{min}\vert }{d^{long}_{gt,min}}+\frac{\vert d^{lat}_{gt,min} - d^{lat}_{min}\vert }{d^{lat}_{gt,min}}}$ &
  Indicate the ADS ability to determine the safety distances. \\ \hline
CI &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle is involved in a collision.\\ Active when $d^{lat}$ and $d^{long}$ are equal to 0.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Capture instances of collisions as a metric;\\ the severity of the collision can be defined by KABCO scale\cite{herbel2010highway}:\\
  K(Fatal Injury), A(Incapacitating Injury), B (Non-Incapacitating Injury),\\ C(Possible Injury), O(No Injury).\end{tabular} \\ \hline
TLV &
  Indicate the subject vehicle that violates a traffic law &
  \begin{tabular}[c]{@{}l@{}}Emphasizes that an ADS vehicle must follow existing laws;\\ exceptions are made, for example, when road closures \\ require temporary violations of driving exclusively inside a traffic lane.\end{tabular} \\ \hline
ABC &
  Indicate the subject vehicle can execute a specific behavior correctly. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics.\end{tabular} \\ \hline
ADSA &
  Indicate the ADS is active when executing behaviors. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics;has some dispute in California\cite{hawkins2019california}.\end{tabular} \\ \hline
HTCDER &
  $HTCDER = \frac{GTI-CDI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
HTCVR &
  $HTCVR = \frac{CDI-CCI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
  
AD &
  \begin{tabular}[c]{@{}l@{}}Indicate the maneuvers (longitudinal/lateral accelerations) \\ of a subject vehicle exceeds specified thresholds.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The thresholds vary by jurisdiction and culture;\\ AD is only involved the subject vehicle;\\ implies the inherent and potential risks of natural driving behaviors;\\ should be included when evaluating ADS.\end{tabular} \\ \hline  
  
\end{tabular}}
\caption{Summary of operational safety metrics along with their key properties. Noting that '*' denotes the metrics that are not selected by IAM but are basic metrics employed in other papers.}  
\label{tab:metrics}
\end{table*}
































The works accentuating micro network often refer to vehicle behavior prediction or trajectory prediction. These tasks essentially deduce the future target vehicle(s) by learning the representation of the current and previous observed states of surrounding vehicles and even the involved environment\cite{mozaffari2020deep}. Recurrent Neural Networks (RNNs) are known as solid tools to master time sequence data. Since the drawback of conventional RNNs is that gradient vanishing or exploding, many works\cite{zyner2018recurrent,zyner2017long,xin2018intention,park2018sequence,deo2018multi,dai2019modeling} exploit Long Short-Term Memory(LTSM) and Gated Recurrent Unit (GRU), which are the upgraded versions of RNN. Because CNN is outstanding on processing spatial dependencies, additional works\cite{lee2017convolution,cui2019multimodal,djuric2020uncertainty} involve CNN in their framework. Further works deploy 3D CNN\cite{luo2018fast,dwivedi2020ssp}  or combination CNN with LSTM\cite{yang2020traffic,liu2020smart,zhao2019multi,messaoud2019non,messaoud2020multi} to their works, which introduced one more dimension to process time-series data. Particularly, \cite{messaoud2019non,messaoud2020multi} applied social pooling to LSTM autoencoder and captured the interaction, and assigned the importance of the target vehicle learned by attention mechanism. 


Similar to the works focusing on marco networks, authors in \cite{li2019grip,li2019grip++,diehl2019graph,diao2019dynamic} deploy GNN to represent atypical distance among vehicles. Especially, \cite{li2019grip,li2019grip++} represent the close agents via graphs and deploy multiple Graph Convolutional Layers to extract spatial dependencies and then use GRU Encoder-Decoder structure to produce the prediction. Since the above model-based or supervised learning performs weakly on interpretability, recent papers \cite{wulfmeier2017large,zhang2018integrating,you2019advanced,huang2021driving} tend to model the driving behavior using Inverse Reinforcement Learning (IRL) which can address the shortcoming by recovering the underlying human logic as reward functions. Moreover, a potential advantage of frameworks\cite{wulfmeier2017large,zhang2018integrating,fernando2020deep} with IRL can better understand the influence from context environment. 
Nevertheless, we may not neglect some works also explore the environmental factor by using various methods. For example, \cite{tang2019multiple,messaoud2020multi} proposed attention-based architecture that can model both the interaction between agents and the influence of the static scene structure. \cite{amirloo2021self} proposed a self-supervised framework that can estimate the cost of dynamical environments.  A more recent work \cite{casas2021mp3} proposed a unified model that can learn the online High-Definition maps (HD maps) and subsequently learn the probabilistic representation of multi-agents.


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}\toprule 
 &
  \multicolumn{2}{c}{CTTC} &
  \multicolumn{2}{c}{IVVR} &
  \multicolumn{2}{c}{OVVR} &
  \multicolumn{2}{c}{OSR} &
  \multicolumn{2}{c}{TCI} &
  \multicolumn{2}{c}{NTC} \\
 &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} &
  P-value &
  \begin{tabular}[c]{@{}c@{}}Slope   \\      Direction\end{tabular} \\ \midrule
Seg   1 All &
  4.38E-03 &
  + &
  3.75E-08 &
  + &
  6.02E-09 &
  + &
  2.28E-09 &
  - &
  6.61E-07 &
  - &
  6.15E-05 &
  + \\
Seg   1 Rear-end &
  7.46E-03 &
  + &
  8.57E-08 &
  + &
  1.52E-08 &
  + &
  3.31E-10 &
  - &
  1.49E-07 &
  - &
  1.38E-04 &
  + \\
Seg   1 Sideswipe &
  2.13E-03 &
  + &
  1.02E-06 &
  + &
  1.27E-06 &
  + &
  6.11E-02 &
  + &
  1.55E-01 &
  - &
  8.40E-06 &
  + \\
Seg   2 All &
  1.17E-02 &
  + &
  2.42E-02 &
  + &
  1.36E-02 &
  + &
  3.49E-01 &
  - &
  4.30E-04 &
  - &
  8.35E-02 &
  + \\
Seg   2 Rear-end &
  1.62E-02 &
  + &
  3.25E-02 &
  + &
  1.64E-02 &
  + &
  3.12E-01 &
  - &
  2.40E-04 &
  - &
  8.96E-02 &
  + \\
Seg   2 Sideswipe &
  4.88E-03 &
  + &
  8.10E-03 &
  + &
  2.32E-02 &
  + &
  6.42E-01 &
  - &
  9.31E-03 &
  - &
  1.13E-01 &
  + \\
Combined   All &
  3.93E-03 &
  + &
  8.06E-04 &
  + &
  2.98E-06 &
  + &
  1.46E-03 &
  - &
  4.21E-08 &
  - &
  1.69E-03 &
  + \\
Combined   Rear-end &
  3.34E-03 &
  + &
  1.80E-03 &
  + &
  7.17E-06 &
  + &
  6.19E-04 &
  - &
  1.34E-08 &
  - &
  3.13E-03 &
  + \\
Combined   Sideswipe &
  9.49E-01 &
  - &
  1.95E-06 &
  + &
  1.77E-07 &
  + &
  2.86E-01 &
  + &
  4.49E-04 &
  - &
  4.63E-06 &
  +\\ \bottomrule
\end{tabular}%
}
\caption{The F-test results of one-predictor models $y_i = \beta_1 x_i + \beta_0$, where $ x_i$ is one of the proposed metrics.The slope indicates the linear relationship between metrics and crashes. For a better generalization, the model for the same type of crash and different segments should have the same direction. }
\label{tab:one-predictor}
\end{table*}
















\section{Geometry Contribution}\label{sec:geo_method}
Road geometry is another significant factor that modulates the crash rate. Indeed, there is a rich set of literature studying this concept, as reviewed in Section \ref{sec:net_analysis}. However, exploiting the detailed geometry contributors (e.g., road grade \ar{what do you mean by grade, do you mean the quality of pavement?}, curvature, number of lanes, geo-distribution of intersections, etc.) is out of our scope. 
\arr{Xiwen: It seems what you are trying to show here is that the road geometry is relevant and modulates the crash rate, but what I wanted to show was the opposite, I wanted to show that the relevance we found between the crash rate and the safety metrics is generalizeable to different roads, which means that they are not just random findings but more general and universal relations!!! Anyway, lets see what you find here!!!} 
Therefore, we just anticipate checking limited factors to demonstrate the road geometry definitely affect the occurrence of collisions by introducing Chi-Squared hypothesis test of independence. The hypothesises are:
    \begin{align}
        H_0:&  ~\text{Crashes Type}~\alpha~\text{is not dependent on Factor}~G_i, \\ \nonumber
        H_a:&  ~\text{Crashes Type}~\alpha~\text{is dependent on  Factor}~G_i,
    \end{align}
    where, $\alpha\in\{\text{All},\text{Rear-end},\text{Sideswipe}\}$
     Then we can build a $r\times c$ tables, in which, each row denotes the different state of the selected factor and each column denotes the different state of the crashes. e.g. cell $\{i,j\}$ represents the observed crashes in time $i$ with geometry condition in state $j$. 
     The Chi-squared statistic $\chi^{2*}$ can be computed by:
     \begin{align}
         E_{i,j}&=\frac{\sum_{k=1}^c O_{i,k}\sum_{k=1}^r O_{k,j}}{rc}, \\ \nonumber
         \chi^{2*}&=\sum_{i=1}^c \sum_{j=1}^r (O_{i,j}-E_{i,j})^2 \sim \chi^2_{(r-1)(c-1)},
     \end{align}
     where, $ E_{i,j}$ and $O_{i,j}$ denote the expected value and observed value of cell $\{i,j\}$, respectively. $\chi^2_{(r-1)(c-1)}$ denotes that the calculated Chi-squared statistic $\chi^{2*}$ obeys $\chi^2$ distribution with $(r-1)(c-1)$ degrees of freedom. 
\begin{comment}
    


Additionally, we will also evaluate the dependence among metrics and the geometry factor, and the  hypothesises become: 
 \begin{align}
        H_0:&  ~\text{Metrics}~m~\text{is not dependent on  Factor}~G_i, \\ \nonumber
        H_a:&  ~\text{Metrics}~m~\text{is dependent on  Factor}~G_i.
    \end{align}
 \end{comment}








\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
 \toprule 
               \textbf{Type}               & All    & Rear-end & Sideswipe \\   \midrule
              \textbf{P-value} & 2.12E-7 &1.38E-9 & 0.451    \\  \bottomrule 
\end{tabular}
\caption{Contribution by road ID or merge condition for the current case. Segment 1 does not have merge lanes, while Segment 2 has merge lanes. }
\label{tab:contribute_id}
\end{table}


As we mentioned in Section \ref{sec:geo_method}, the chi-squared test is used to derive the geometry factors which are associated with crashes. Recap the null hypothesis is that the selected factor is independent of crashes. We set the significance level as 0.05, meaning that if the obtained P-value is less than 0.05, we reject the null hypothesis and believe that they are correlated. Here, we simply represent the factor by the ID of these segments, since in fact, at least, the environment of them should have diversity. 
The result is shown in Table \ref{tab:contribute_id}, which indicates according to this sample data, the difference of geometry should relate to the all type or rear-end crashes, but interestingly, sideswipe crashes seem not sensitive to the environment. We have to admit that this taxonomy is very rough, but also concludes one apparent geometry feature: i) No merge Lanes, ii) have merge lanes. A more conclusive taxonomy would be helpful for future in-depth analysis. Like we discuss earlier, these results  cannot show how the different factors affect the crashes.
Table \ref{tab:contribute_id} can provide some evidence in the above association analysis that metrics should integrate with road geometry information to better interpret the crashes.





\section{excluded parts from the results section}
\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/p_rear.jpg}}
\caption{The magnitude of the P-value tested for rear-end crashes. Each model in the test has only one predictor.}
\label{fig:p_value_rear}
\end{center}
\end{figure}

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/p_side.jpg}}
\caption{The magnitude of the P-value tested for sideswipe crashes.Each model in the test has only one predictor.}
\label{fig:p_value_sideswipe}
\end{center}
\end{figure}




\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}\toprule 
 \multicolumn{1}{c}{} & \multicolumn{2}{c}{\arr{TTC-CV}}                                                      & \multicolumn{2}{c}{IVVR}                                                          & \multicolumn{2}{c}{OVVR}                                                          & \multicolumn{2}{c}{OSR}                                                           & \multicolumn{2}{c}{TCI}                                                           & \multicolumn{2}{c}{NTC}                                                           \\
\multicolumn{1}{c}{} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\ Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Correlation\\      Coefficient\end{tabular} \\ \midrule
Seg 1 All            & 4.38E-03 & +0.3629                                                           & 3.75E-08 & +0.6397                                                                & 6.02E-09 & +0.6668                                                                & 2.28E-09 & -0.6801                                                                & 6.61E-07 & -0.5911                                                                & 6.15E-05 & +0.4935                                                                \\
Seg 1 Rear-end       & 7.46E-03 & +0.3421                                                           & 8.57E-08 & +0.6265                                                                & 1.52E-08 & +0.6534                                                                & 3.31E-10 & -0.7047                                                                & 1.49E-07 & -0.6173                                                                & 1.38E-04 & +0.4726                                                                \\
Seg 1 Sideswipe      & 2.13E-03 & +0.3890                                                           & 1.02E-06 & +0.5830                                                                & 1.27E-06 & +0.5787                                                                & 6.11E-02 & +0.2432                                                                & 1.55E-01 & -0.1857                                                                & 8.40E-06 & +0.5402                                                                \\
Seg 2 All            & 1.17E-02 & +0.4401                                                           & 2.42E-02 & +0.3977                                                                & 1.36E-02 & +0.4317                                                                & 3.49E-01 & -0.1710                                                                & 4.30E-04 & -0.5856                                                                & 8.35E-02 & +0.3107                                                                \\
Seg 2 Rear-end       & 1.62E-02 & +0.4218                                                           & 3.25E-02 & +0.3789                                                                & 1.64E-02 & +0.4212                                                                & 3.12E-01 & -0.1845                                                                & 2.40E-04 & -0.6056                                                                & 8.96E-02 & +0.3051                                                                \\
Seg 2 Sideswipe      & 4.88E-03 & +0.4852                                                           & 8.10E-03 & +0.4599                                                                & 2.32E-02 & +0.4002                                                                & 6.42E-01 & -0.0853                                                                & 9.31E-03 & -0.4525                                                                & 1.13E-01 & +0.2859                                                                \\
Combined All         & 3.93E-03 & +0.2979                                                           & 8.06E-04 & +0.3434                                                                & 2.98E-06 & +0.4652                                                                & 1.46E-03 & -0.3270                                                                & 4.21E-08 & -0.5340                                                                & 1.69E-03 & +0.3230                                                                \\
Combined Rear-end    & 3.34E-03 & +0.3028                                                           & 1.80E-03 & +0.3212                                                                & 7.17E-06 & +0.4489                                                                & 6.19E-04 & -0.3503                                                                & 1.34E-08 & -0.5502                                                                & 3.13E-03 & +0.3049                                                                \\
Combined Sideswipe   & 9.49E-01 & -0.0068                                                           & 1.95E-06 & +0.4728                                                                & 1.77E-07 & +0.5124                                                                & 2.86E-01 & +0.1124                                                                & 4.49E-04 & -0.3586                                                                & 4.63E-06 & +0.4571   \\ \bottomrule                                                            
 
 
 
\end{tabular}%
}
\caption{The F-test results of one-predictor models $y_i = \beta_1 x_i + \beta_0$, where $ x_i$ is one of the proposed metrics.The slope indicates the linear relationship between metrics and crashes. For a better generalization, the model for the same type of crash and different segments should have the same direction. \xc{update Pearson correlation coefficient } \arr{remove combined and keep a copy}}
\label{tab:one-predictor}
\end{table*}

\begin{table*}[]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{lcccccccccc}\toprule 
                 & \multicolumn{6}{c}{t-Test   P-value}                            & \multicolumn{4}{c}{Model   Criterion}              \\
                  & CTTC     & IVVR     & OVVR     & OSR      & TCI      & NTC      & F   P-value & R-squared & Adj.   R-squared & ACI   \\ \midrule
Seg   1 All       & 2.09E-01 & 1.35E-02 & 1.51E-01 & 2.70E-04 & 2.86E-01 & 4.05E-01 & 2.65E-16    & 0.7902    & 0.7665           & 564.0 \\
Seg   1 Rear-end  & 3.39E-01 & 1.03E-02 & 1.80E-01 & 8.98E-05 & 2.44E-01 & 4.24E-01 & 7.40E-17    & 0.8003    & 0.7777           & 553.6 \\
Seg   1 Sideswipe & 7.16E-02 & 2.04E-01 & 3.74E-01 & 7.08E-01 & 8.63E-01 & 3.75E-01 & 1.33E-05    & 0.4465    & 0.3839           & 324.5 \\
Seg   2 All       & 4.04E-02 & 7.97E-05 & 1.90E-04 & 7.05E-01 & 7.11E-08 & 2.09E-01 & 8.59E-11    & 0.8896    & 0.8631           & 298.3 \\
Seg   2 Rear-end  & 6.87E-02 & 1.15E-04 & 1.26E-04 & 8.35E-01 & 3.02E-08 & 1.77E-01 & 6.96E-11    & 0.8915    & 0.8654           & 290.8 \\
Seg   2 Sideswipe & 4.46E-02 & 1.17E-03 & 5.14E-02 & 5.27E-01 & 9.81E-04 & 5.46E-01 & 1.88E-06    & 0.7482    & 0.6878           & 178.7 \\
% Combined   All    &2.01E-03 & 4.73E-06 & 4.91E-07 & 6.26E-03 & 2.32E-15 & 8.58E-01 & 8.02E-26 & 0.7791 & 0.7635 & 877.3 \\
% Combined   Rear-end  & 3.34E-03 & 6.09E-06 & 4.80E-07 & 2.10E-03 & 5.65E-16 & 8.78E-01 & 1.94E-26 & 0.7864 & 0.7714 & 859.5 \\
% Combined   Sideswipe & 4.49E-02 & 3.29E-03 & 4.89E-03 & 2.94E-01 & 1.95E-06 & 9.78E-01 & 5.82E-11 & 0.4956 & 0.4600 & 516.6 \\ 
\bottomrule 
\end{tabular}
}
\caption{The overall analysis. The model considers all metrics as the independent variables. True that in each segment, all types of crashes and rear-end crashes can be explained well by the proposed models; however, some independent variables are not active in the models (t-test p-value greater than 0.05). \arr{remove individual feature contributions and the combined segments here, but a keep a copy of it for future use.}}
\label{tab:ols_analysis_1}
\end{table*}











\section{results}

% \begin{figure}[]
% \begin{center}
% \centerline{\includegraphics[width=0.8\columnwidth]{figures/gt_vs_estimate_full.png}}
% \caption{The scatter plot of the ground truth and the estimated value of the crash count by the full model in different segments. Each data point represents a 10-min interval.\xc{Plan to update. See Fig. \ref{fig:fitted_new}}}
% \label{fig:fitted}
% \end{center}
% \end{figure}




% \begin{figure}[]
% \begin{center}
% \centerline{\includegraphics[width=1\columnwidth]{figures/P_all_new.jpg}}
% \caption{The illustration of P-values obtained for different metrics in association with all-types crashes using one-predictor models. The magnitude is shown as $-\log_{10}(P)$ for visualization convenience, so the higher bars represent more significance.\xc{Plan to removed}}
% \label{fig:p_value_all}
% \end{center}
% \end{figure}




%\begin{figure}[]
%\begin{center}
%\centerline{\includegraphics[width=1\columnwidth]{figures/magnitude.png}}
%\caption{The significance of the P-value in terms of its magnitude computed by $-\log_{10}(P)$.\xc{update}}
%\label{fig:magnitude}
%\end{center}
%\end{figure}


% \begin{figure}[]
% \begin{center}
% \centerline{\includegraphics[width=1\columnwidth]{figures/coeff_new.png}}
% \caption{The significance of the Pearson correlation coefficient between different safety metrics and crash types across two segments.\xc{Plan to update}}
% \label{fig:coeff}
% \end{center}
% \end{figure}







% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccc}\toprule 
%  \multicolumn{1}{c}{} & \multicolumn{2}{c}{TTC-CV}                                                      & \multicolumn{2}{c}{IVVR}                                                          & \multicolumn{2}{c}{OVVR}                                                          & \multicolumn{2}{c}{OSR}                                                           & \multicolumn{2}{c}{TCI}                                                           & \multicolumn{2}{c}{NTC}                                                           \\
% \multicolumn{1}{c}{} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\ Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\      Coefficient\end{tabular} & P-value  & \begin{tabular}[c]{@{}c@{}}Pearson\\      Coefficient\end{tabular} \\ \midrule
% Seg 1 All            & 4.38E-03 & +0.3629                                                           & 3.75E-08 & +0.6397                                                                & 6.02E-09 & +0.6668                                                                & 2.28E-09 & -0.6801                                                                & 6.61E-07 & -0.5911                                                                & 6.15E-05 & +0.4935                                                                \\
% Seg 1 Rear-end       & 7.46E-03 & +0.3421                                                           & 8.57E-08 & +0.6265                                                                & 1.52E-08 & +0.6534                                                                & 3.31E-10 & -0.7047                                                                & 1.49E-07 & -0.6173                                                                & 1.38E-04 & +0.4726                                                                \\
% Seg 1 Sideswipe      & 2.13E-03 & +0.3890                                                           & 1.02E-06 & +0.5830                                                                & 1.27E-06 & +0.5787                                                                & 6.11E-02 & +0.2432                                                                & 1.55E-01 & -0.1857                                                                & 8.40E-06 & +0.5402                                                                \\
% Seg 2 All            & 1.17E-02 & +0.4401                                                           & 2.42E-02 & +0.3977                                                                & 1.36E-02 & +0.4317                                                                & 3.49E-01 & -0.1710                                                                & 4.30E-04 & -0.5856                                                                & 8.35E-02 & +0.3107                                                                \\
% Seg 2 Rear-end       & 1.62E-02 & +0.4218                                                           & 3.25E-02 & +0.3789                                                                & 1.64E-02 & +0.4212                                                                & 3.12E-01 & -0.1845                                                                & 2.40E-04 & -0.6056                                                                & 8.96E-02 & +0.3051                                                                \\
% Seg 2 Sideswipe      & 4.88E-03 & +0.4852                                                           & 8.10E-03 & +0.4599                                                                & 2.32E-02 & +0.4002                                                                & 6.42E-01 & -0.0853                                                                & 9.31E-03 & -0.4525                                                                & 1.13E-01 & +0.2859                                                                \\
% % Combined All         & 3.93E-03 & +0.2979                                                           & 8.06E-04 & +0.3434                                                                & 2.98E-06 & +0.4652                                                                & 1.46E-03 & -0.3270                                                                & 4.21E-08 & -0.5340                                                                & 1.69E-03 & +0.3230                                                                \\
% % Combined Rear-end    & 3.34E-03 & +0.3028                                                           & 1.80E-03 & +0.3212                                                                & 7.17E-06 & +0.4489                                                                & 6.19E-04 & -0.3503                                                                & 1.34E-08 & -0.5502                                                                & 3.13E-03 & +0.3049                                                                \\
% % Combined Sideswipe   & 9.49E-01 & -0.0068                                                           & 1.95E-06 & +0.4728                                                                & 1.77E-07 & +0.5124                                                                & 2.86E-01 & +0.1124                                                                & 4.49E-04 & -0.3586                                                                & 4.63E-06 & +0.4571   \\ 
% \bottomrule                                                            
 
 
 
% \end{tabular}%
% }
% \caption{F-test results for one-predictor models $y_i = \beta_1 x_i + \beta_0$, where $ x_i$ is one of the proposed metrics. The slope (also as the Pearson Coefficient) indicates the linear relationship between the metric and crash. For a better generalization, the model for the same type of crash and different segments should have the same direction.\xc{See new table \ref{tab:coeff_individual}}}
% \label{tab:one-predictor}
% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}





% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \caption{The Pearson correlation, Spearman's correlation, and Kendall correlation for the metrics across all segments.}
% \label{tab:coeff_individual}
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{clrrrrrrrr} \toprule
% \multicolumn{1}{l}{}        &           & \multicolumn{1}{l}{IVVR} & \multicolumn{1}{l}{OVVR} & \multicolumn{1}{l}{OSR} & \multicolumn{1}{l}{OSR+} & \multicolumn{1}{l}{OSR++} & \multicolumn{1}{l}{TCI} & \multicolumn{1}{l}{NTC} & \multicolumn{1}{l}{TTC} \\ \midrule
% \multirow{3}{*}{Pearson}    & All Type  & 0.308                    & 0.531                    & -0.559                  & -0.583                   & -0.565                    & -0.328                  & 0.469                   & 0.308                   \\
%                             & Rear-end  & 0.305                    & 0.521                    & -0.553                  & -0.580                   & -0.567                    & -0.315                  & 0.462                   & 0.310                   \\
%                             & Sideswipe & 0.213                    & 0.335                    & -0.314                  & -0.300                   & -0.266                    & -0.228                  & 0.270                   & 0.090                   \\ \midrule
% \multirow{3}{*}{Spearman's} & All Type  & 0.330                    & 0.377                    & -0.390                  & -0.387                   & -0.374                    & -0.246                  & 0.363                   & 0.273                   \\
%                             & Rear-end  & 0.305                    & 0.358                    & -0.386                  & -0.384                   & -0.379                    & -0.235                  & 0.354                   & 0.265                   \\
%                             & Sideswipe & 0.255                    & 0.267                    & -0.212                  & -0.205                   & -0.197                    & -0.165                  & 0.188                   & 0.091                   \\ \midrule
% \multirow{3}{*}{Kendall}    & All Type  & 0.453                    & 0.536                    & -0.538                  & -0.536                   & -0.532                    & -0.329                  & 0.512                   & 0.384                   \\
%                             & Rear-end  & 0.429                    & 0.515                    & -0.535                  & -0.532                   & -0.525                    & -0.313                  & 0.503                   & 0.373                   \\
%                             & Sideswipe & 0.330                    & 0.350                    & -0.283                  & -0.275                   & -0.264                    & -0.223                  & 0.247                   & 0.104  \\ \bottomrule                 
% \end{tabular}%
% }
% \end{table*}


%We build the models from both ends to the middle. Specifically, we build one-predictor models and the full model simultaneously. One-predictor model can be written as $y_i = \beta_1 x_i +\beta_0$, where $x_i$ is one of the proposed metrics and $y_i$ is the observed crash. The full models consider all metrics as their predictors. Then, we search enough good collective metrics and restrict the models for each type of crash based on the results offer from one-predictor models and the full models. The selected models should have a good generation in different segments With acceptable performance. Noting that the results of one-predictor models can offer the order to select the metrics, while the full model can provide the approximate optimal linear model performance.  









% The immediate observation is that the Pearson correlation slope sign for most metrics (except OSR) are consistent. For example, the positive slope of IVVR and OVVR shows that higher individual and overall speed variations results in a higher crash rates across the two segments. The same trend holds for TTC-CV meaning that the higher variations of TTC-CV indicate a higher chance of a crash. The negative slope of TCI indicates that the more diverse is the vehicle types (lower TCI) the most likely are crashes. The p-values of the F-test also are above 5\% for most scenarios conforming the importance of the introduced safety metrics in crash risk assessment.  



% We also visualize the magnitude of the t-test P-value for one-predictor models in Fig. \ref{fig:p_value_all}. The p-values are considerably lower than the significance level of 0.05, shown by a red dashed line.  
% Fig. \ref{fig:coeff} summarizes the relations between different safety metrics and crash types in terms of Pearson correlation. The correlation is higher than 50\% for most pairs (safety metric-crash type). However, one metric may not be sufficient for a reasonable prediction, as expected. 

%Therefore, we next step is searching the accepted models by restricting some estimators. We have multiple references to restricting the models, such as R-square, adjusted R-square, etc., and sometimes they may conflict. For example, the full model "Combined All" has a better adjusted R-square score but a worst AIC score than the full model "Combined Sideswipe". 
%Thus, the strategy to search the metrics is based on the results of one-predictor models in Table \ref{tab:one-predictor}, and guarantee the reduced models for each segment can achieve acceptable performance with enough generalization. 
%Noting that when processing the models, we also need to consider the collinearity or correlation among metrics (shown in able []). It indicates OVVR and IVVR have relatively high collinearity, meaning that we do not expect these two metrics exist in the same model simultaneously. 




%\ref{tab:one-predictor} and Table \ref{tab:ols_analysis_1}. The results of one-predictors models give us some evidence of generalization that the slope directions are uniform for most of metrics (except OSR). We also visualize the magnitude of the t-test P-value for one-predictor models for different crash types in Fig \ref{fig:p_value_all}, Fig \ref{fig:p_value_rear}, and Fig \ref{fig:p_value_sideswipe}, and the significant level 0.05 is marked as a red dash line.  The calculated statistical data in Table \ref{tab:ols_analysis_1} shows that although the full models have adequate scores (~80 R-squared scores in All type and Rear-end); however, there are specific metrics suitable for a specific model, which is undesirable. For example, true that the models  Seg. 1 Rear-end, Seg. 2 Rear-end, Combined Rear-end all obtained a small F-test P-value ($7.4E-14$, $6.96E-11$, and $5.82E-11$, respectively) and are significant; however, they have different reliable estimators (IVVR and OSR for Seg. 1 Rear-end, CTTC, IVVR, OVVR and TCI for Seg. 2 Rear-end, and CTTC, IVVR, OVVR, OSR, and TCI for Combined Rear-end). These facts result in the models are low generalization for different scenarios, which is not unsatisfactory. Therefore, we next step is searching the accepted models by restricting some estimators. We have multiple references to restricting the models, such as R-square, adjusted R-square, etc., and sometimes they may conflict. For example, the full model "Combined All" has a better adjusted R-square score but a worst AIC score than the full model "Combined Sideswipe". Thus, the strategy to search the metrics is based on the results of one-predictor models in Table \ref{tab:one-predictor}, and guarantee the reduced models for each segment can achieve acceptable performance with enough generalization.  Nothing that when processing the models, we also need consider the collinearity or correlation among metrics (shown in able []). It indicates OVVR and IVVR have relatively high collinearity, meaning that we do not expect these two metrics exist in the same model simultaneously. 

























% \caption{The overall analysis. The model considers all metrics as the independent variables.}
%\label{tab:ols_analysis_1}

% \begin{table*}[htbp]
% \centering\resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lrrrrrrr} \toprule
%              & \multicolumn{3}{c}{t-Test P-value}                                            & \multicolumn{4}{c}{Model Criterion}                                                                                          \\
%              & \multicolumn{1}{c}{TTC-CV} & \multicolumn{1}{c}{OVVR} & \multicolumn{1}{c}{TCI} & \multicolumn{1}{c}{F P-value} & \multicolumn{1}{c}{R-squared} & \multicolumn{1}{c}{Adj. R-squared} & \multicolumn{1}{c}{ACI} \\ \midrule
% Seg 1 All    & 4.16E-03                 & 2.62E-09                 & 2.69E-08                & 3.93E-15                      & 0.7115                        & 0.6961                             & 577.1                   \\
% Seg 2 All    & 5.18E-03                 & 2.18E-06                 & 8.11E-09                & 1.24E-09                      & 0.7903                        & 0.7678                             & 312.9                   \\
% Combined All & 5.30E-12
%                 & 1.15E-14
%                  & 8.18E-17              & 1.44E-23                      & 0.7099                        & 0.7                             & 896.4 \\  \bottomrule                
% \end{tabular}}
% \caption{The first accepted restricted model "$TTC\text{-}CV+OVVR+TCI$" for all type crashes analysis.\xc{Plan to removed}  }
% \label{tab:my-ols_analysis_all}
% \end{table*}




% \begin{table*}[htbp]
% \centering\resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lccccccc} \toprule
%              & \multicolumn{3}{c}{t-Test P-value}                                            & \multicolumn{3}{c}{Model Criterion}                                                                & \multicolumn{1}{l}{}    \\
%              & \multicolumn{1}{c}{TTC-CV} & \multicolumn{1}{c}{IVVR} & \multicolumn{1}{c}{TCI} & \multicolumn{1}{c}{F P-value} & \multicolumn{1}{c}{R-squared} & \multicolumn{1}{c}{Adj. R-squared} & \multicolumn{1}{c}{ACI} \\ \midrule
% Seg 1 All    & 6.24E-03                 & 6.55E-09                 & 9.03E-09                & 9.59E-15                      & 0.7021                        & 0.6862                             & 579.1                   \\
% Seg 2 All    & 9.75E-03                 & 8.24E-05                 & 1.76E-07                & 4.04E-08                      & 0.7303                        & 0.7014                             & 320.9                   \\
% Combined All & 1.28E-01                 & 1.32E-08                 & 2.82E-06                & 9.12E-10                      & 0.3989                        & 0.3784                             & 526.7   \\ \bottomrule               
% \end{tabular}}
% \caption{The second accepted restricted model "$TTC\text{-}CV+IVVR+TCI$" for all type crashes analysis.\xc{Plan to removed}  }
% \label{tab:my-ols_analysis_all_2}
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lcccccc}\toprule
%                   & \multicolumn{2}{l}{t-Test P-value} & \multicolumn{4}{c}{Model Criterion}            \\ 
%                   & OVVR             & TCI             & F P-value & R-squared & Adj. R-squared & ACI   \\ \midrule
% Seg 1 Rear-end    & 8.65E-10         & 8.62E-08        & 2.79E-14  & 0.6655    & 0.6538         & 584.0 \\
% Seg 2 Rear-end    & 7.48E-07         & 3.18E-08        & 8.97E-09  & 0.7214    & 0.7022         & 319.9 \\
% Combined Rear-end & 1.79E-08         & 2.76E-10        & 3.89E-14  & 0.5004    & 0.4891         & 944.4 \\ \bottomrule
% \end{tabular}
% }
% \caption{The third accepted restricted model "$OVVR+TCI$" for all type crashes analysis. \xc{Plan to removed} }
% \label{tab:my-ols_analysis_all_3}
% \end{table*}


% \begin{table*}[htbp]
% \centering\resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lrrrrrrr} \toprule
%                   & \multicolumn{3}{c}{t-Test P-value}                                            & \multicolumn{3}{c}{Model Criterion}                                                                & \multicolumn{1}{l}{}    \\
%                   & \multicolumn{1}{c}{TTC-CV} & \multicolumn{1}{c}{OVVR} & \multicolumn{1}{c}{TCI} & \multicolumn{1}{c}{F P-value} & \multicolumn{1}{c}{R-squared} & \multicolumn{1}{c}{Adj. R-squared} & \multicolumn{1}{c}{ACI} \\ \midrule
                  
% Seg 1 Rear-end    & 8.35E-03                 & 4.98E-09                 & 4.83E-09                & 2.96E-15                      & 0.7145                        & 0.6992                             & 569.0                   \\
% Seg 2 Rear-end    & 7.49E-03                 & 1.56E-06                 & 3.09E-09                & 7.04E-10                      & 0.7986                        & 0.7770                             & 304.6                   \\
% Combined Rear-end & 2.24E-12                 & 2.40E-14                 & 1.12E-17                & 4.89E-24                      & 0.7169                        & 0.7073                             & 879.4  \\ \bottomrule
% \end{tabular}}
% \caption{The first accepted restricted model "$TTC\text{-}CV+OVVR+TCI$" for Rear-end crashes analysis.\xc{Plan to removed} }
% \label{tab:my-ols_analysis_rear_end}
% \end{table*}


% \begin{table*}[htbp]
% \centering\centering\resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lrrrrrrr} \toprule
%                   & \multicolumn{3}{c}{t-Test P-value}                                            & \multicolumn{3}{c}{Model Criterion}                                                                & \multicolumn{1}{l}{}    \\
%                   & \multicolumn{1}{c}{TTC\text{-}CV} & \multicolumn{1}{c}{IVVR} & \multicolumn{1}{c}{TCI} & \multicolumn{1}{c}{F P-value} & \multicolumn{1}{c}{R-squared} & \multicolumn{1}{c}{Adj. R-squared} & \multicolumn{1}{c}{ACI} \\ \midrule
% Seg 1 Rear-end    & 1.19E-02                 & 1.02E-08                 & 1.56E-09                & 5.96E-15                      & 0.7072                        & 0.6915                             & 570.5                   \\
% Seg 2 Rear-end    & 1.40E-02                 & 1.06E-04                 & 1.11E-07                & 4.03E-08                      & 0.7304                        & 0.7015                             & 313.9                   \\
% Combined Rear-end & 4.44E-10                 & 1.15E-09                 & 3.29E-16                & 1.89E-19                      & 0.6397                        & 0.6274                             & 901.6                   \\ \bottomrule
% \end{tabular}}
% \caption{The second accepted restricted model "$TTC\text{-}CV+IVVR+TCI$" for Rear-end crashes analysis. \xc{Plan to removed}}
% \label{tab:my-ols_analysis_rear_end_2}
% \end{table*}



% \begin{table*}[]
% \centering
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{lcccccc} \toprule
%                   & \multicolumn{2}{c}{t-Test P-value}                 & \multicolumn{4}{c}{Model Criterion}                                                                                          \\
%                   & \multicolumn{1}{l}{TTC-CV} & \multicolumn{1}{l}{IVVR} & \multicolumn{1}{l}{F P-value} & \multicolumn{1}{l}{R-squared} & \multicolumn{1}{l}{Adj. R-squared} & \multicolumn{1}{l}{ACI} \\ \midrule
% Seg 1 Sidewipe    & 1.17E-02                 & 5.80E-06                & 2.94E-07                      & 0.4101                        & 0.3894                             & 320.3                   \\
% Seg 2 Sidewipe    & 2.02E-02                 & 3.36E-02                & 2.05E-03                      & 0.3474                        & 0.3024                             & 201.2                   \\
% Combined Sidewipe & 4.93E-01                 & 1.74E-06                & 1.02E-05                      & 0.2276                        & 0.2103                             & 547.8       \\ \bottomrule           
% \end{tabular}%
% }\caption{The first accepted restricted model "$TTC\text{-}CV+IVVR$" for Sideswipe crashes analysis. \xc{Plan to removed}}
% \label{tab:my-ols_analysis_sidewipe}
% \end{table*}





%shorter version: 
% We observed that the crash rate can also be predicted even with a few extracted safety metrics, due to the inherent relation among the developed metrics. Therefore, it is advantageous to remove some of the predictors, especially for smaller datasets (like the utilized 10 hour videos per segment). We use a greedy method by starting from the full-predictor model and eliminating the predictors with lower contribution (higher p-values) as long as the overall predictability increases or remains satisfactory. Likewise, we can start combining one-predictor modes until achieving a desired performance. We call the resulting models as restricted models. The results of this analysis are presented in Tables \ref{tab:my-ols_analysis_all} to \ref{tab:my-ols_analysis_sidewipe}, which show much higher prediction performance can be achieved using fewer hand-picked predictors.   




%We build the models from both ends to the middle. Specifically, we build one-predictor models and the full model simultaneously. One-predictor model can be written as $y_i = \beta_1 x_i +\beta_0$, where $x_i$ is one of the proposed metrics and $y_i$ is the observed crash. The full models consider all metrics as their predictors. Then, we search enough good collective metrics and restrict the models for each type of crash based on the results offer from one-predictor models and the full models. The selected models should have a good generation in different segments With acceptable performance. Noting that the results of one-predictor models can offer the order to select the metrics, while the full model can provide the approximate optimal linear model performance.  

\begin{comment}
Table \ref{tab:my-ols_analysis_all}, \ref{tab:my-ols_analysis_all_2}  and \ref{tab:my-ols_analysis_all_3} illustrate the accepted restricted models for all type crashes. %The models in Table \ref{tab:my-ols_analysis_all_3} reduce CTTC metrics is due to it requires prior knowledge which may introduce bias.


Table \ref{tab:my-ols_analysis_rear_end} and Table \ref{tab:my-ols_analysis_rear_end_2} illustrate the accepted restricted models for rear-end crashes. Table \ref{tab:my-ols_analysis_sidewipe} illustrate the accepted restricted model for sideswipe crashes.%after tuning.
\end{comment}





%In temporal dimension, the results may offer some heuristic phenomena or conclusion: i) OVVR/IVVR may be considered as a fundamental estimator when assessing the crashes related tasks. ii) TCI shows that an unbalanced traffic flow has a greater probability to have crashes. The phenomenon may be distinctive from our common sense. iii) The accepted model for sideswipe crashes performs poorly, which may be caused by the limited number of sideswipe crashes, and we need in-depth analysis. iv) CTTC also is an important factor that can participate in most of the models; however, it may be limited due to the required prior knowledge. In spatial domain, the metrics in models with mixing data often cannot interpret the crashes well. i.e. We observed a metrics-crash pair $/{x_1,y_1 /}$ in segment 1,  and another pair $/{x_2,y_2 /}$, where $x_1>x_2$. $y_1$ and $y_2$ should have the same crash type. The model shows $y_i$ and $x_i$ has positive linear relationship; however, since they are measured in different environment,  $y_1$ may not greater than $y_2$. The distance of the models  in different environment may caused by the road geometry factors.

%\fbox{until here}











\begin{comment}


\begin{table}[]
\centering
\begin{tabular}{llllll} \toprule
\textbf{Metrics}         & IVVR   & OVVR   & OSR    & TCI    & NTC      \\  \midrule
\textbf{P-value} & 0.9999 & 0.9999 & 0.9999 & 0.9999 & 8.98E-21   \\  \bottomrule 
\end{tabular}
\caption{The Chi-squared results of metrics.}
\label{tab:metrics_vs_gemotry}
\end{table}
\end{comment}




==> excluded_statistical_tests.tex <==


\fbox{Years vs hours (good)}
\xc{To reduce the numbers of categories that maintain the robustness of Chi-square test, we split the 24 hour into 3 durations, which means each duration has 8 hours. Now the number of categories are reduced to one-eighth. An example of the observation contingency table is shown in Table \ref{tab: Years vs hour example}. We perform the test 1000 times (i.e. randomly split the durations 1000 times), and the average results are shown in Table \ref{tab:Years vs hours}. }


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The example of the Chi-square test for years vs hours with randomly separated durations}
\label{tab: Years vs hour example}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lrrrrr} \toprule
Year       & 2015 & 2016 & 2017 & 2018 & 2019 \\ \midrule
Duration 1 & 407  & 456  & 431  & 446  & 433  \\
Duration 2 & 380  & 402  & 361  & 373  & 369  \\
Duration 3 & 349  & 435  & 413  & 397  & 380  \\ \bottomrule
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The chi-square test for years vs hours averages the results of 1000 tests.}
\label{tab:Years vs hours}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lrrr} \toprule
         & \multicolumn{1}{l}{All Type} & \multicolumn{1}{l}{Rear-end} & \multicolumn{1}{l}{Sideswipe} \\ \midrule
Statstic & 12.49404                     & 16.72444                     & 9.186534                      \\
P-value  & 0.275962                     & 0.195133                     & 0.41611 \\ \bottomrule                      
\end{tabular}%
}
\end{table}


\fbox{Week day (Sun to Sat) vs Hour  (not good)}
\xc{Similar to the Chi-square test for Years vs hours, the average results of 1000 times test are shown in Table \ref{tab:week vs hours}.}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The chi-square test for Week day vs hours averages the results of 1000 tests.}
\label{tab:week vs hours}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lrrr}\toprule
         & \multicolumn{1}{l}{All Type} & \multicolumn{1}{l}{Rear-end} & \multicolumn{1}{l}{Sideswipe} \\ \midrule
Statstic & 52.8778                      & 51.79143                     & 20.64542                      \\
P-value  & 0.04919                      & 0.026707                     & 0.181162 \\ \bottomrule                    
\end{tabular}%
}
\end{table}

\fbox{Weekday (Mon to Thur) vs Hour(good)}
\xc{Similar to the Chi-square test for Years vs hours, the average results of 1000 times test are shown in Table \ref{tab:weekday vs hours}.}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The chi-square test for years vs hours averages the results of 1000 tests.}
\label{tab:weekday vs hours}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lrrr}\toprule
         & \multicolumn{1}{l}{All Type} & \multicolumn{1}{l}{Rear-end} & \multicolumn{1}{l}{Sideswipe} \\ \midrule
Statstic & 8.604817                     & 10.76176                     & 6.886484                      \\
P-value  & 0.334285                     & 0.228551                     & 0.422137 \\ \bottomrule                    
\end{tabular}%
}
\end{table}




\fbox{Hour Vs Hour}

\xc{To show the meaningful difference among hours, we use \textit{one-way} Chi-square test.
The p-value is very close to zero, which means the null hypothesis that the crashes are normally distributed via hour can be rejected.}



\begin{table}[htbp]
\centering
\caption{One-way Chi-square test for hours }
\label{tab:chi_square_hour}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{llll} \toprule
         & All Type & Rear-end & Sideswipe \\ \midrule
Statstic & 5350.39& 5028.855 & 691.545  \\
P-value  & 0.0& 0.0 & 2.679e-131  \\ \bottomrule
\end{tabular}%
}
\end{table}


\fbox{contingency Chi-square test: Years vs  Type}

\xc{contingency Chi-square test: Years vs  Type. The result is shown in Table \ref{tab:vhi_year_vs_type}.}
\begin{table}[]
\centering
\caption{The contingency Chi-square results for Year (2015-2019) Vs Type (Rear-end/Sideswipe).}
\label{tab:vhi_year_vs_type}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lll} \toprule
     & Statistic & P-value \\\midrule
Year vs type & 5.605     & 0.231   \\ \bottomrule
\end{tabular}%
}
\end{table}

\fbox{contingency Chi-square: week day every year vs  Type}
 \xc{ week day every year vs  Type (e.g. Mondays in 2015/2016/2017/2018/2019 VS type in Rear-end/Sideswipe. Its observation table is shown in Table \ref{tab:day_every_year_vs_type_example}).} The results for the seven days are shown in Table \ref{tab:day_every_year_vs_type}. 



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The observation table for Monday every year Vs Crash Type}
\label{tab:day_every_year_vs_type_example}
\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{lrr} \toprule
                  & \multicolumn{1}{l}{Rearend} & \multicolumn{1}{l}{Sideswipe} \\ \midrule
Mondays   in 2015 & 1.80E+01                    & 1.30E+01                      \\
Mondays   in 2016 & 2.80E+01                    & 1.20E+01                      \\
Mondays   in 2017 & 1.90E+01                    & 1.40E+01                      \\
Mondays   in 2018 & 3.10E+01                    & 1.60E+01                      \\
Mondays   in 2019 & 4.30E+01                    & 1.70E+01  \\ \bottomrule                   
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The results of the Chi-square test for week day every year vs Type.}
\label{tab:day_every_year_vs_type}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr} \toprule
Scenario      & \multicolumn{1}{l}{S} & \multicolumn{1}{l}{M} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{W} & \multicolumn{1}{l}{Y} & \multicolumn{1}{l}{F} & \multicolumn{1}{l}{S} \\ \midrule
statistic & 3.05E+00              & 5.45E+00              & 2.57E+00              & 3.36E+00              & 1.97E+00              & 1.07E+01              & 6.26E+00              \\
P-value   & 5.49E-01              & 2.44E-01              & 6.32E-01              & 5.00E-01              & 7.42E-01              & 2.99E-02              & 1.81E-01 \\ \bottomrule            
\end{tabular}%
}
\end{table}




\fbox{one day vs year (all type) (Friday is not good)}
\xc{An example (shown in Table \ref{tab:one day vs year(all type)_example} ) is all type crashes happened on Sundays in 2015/2016/2017/2018/2019 vs happened this year. We perform such test from Sunday to Monday, and the results are shown in Table \ref{tab:one day vs year(all type)}.}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{An example of the Chi-square for one day (Sunday) vs year}
\label{tab:one day vs year(all type)_example}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{rrr}\toprule 
\multicolumn{1}{l}{Year} & \multicolumn{1}{l}{All   type on Sundays} & \multicolumn{1}{l}{All   type at the year} \\  \midrule
2015                     & 7.90E+01                                  & 1.14E+03                                   \\
2016                     & 1.25E+02                                  & 1.29E+03                                   \\
2017                     & 1.26E+02                                  & 1.21E+03                                   \\
2018                     & 9.70E+01                                  & 1.22E+03                                   \\
2019                     & 1.03E+02                                  & 1.18E+03 \\ \bottomrule                                 
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The results of the Chi-square for one day vs year with all type crashes.}
\label{tab:one day vs year(all type)}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr} \toprule
      Scenario    & \multicolumn{1}{l}{Sun} & \multicolumn{1}{l}{M} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{W} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{F} & \multicolumn{1}{l}{Sat} \\ \midrule
statistic & 3.05E+00                & 5.45E+00              & 2.57E+00              & 3.36E+00              & 1.97E+00              & 1.07E+01              & 6.26E+00                \\
P-value   & 5.49E-01                & 2.44E-01              & 6.32E-01              & 5.00E-01              & 7.42E-01              & 2.99E-02\xc{Not good}              & 1.81E-01               
\end{tabular}%
}
\end{table}


\fbox{one day vs year (Rear-end) (Sun and Sat are not good)}
\xc{An example (shown in Table \ref{tab:tab:one day vs yearRear-end_example} ) is Rear-end crashes happened on Mondays in 2015/2016/2017/2018/2019 vs happened this year. The results are shown in Table \ref{tab:one day vs yearRear-end}.}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{An example of the Chi-square for one day (Sunday) vs year}
\label{tab:tab:one day vs yearRear-end_example}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{rrr}\toprule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{Rear-end on Sundays} & \multicolumn{1}{l}{Rear-end at the year} \\ \midrule
2015                 & 4.20E+01                                  & 8.47E+02                                   \\
2016                 & 8.70E+01                                  & 9.52E+02                                   \\
2017                 & 9.00E+01                                  & 8.84E+02                                   \\
2018                 & 6.40E+01                                  & 8.94E+02                                   \\
2019                 & 6.70E+01                                  & 8.95E+02 \\ \bottomrule                                 
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The results of the Chi-square for one day vs year with rear-end crashes.}
\label{tab:one day vs yearRear-end}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr} \toprule
 Scenario         & \multicolumn{1}{l}{Sun} & \multicolumn{1}{l}{M} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{W} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{F} & \multicolumn{1}{l}{Sat} \\ \midrule
statistic & 1.35E+01                & 7.00E+00              & 2.10E+00              & 4.65E+00              & 4.10E-01              & 1.50E+00              & 1.67E+01                \\
P-value   & 9.13E-03\xc{not good}               & 1.36E-01              & 7.18E-01              & 3.25E-01              & 9.82E-01              & 8.27E-01              & 2.23E-03\xc{not good}    \\ \bottomrule               
\end{tabular}%
}
\end{table}

\fbox{one day vs year (Sideswipe) ( good)}
\xc{Similarly, the results of the Chi-square for one day vs year with sideswipe crashes are shown in Table \ref{tab:one day vs year Sideswipe}.}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The results of the Chi-square for one day vs year with sideswipe crashes.}
\label{tab:one day vs year Sideswipe}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr}
          & \multicolumn{1}{l}{Sun} & \multicolumn{1}{l}{M} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{W} & \multicolumn{1}{l}{T} & \multicolumn{1}{l}{F} & \multicolumn{1}{l}{Sat} \\
statistic & 8.58E-01                & 1.50E+00              & 2.73E+00              & 2.81E+00              & 3.40E+00              & 5.18E+00              & 3.72E+00                \\
P-value   & 9.31E-01                & 8.27E-01              & 6.05E-01              & 5.90E-01              & 4.93E-01              & 2.69E-01              & 4.46E-01               
\end{tabular}%
}
\end{table}






%=======================================
some text for correlation coefficients
%=======================================

\begin{itemize}
    \item \textbf{Pearson Correlation Coefficient} \cite{benesty2009pearson}: This is the basic coefficient to measure the linear correlation between two data distributions. It can be considered as the normalization version of covariance. Formally, it is presented as
    \begin{align}
        r_{p}=\frac{\sum\left(x_{i}-\bar{x}\right)\left(y_{i}-\bar{y}\right)}{\sqrt{\sum\left(x_{i}-\bar{x}\right)^{2} \sum\left(y_{i}-\bar{y}\right)^{2}}}
    \end{align}
    where $(x_i,y_i)$  denotes the $i$th observed sample pairs of the two distributions $\mathcal{X}$ and $\mathcal{Y}$. $\hat{x}$ and $\hat{y}$ are the respective expected value.
    
    \item \textbf{Spearman'S Correlation Coefficient}\cite{sedgwick2014spearman}: This rank correlation coefficient is used to measure the intensity of the monotonic relationship (i.e. How well to use a monotonic function to present two variables). Formally, it is presented as
    \begin{align}
        r_s = \frac{\operatorname{cov}(\mathrm{R}(X), \mathrm{R}(Y))}{\sigma_{\mathrm{R}(X)} \sigma_{\mathrm{R}(Y)}},
    \end{align}
    where $\mathrm{R}(X)$ and $\mathrm{R}(Y)$ denote the ranks of variable $X$ and $Y$, respectively. $\sigma_{\mathrm{R}(\cdot)}$ denotes the standard deviations of the rank variables. If all ranks are non-overlapping, $r_s$ can be also presented as
    \begin{align}
        r_{s}=1-\frac{6 \sum \left(R(X_i)-R(X_i)\right)^{2}}{n\left(n^{2}-1\right)},
    \end{align}
    where $n$ denotes the number of sample pairs, 
    Noting that this coefficient does not assume the data sampled from a normal distribution and has a linear relationship.
    
    \item \textbf{Kendall Correlation Coefficient} is another rank correlation coefficient, which based on concordance of the pair of observations. Suppose any two pairs of samples $(x_i,y_i)$ and $(x_j,y_j)$, where $i<j$. Two pairs are concordant if $\operatorname{sgn}\left(x_{i}-x_{j}\right)$ and $\operatorname{sgn}\left(y_{i}-y_{j}\right)$ are consistent, where $\operatorname{sgn}(\cdot)$ denotes the sign of the element.
    The coefficient $\tau$ is computed by
    \begin{align}
        \tau=\frac{2}{n(n-1)} \sum_{i<j} \operatorname{sgn}\left(x_{i}-x_{j}\right) \operatorname{sgn}\left(y_{i}-y_{j}\right)
    \end{align}
    Noting that it also does not depend on any assumptions on the distributions and is more robust than Spearman's Correlation Coefficient. 
\end{itemize}


%================================================
% some text for regression
%=================================================
\xc{xiwen: Maybe we can remove some detail for linear regression}
The goal of the association analysis is finding consistent temporal and spatial correlations between the extracted safety metrics and the frequency of different crash types.  

The temporal analysis aims to verify the utility of the proposed metrics in predicting crash count in each road segment for a given time interval. The spatial analysis investigates the generalization of the identified relations to other road segments with similar conditions. 
Our approach to this problem is constructing a linear regression model that explains crash count in terms of extracted safety metrics. More specifically, we have 

\begin{align} \label{eq:linear}
y_i =\mathbf{x}_i^T\mathbf{\beta}+\varepsilon_i, 
\end{align}
where $\mathbf{x}_i=[x_{i1},x_{i2},\dots,x_{iM}]$ is the set of $M$ extracted safety metrics for a given scenario (i.e. time interval), $y_i$ is the crash count, $\mathbf{\beta}_i=[\beta_{i1},\beta_{i2},\dots,\beta_{iM}]$ is the vector of model parameters, and $\varepsilon_i \sim \mathcal{N}(0,\sigma^2)$ is the zero mean model noise with variance $\sigma^2$.  
For instance, to find temporal correlations between the safety metrics and the rear-end crash types in a specific road segment, we split the time into twenty four 1-hour intervals. Then each data sample $\mathbf{x}_i$ represents the average of safety metrics extracted from the traffic video in a 1-hour interval (e.g., 1:00pm-2:00pm) for that specific road segment. Likewise, $y_i$ is the frequency of rear-end crashes for all days of the data during the same time interval (1:00pm-2:00pm) that occurred in the same road segment. 

Our hypothesis is that the extracted safety metrics show strong temporal and spatial correlations with the crash count. To this end, we first show that the developed models have high predictability. Then, we investigate the contribution of each individual safety metric through a formal statistical hypothesis test methods. 



The residual sum of squares (RSS) for model in Eq (\ref{eq:rss}) is calculated as 

 \begin{align}\label{eq:rss}
 RSS=\hat{\mathbb{\varepsilon}}^T\hat{\mathbb{\varepsilon}}=(\mathrm{y}-\mathrm{X}\hat{\mathrm{\beta}})^T(\mathrm{y}-\mathrm{X}\hat{\mathrm{\beta}}),
 \end{align}
where $\mathrm{X}=[\mathbf{x}_1,\mathbf{x}_2,...,\mathbf{x}_N]^T$ is the data matrix (each row is a data sample $\mathbf{x}_i^T$), and  $\hat{\beta}$ is the estimated model parameters. Using the ordinary least square (OLS), solution of $\hat{\mathrm{\beta}}$ is:

 \begin{align}
     \hat{\mathrm{\beta}}=(\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^T\mathrm{y}\sim\textit{N}(\mathrm{\beta},(\mathrm{X}^T\mathrm{X})^{-1}\sigma^2),
 \end{align}

From the frequentist's perspective, the true $\beta$ is deterministic but unknown, and we should estimate $\hat{\beta}$ as close to $\beta$ as possible.
Since $\varepsilon\sim N(0,\sigma^2 I)$, therefore, we have $y\sim N(X\beta,\sigma^2 I)$. Also, we know that the best estimation of $\beta$ by LSE is $\hat{\beta}=(\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^T\mathrm{y}$. Note that $Y\sim N(\mu,\Sigma)$ implies
$(a+BY)\sim N(a+B\mu,B\Sigma B')$; therefore, we have \cite{faraway2004linear}:
% \cite{\url{https://online.stat.psu.edu/stat462/node/137/}} \arr{put the ref here, better to put a book or paper than lecture notes}:

 \begin{align*}
     \hat{\beta}&\sim N(\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^TX\beta,(\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^T((\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^T)^T \varepsilon^2)\\
     \hat{\beta}&\sim N(\beta,(\mathrm{X}^T\mathrm{X})^{-1}\mathrm{X}^T\mathrm{X}(\mathrm{X}^T\mathrm{X})^{-1}\varepsilon^2)\\
     \hat{\beta}&\sim N(\beta,(\mathrm{X}^T\mathrm{X})^{-1}\varepsilon^2)
 \end{align*}
 
This justifies the validity of using the subsequent statistical analysis 
for the relevance of normally distributed model parameters. 
%\fbox{until here}
%\arr{It is not clear what is the main purpose here. The full model is what you explained above, but the one-predictor model does not make a lot of sense. 1-why one predictor and not using 2 or 3 predictors, do you mean adding features greedily until the model is good. And second one predictor model does not provide anything more than checking the Pearson correlation...} 
%\xc{Because this is a backward to select features which begins from the full model. I think the full model can give a global view to see which variables are suitable for a crash type in different segments. The one-predictor model is used to help us to determine which variable is removed first.  }













\item \textbf{T-test}\xc{Plan to remove}: We use this test to verify if a specific predictor of the model is active or not. The hypotheses are:

    \begin{align}
        H_0:&  ~\beta_j=0, \\ \nonumber
        H_a:& ~\beta_j\neq 0.
    \end{align}
The t-test statistic can be computed by:

     \begin{align}
         t_j=\frac{\hat{\beta_j}}{\text{std}(\hat{\beta_j})}\sim t(n-p),
     \end{align}
     where, std$(\hat{\beta_j)}$ is the standard deviation of $\hat{\beta_j}$ computed as
     
    \begin{align}
         \text{std}(\hat{\beta_j)}& = \sqrt{\sigma^2(\mathrm{X}^T\mathrm{X}^{-1})_{jj}}.
     \end{align}
    
    Similarly, If the p-value is less than the given significance level $\alpha$, the predictor contribution is non-zero. %we should reject the null hypothesis.
    
    



==> figures/table.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
Method &
  Dataset &
  Performance(mAP) &
  Features \\ \hline
\multicolumn{4}{|l|}{\textit{One-stage}} \\ \hline
SDS (2014)\cite{hariharan2014simultaneous} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2011\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}52.6\%\\ 51.6\%\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}MCG\cite{arbelaez2014multiscale} to generate proposal;\\ Define Instance Segmentation.\end{tabular} \\ \hline
DeepMask (2015)\cite{pinheiro2015learning} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2007\\ MS COCO\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}improves Fast R-CNN  to 69.9\%@1.2s/image\\ @1.6s/image\end{tabular} &
  Bottom-up proposals generation. \\ \hline
SharpMask (2016)\cite{pinheiro2016learning} &
  MS COCO 2015 &
  25.1\%(AP), 45.8\%(AP^{50}), 24.8\%(AP^{75}) &
  \begin{tabular}[c]{@{}l@{}}Add top-down refinement network\\  to DeepMask.\end{tabular} \\ \hline
MNC (2016) \cite{dai2016MNC}&
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2015\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}63.5\% on validation set (mAP@0.5)\\ 29.7\% on test-dev set(mAP@0.5)\\ @360 ms/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}New Cascaded multi-task architecture;\\ End to End trainable;\\ No external modules.\end{tabular} \\ \hline
Mask R-CNN (2017)\cite{he2017mask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1\%(AP), 60\%(AP^{50}), 39.4\%(AP^{75})\\ @200ms/frame\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of Faster R-CNN;\\ \textit{RoIAlign} can better retain spatial information\end{tabular} \\ \hline
FCIS (2017)\cite{li2017fully} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2016\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}65.7\% (mAP@0.5) and 52.1\% (mAP@0.7) \\ 59.9\%(mAP@0.5) \\ @0.24s/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of InstanceFCN\\ End to end trainable;\\ Can detect and segment objects jointly \\ and simultaneously; \\ Propose position-sensitive inside/outside \\ score maps.\end{tabular} \\ \hline
\multicolumn{4}{|l|}{\textit{Two-stage}} \\ \hline
InstanceFCN(2016)\cite{dai2016instance} &
  PASCAL VOC 2012 &
  61.5\% (mAP@0.5) and 43.0\% (mAP@0.7) &
  \begin{tabular}[c]{@{}l@{}}Propose instance-sensitive score maps;\\ Apply \textit{hole algorithm}\cite{chen2014semantic} to VGGNet;\\ Use  Local coherence to simplify the \\ complexity.\end{tabular} \\ \hline
YOLACT (2019)s\cite{bolya2019yolact} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}29.9\%(AP)@33fps\\ 72.3\%(AP^{50}), 56.2\%(AP^{70})@47.6fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Divide the tasks into non-local prototype \\ masks generation and instance-wise \\ mask coefficients prediction\end{tabular} \\ \hline
YOLACT++(2020)s\cite{bolya2019yolact++} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  33.5(AP)@34.1fps &
  \begin{tabular}[c]{@{}l@{}}Add re-scoring branch;\\ Add DCN to speed up;\\ Try different anchor aspect ratio and scales\end{tabular} \\ \hline
SOLO (2019)\cite{wang2019solo} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1(AP)@10.4fps\\ 34.2(AP)@22.5fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Propose instance category;\\ Only needs to perform two pixel-level \\ classification problem; \\ Global mask representation\end{tabular} \\ \hline
SOLOv2 (2020)\cite{wang2020solov2} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}38.8(AP)@18fps\\ 37.1\%(AP)@31.3fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Improve SOLO by mask learning and\\  \textit{matrix NMS}.\end{tabular} \\ \hline
TensorMask (2019)\cite{chen2019tensormask} &
  MS COCO &
  37.1\% (AP)@0.38s/image &
  \begin{tabular}[c]{@{}l@{}}Represent masks by multi-scale \\ structured high-dimensional(4D) tensors;\\ Scale-adaptive sizes are implemented\\  by Bipyramid structure.\end{tabular} \\ \hline
PolarMask (2020) \cite{xie2020polarmask}&
  MS COCO &
  32.1\% (AP)@12.3fps &
  \begin{tabular}[c]{@{}l@{}}Introduces contour representation\\  in the Polar coordinates;\\ The complexity is close to a \\ single-shot objector.\end{tabular} \\ \hline
BlendMask (2020)\cite{chen2020blendmask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}41.3\%(AP)@116ms/image\\ 34.5\%(AP)@39.7ms/image (real-time setting)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Combine benefits from both top-down \\ and bottom-up methods.\end{tabular} \\ \hline
CondInst (2020)\cite{tian2020conditional} &
  MS COCO &
  35.4\%(AP)@49ms/image &
  \begin{tabular}[c]{@{}l@{}}No need for RoI cropping and \\ feature alignment;\\ mask FCN network parameters are \\ dynamically-generated;\\ Mask prediction heads are compact.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Differences between some state-of-the-art methods. The data of 'Performance' is provided by its corresponding papers. Since test it by different GPU conditions, the numbers are for reference only.}
\label{tab:Instance segementation}
\end{table*}

==> introduction.tex <==
\section{Introduction}






%\arr{no need for this info, comment for later:}
%Since industrial development and technological progress, the manufacturing cost of vehicles has dropped significantly, and benefit from the low cost, people are likely to purchase more vehicles. According to \cite{global_car_sales}, even with the effect of the global coronavirus pandemic, worldwide car sales are supposed to grow to over 71 million. \\



Vehicular technology has witnessed several key milestones in recent years. \arr{add some [but short] details-->]} Electric vehicles (EVs) gradually overtake the regular car markets, and more operation and maintenance and road infrastructures are being developed every year. Moderns are heavily equipped with different sensors and electronics features that make driving more convenient and safer. The use of artificial intelligence (AI) and deep learning (DL) methods have enabled an unprecedented level of autonomy for self-driving cars with day-by-day improvements. High-performance computing (HPCs) and graphics/tensor processing units (GPU/TPUs) have made volume data aggregation and processing, more feasible than ever. Other technologies such as connected vehicles (CVs), and crowd-sourcing methods facilitate data sharing among vehicles for AI-based collective coordination of traffic flow. 


%Another fact is that the annual fatalities of the U.S. rose to 38,680\cite{}. Safety of public transport becomes a critical issue and receives more and more attention from society. 
Despite these technological advances, driving safety remains one of the key challenges of today's society. Statistics how that the mortality of motor-vehicle related injuries have been stayed as high as 11 per hundred thousands people in the last five years in the US  \ar{cite}\cite{https://www.statista.com/statistics/184607/deaths-by-motor-vehicle-related-injuries-in-the-us-since-1950/}. This is a global issue, and about 1.3 million people die by car accidents worldwide and million are injured every year according to world health organization (WHO) \cite{https://www.who.int/news-room/facts-in-pictures/detail/road-safety}. 
These statistics reveals that the modern technology has not yet been fully utilized to prevent these casualties and fatalities, most of which could have been avoided. 


%especially the videos captured by roadside cameras to assess and improve traffic safety. 
Driving safety is pursued from different perspectives by research communities. 
New sensors and warning systems to improve safety of vehicles are under design and development. 
Another research direction is pure safety analysis, where researchers often explore the casualty of incidents based on vehicle geometry and vehicle state ( i.e., the direction, velocity of the vehicle). This analysis rely on a set of key parameters know as \textit{safety metric}. 
\fbox{Razi revised until here}
Additionally, Autonomous Driving (AV) studies often take safety as their primary priority in their set of sub-tasks, such as perception, behavior modeling, motion planning, etc.,. Certainly, since the safety issues, almost all researchers tend to assess their algorithms on simulation platforms (such as SUMO\cite{}, CARLA\cite{}, etc.,.) before deploying them on a real ADS (Automated Driving System)-equipped vehicle. Another branch of studies is interested in network traffic analysis. Many tasks such as road network geometry, congestion prediction, and bottleneck detection serve the improvement of traffic safety. Algorithms from Computer Science can also offer contributions to the analysis of traffic works.  Explicitly, advanced video processing technologies (such as camera calibration, denoising, super-resolution, feature extraction, etc.,. ) can enhance the quality of the collected data. Likewise, data-driven machine learning and deep learning algorithms can be easily deployed and offer more accurate analysis for complicated and dynamic traffic scenarios. We also noted some researchers introduced many cutting-edge technologies to exploit the hardware and communication support for traffic safety. Especially, The recent admirable works also have been benefited from the boosted power of computing platforms, such as Graphics/Tensor Processing Units (GPUs/TPUs). Even High-Performance Computing (HPC) clusters provide a super powerful platform that makes researchers possible to process massive amounts of data. The concept of Vehicular Ad Hoc Networks (VANETs) (e.g., Vehicle-to-Vehicle  (V2V), Vehicle-to-Infrastructure (V2I) communications, and Vehicle-to-Everything (V2X)) and Vehicular Edge Computing (VEC) are established on the development of the Internet of Things (IoTs) and the fast and high-quality wireless communication. 



A new research opportunity is developing integrative analysis frameworks that process multi-modal traffic data (e..g vehicle sensor data, crowd-sourced positioning inform, video collected by roadside and dashboard cameras, EV operation log files, and crash report) to elucidate the most dominant causes of car crashes with hope on developing policies and guidelines that minimizes safety risks. 


%old version: \textcolor{gray}{In fact,  traffic safety is not a narrow sense discipline but involves many academic directions. The data source is fundamental to the whole research. Fortunately, a large number of datasets covering diverse tasks have been collected from multi-modal sources (such as cameras, Lidar, UAVs, etc.) and published in recent years. We review the detailed datasets according to the task taxonomy in the paper\cite{}. The most relevant topics are referred to as pure safety analysis.  Researchers often explore the casualty of incidents based on vehicle geometry and vehicle state ( i.e., the direction, velocity of the vehicle). Besides, researchers develop surrogate metrics to evaluate the safety risks. Additionally, Autonomous Driving (AV) studies often take safety as their primary priority in their set of sub-tasks, such as perception, behavior modeling, motion planning, etc.,. Certainly, since the safety issues, almost all researchers tend to assess their algorithms on simulation platforms (such as SUMO\cite{}, CARLA\cite{}, etc.,.) before deploying them on a real ADS (Automated Driving System)-equipped vehicle. Another branch of studies is interested in network traffic analysis. Many tasks such as road network geometry, congestion prediction, and bottleneck detection serve the improvement of traffic safety. Algorithms from Computer Science can also offer contributions to the analysis of traffic works.  Explicitly, advanced video processing technologies (such as camera calibration, denoising, super-resolution, feature extraction, etc.,. ) can enhance the quality of the collected data. Likewise, data-driven machine learning and deep learning algorithms can be easily deployed and offer more accurate analysis for complicated and dynamic traffic scenarios. We also noted some researchers introduced many cutting-edge technologies to exploit the hardware and communication support for traffic safety. Especially, The recent admirable works also have been benefited from the boosted power of computing platforms, such as Graphics/Tensor Processing Units (GPUs/TPUs). Even High-Performance Computing (HPC) clusters provide a super powerful platform that makes researchers possible to process massive amounts of data. The concept of Vehicular Ad Hoc Networks (VANETs) (e.g., Vehicle-to-Vehicle  (V2V), Vehicle-to-Infrastructure (V2I) communications, and Vehicle-to-Everything (V2X)) and Vehicular Edge Computing (VEC) are established on the development of the Internet of Things (IoTs) and the fast and high-quality wireless communication. }



\ar{Now, lets define the concept of Safety metrics, and mention they are used to analyze individual car accidents. }






\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/topics.png}}
\caption{The various topics related to traffic safety.}
\label{fig:topics}
\end{center}
\end{figure}

\begin{figure*}[]
\begin{center}
\centerline{\includegraphics[width=1\textwidth]{figures/pipeline.png}}
\caption{The pipeline framework. }
\label{fig:pipline}
\end{center}
\end{figure*}




The community has a long history to design, improve, evaluate, and deploy amount of operational metrics, varying from Collision (TTC), Post-Encroachment Time (PET), to Deceleration Rate to Avoid a Crash (DRAC).[A more detail of individual operational metrics can refer to Appendix \ref{sec:safety-metrics}. ] Essentially, design a novel and constructive metrics may regard part or all of the following aspects:
\begin{itemize}
        \item A metric should have a strong-oriented motivation. Before design the metrics, we need investigate the problem or the task expected to solve. Moreover, we may need to seek the theoretical support from existing knowledge.
    \item Consider to the measurement source is also important. Some measurement data can directly obtain by external equipment (such as roadside cameras), while some data should access the measured vehicle. The latter one is often referring to metrics for ADS vehicles (such as) and may involve some privacy issues. The accuracy of the source would be a strong problem challenging the metrics. For example, the roadside cameras are not able to offer accurate location or velocity information for each vehicle since the oblique angle of view leads to environment distortion and vehicles overlapping. Some cameras may jitter because of the wind. The existed calibration algorithms are not feasible to solve all problems perfectly. Moreover, the complexity to obtain the data would be another impact to design metrics, and a complicated data source may result in a low usage frequency. 
    \item A good metrics also have to be defined unambiguously. The basic requirement is that the primitives used to define the metrics should be orthogonal, meaning that this definition cannot be described as a combination of some other metrics. An additional bonus point is that assign the metrics with formulated expression, which may in-depth clarify the concept and be friendly for computing setup. 
    \item The last success factor should be its achievable contribution. Some statistic methods with considerable data may be deployed to verify its effectiveness. The complexity to compute the data partially determines the usage frequency and naturally the contribution of the metrics as well. Generalization of the metrics may also be examined; however, there are many existing metrics that only involve limited objects and with idealized assumption, therefore, they may not directly explain the dynamic traffic well. Notably, in fact, the achievable contribution may take a long time to be evaluated, and some factors may be trade-off according to some piratical issues.
\end{itemize}


\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/metrics_design_factors.png}}
\caption{The basic factors to design a successful metrics.}
\label{fig:design_factor}
\end{center}
\end{figure}

\begin{figure*}[]
\begin{center}
\centerline{\includegraphics[width=0.9\textwidth]{figures/comparison_metrics.png}}
\caption{The schematic diagram of conventional/network-level metrics and the vehicle cluster.(a) The region of interest when measuring conventional metrics. (b) The region of interest when measuring network-level metrics. (c) The concept of the vehicle cluster.}
\label{fig:comparison_metrics}
\end{center}
\end{figure*}

We review the related literature, we admit that many existing works studied on metrics; however, they often only consider the geometry and the state of limited involved vehicles, focus this problem at the incident level, and lack the overall assessment.  In contrast, some literature took their eyes on marco-scale network research and only look at consequences while ignoring the high-resolution driving causes of crashes. specifically, they emphasize traffic properties distribution(e.g., volume, density, congestion condition, etc. ) and road network topology. Other researchers studied the high-resolution mirco-level driving behaviors, but they are weakly correlated with exploring crash causality. According to these limitations, we made the following contribution:
\begin{itemize}
    \item First, we define a set of network-level metrics that gauge the overall safety profile of a traffic network. Figure \ref{fig:comparison_metrics}(a)(b) demonstrates the region of interest of conventional metrics and network-level metrics, respectively. Compared with the incident-level metrics, our proposed network-level metrics is from the micro-level and exploit the inherent relations among all vehicles. 
    \item Secondly, we provide a formal analysis framework to assess the contribution of each safety metric on predicting the crash rate. An overall pipeline is shown in Fig \ref{fig:pipline}. In detail, one branch of the framework is applied to sanitize and organize the crash data, which the second branch is applied to extract and translate the necessary trajectories from traffic surveillance videos. The third branch is applied to computing the value of the network-level metrics from the extracted trajectories. Afterward, the processed metrics value and the crash data will serve spatial association analysis and temporal association analysis. The goal is to verify the effectiveness of the proposed metrics and may benefit future works such as crash explanation, risk prediction, traffic optimization, etc.  
\end{itemize}


The paper is organized as following: ...






















\begin{comment}


(Deep learning method)
Yolo...

(Motivation)
In this paper, our goal is to evaluate the crash risk of current area based on the traffic metrics that captured in real-time, and optimize the road situation according to the deep learning based traffic analysis.

Previous research work [ref] discussed about predict traffic incidents based on the current traffic flow and node analysis. Meanwhile, previous  work only focus on the correlation of the macro level indices and crash ratio. Our work, focus on not just novelty macro level traffic metrics, but we also explored the internal relationships between traffic incidents and the micro level traffic metrics that involved each individual objects.

Based on our developed traffic metrics, it is possible to evaluate the crash risk of current traffic and even predict the traffic incidents at real-time.

\end{comment}




==> network_metrics_draft.tex <==
\section{Proposed Metrics for Network-level Analysis}

It is clear from the discussion above that most of the metrics are defined for scenarios where only two vehicles are involved. This represents a micro-scale perspective to the safety problem while ignoring the network-level metrics that may contribute to the overall traffic safety. For instance, the composition of traffic (e.g., the ratio of trucks to all vehicles) can contribute to the frequency and severity of collisions. In this paper, we take this approach and offer a set of new metrics that can be used for the overall and long-term safety assessment of traffic flow, especially on %cities and 
highways. These are sample metrics, and we do not claim they are comprehensive by any means. Indeed, we believe that this area needs further investigation. The summary of these metrics is provided in Table.\ref{tab:newmetric}. 


\textbf{Individual Velocity Variation Rate (IVVR)} is defined as the variation of velocities for each vehicle in a specific zone or time interval. We define it as
\begin{align}
    IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}
\end{align}
where $v_i^{max},v_i^{min},v_i^{av}$ are the minimum, maximum, and average velocities of vehicle $i$. The higher values of this metric means that on average each vehicle changes its speed more often by accelerating and decelerating. This can be due to the road profile, density of intersections and exits, or road conditions. 


\textbf{Overall Velocity Variation Rate (OVVR)} is defined as the variation of average velocities among vehicles in a specific zone or time interval. OVVR is defined as 
\begin{align}
    OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}},
\end{align}
where $v_i^{av}$ is the average velocity of vehicle $i$, and $v^{av}=\sum_{i=1}^N{v_i^{av}}/N$ is the average velocity of all vehicles. Similar to IVVR, this metric can be associated with crash rate in specific highway sections.

\textbf{Over Speeding Rate (OSR)} is defined as the rate of over-speeding by vehicles as follows:
\begin{align}
    OSR =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max} > v_L),
\end{align}

\begin{align}
    OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i),
\end{align}
%\xc{Modified OSR $OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$. 
%where $Threshold_i>1$ (e.g.,  Levl 1:$Threshold_1=1.1$, Level2:$Threshold_2=1.2$ ... ) indicates the different level of over-speeding }
where $Threshold_i$ is used to capture different levels of over-speeding.
Here, $v_L$ is the speed limit, and $I(x>y)$ is the indicator function with $I(x>y)=1$ for $x>y$ and $I(x>y)=0$ otherwise.  
Speed limits are typically set based on a standardized set of guidelines and national manuals, taking into account road geometry features such as the radii of curves, sight distance, and weather conditions. A high OSR, when associated with a high crash rate, may indicate the need for taking more warning and prevention measures to avoid over-speeding, noting that over-speeding can be an important contributor to crashes. On the other hand, high OSR, when it does not correlate with a high accident rate, can indicate the need for revising the set speed limits without compromising traffic safety. 

The aforementioned traffic metrics can be characterized by processing the roadside cameras or by crowd-sourcing and accumulating information provided by vehicles' dash cameras.

\textbf{Traffic Composition Indicator (TCI)} is defined to gauge the diversity of vehicle types in specific road sections.  
For instance, it is known that a higher density of trucks on roads can correlate with the frequency and severity of road accidents; hence trucks are prohibited in some road sections in highly-populated areas \cite{meyers1981comparison}. This can be due to trucks' larger deceleration inertia, more frequent break failures, and lower maneuverability levels. In general, if vehicles classified into classes $c=1,2,3,\dots,C$, then the traffic composition can be defined as
\begin{align}
    TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2},\\
\end{align}
where $N_c$ is the number of vehicles in class $c$, and the metric is defined similarly to the Jain fairness index. This metric ranges from $1/C$ for the most unbalanced composition to $1$ for an equal number of vehicles from each type. If one is interested in evaluating the rate of a specific class like trucks to all vehicles, the following metric can be used:
\begin{align}
     f_c = \frac{N_c}{\sum_{i=1}^C N_i}.
\end{align}

When classifying cars into two classes $c=1$ for trucks and $c=2$ for non-trucks, these two metrics are related as 
\begin{align}
     TCI = \frac{1}{2(1-2 f_1 f_2)}.
\end{align}

Lower $TCI$ values mean that most cars are of the same type with lower risks. This metric can be estimated by processing roadside videos but requires high-complexity learning methods for vehicle detection and classification. 
 
\textbf{Normalized Traffic Density (NTC)} is defined as the density of vehicles on road sections as 
%  \begin{align}
%      NTC = \frac{N_v}{N_l*L},
%  \end{align}
 
  \begin{align}
     NTC = \frac{\sum l_i/\bar{l}}{N_l*L},
 \end{align}
%\xc{$NTC = \frac{\sum l_i/\bar{l}}{N_l*L},
where  $l_i$ is the length of a vehicle, $\bar{l}$ is the average of all vehicles' length. We normalize the vehicle by its length to capture the effect of vehicle's size. %later we cn check, I am not sure it is necessary to make it this complex?

Here, 
%$N_v$ is the number of vehicles, 
$N_l$ is the number of lanes, and $L$ is the length of the road section. This parameter can be easily captured by video processing and vehicle recognition. Higher NTC values are expected to be associated with higher crash rates, and may raise the request for traffic load balance strategies.  
 
\textbf{Traffic Recovery Time (TRT)} is defined as the time required for traffic flow recovery after accidents. 
The system of vehicular flow can be considered as a non-equilibrium system of interacting particles \cite{sugiyama2008traffic}, and the instability of a flow-free state is induced by the collective effects of the increase of fluctuations. 
It is known that any traffic event can suddenly lead to a jamming state, and TRT reflects the time span from an event epoch to the status change to free flow. This time is expected to be much shorter than the interval between the consecutive events for flow stability. TRT can be defined as:
\begin{align}
    TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|,
\end{align}
where $N_e$ is the number of events in the monitoring interval, and $t_b(i)$ and $t_r(i)$, respectively, denote the event start epoch, and the flow recovery epoch for event $i$. These parameters can be easily captured by roadside videos or fusing information obtained from dash cameras. 
%\arr{update the table accordingly}

The summary of the proposed network-level safety metrics is presented in Table \ref{tab:newmetric}. We believe that this list is not comprehensive by any means and can initiate efforts to develop a more comprehensive list of network-level safety metrics. 

\begin{table*}[htbp]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric} &
  \textbf{Definition} &
  \textbf{Features} \\ \hline
IVVR &
  $IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects the instability of traffic flow by car speed variations and crash rate;\\ Can partially offer network re-design suggestions\end{tabular} \\ \hline
OVVR &
  $OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}}$ &
  \begin{tabular}[c]{@{}l@{}}Overall speed variation of vehicles; \\Defined similar to IVVR for overall traffic speed variation;\\ Not easily affected by outliers \end{tabular}\\ \hline
OSR &
  $ OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$ &
  \begin{tabular}[c]{@{}l@{}}Indication of speed limit violations; Can offer suggestions for network design\end{tabular} \\ \hline
TCI &
  \begin{tabular}[c]{@{}l@{}}$TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2}$\\ $f_c = \frac{N_c}{\sum_{c=1}^C N_c}$\\ $TCI = \frac{1}{2(1-2 f_1 f_2)}$, two classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Flow composition indicator;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
NTC &
  $NTC = \frac{\sum l_i/\bar{l}}{N_l*L}$ &
  \begin{tabular}[c]{@{}l@{}}Consider vehicle shape;\\ Reflects traffic density;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
TRT &
  $TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|$ &
  \begin{tabular}[c]{@{}l@{}}
  A simple and reasonable way to evaluate severity of the accidents;\\
  Can also take traffic stability into consideration\end{tabular}\\ \hline
\end{tabular}%
}
\caption{A set of proposed network-level safety metrics.} %\xc{modified}}
\label{tab:newmetric}
\end{table*}

==> safety.tex <==
\section{Taxonomy for Operational Safety Metrics } \label{sec:safety-metrics}
%\xc{Jeffrey reorganize this section. His comments are in the following}
\begin{comment}


An essential objective of driving safety analysis is extracting \textit{safety metrics}, which are quantifiable measures extracted from traffic videos (or other data sources) that determine the relative risk of an event that may lead to a crash. Here, we review key safety metrics that have been broadly used for driving safety analysis. It is notable that many algorithms developed for AVs utilize safety metrics for safe navigation decisions and avoiding crashes; however, we consider both self-driving and human-driven vehicles.
%the amount of risk into running to a crash between involving vehicles

A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration). A more recent paper provides a more updated list of safety metrics for ADS-equipped vehicles \cite{wishart2020driving}. Two important aspects are considered in this review. First, we propose additional safety metrics for network-level analysis \ar{\cite{wishart2020driving}?}\xc{This work stills focus on only involved vehicles, and doesn't propose any metric for network-level analysis}. Secondly, safety metrics are typically calculated by processing the visual information from the AV's perspective, while we also consider extracting safety features from an external observer's point of view. For example, we consider integrative processing of roadside and aerial traffic videos.  


First, let us review the widely used basic safety metrics of (i) temporal-based indicators: Time to Collision (TTC), Extended Time to Collision (Time Exposed Time-to-Collision(TET), Time Integrated Time-to-Collision(TIT)\cite{minderhoud2001extended}), Modified TTC (MTTC), Crash Index (CI), Time-to-Accident (TA), Time Headway (H), and Post-Encroachment Time (PET); (ii) distance-based indicators: Potential Index for Collision with Urgent Deceleration (PICUD), Proportion of stopping Distance (PSD), Margin to Collision (MTC), Difference of Space Distance and Stopping Distance (DSS), Time Integrated DSS (TIDSS), and Unsafe Density (UD); (iii) deceleration-based indicators: Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index(CPI), and Criticality Index Function (CIF). 

Our main references include \cite{gettman2003surrogate}, \cite{mahmud2017application} and \cite{wishart2020driving}. 

We also mention the approach an observer system takes to monitor video and extract safety metrics. The observer system also called \textbf{system} in the rest of this paper for convenience, is a terrestrial or aerial monitoring system that collects traffic video for processing from an external observer's point of view. 
A list of these metrics, along with their brief descriptions, is presented in Table \ref{tab:metrics}.

\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


%\begin{figure}[htbp]
%\begin{center}
%\centerline{\includegraphics[width=0.8\columnwidth]{figures/human-driven metrics.png}}
%\caption{Related metrics on a conflict point.Source from \cite{gettman2003surrogate}}
%\label{fig:safety metircs}
%\end{center}
%\end{figure}






%\section{Operational Safety Metrics}\label{Jeffrey comment}
An essential objective of driving safety analysis is extracting \textit{operational safety metrics}, which are quantifiable measures extracted from traffic videos (or other data sources) that determine the relative risk of an event that may lead to a crash. 

In this section, we review key safety metrics that have been broadly used for driving safety analysis. 
%A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration). A more recent paper provides a more updated list of safety metrics for ADS-equipped vehicles \cite{wishart2020driving}. 
%Razi added
Two aspects are considered in our review.  First, we consider both AVs and human-driven vehicles, in contrast to some work that focus only on one class of vehicles. Secondly, we consider extracting and processing safety metrics from an external observer's point of view, such as a roadside infrastructure, or an aerial traffic monitoring system.  
A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration):
\begin{enumerate}[i]
  \item \textbf{Temporal-based indicators:} Time to Collision (TTC), Extended Time to Collision (Time Exposed Time-to-Collision(TET), Time Integrated Time-to-Collision(TIT)\cite{minderhoud2001extended}), Modified TTC (MTTC), Crash Index (CI), Time-to-Accident (TA), Time Headway (H), and Post-Encroachment Time (PET). 
  \item \textbf{Distance-based indicators:} Potential Index for Collision with Urgent Deceleration (PICUD), Proportion of stopping Distance (PSD), Margin to Collision (MTC), Difference of Space Distance and Stopping Distance (DSS), Time Integrated DSS (TIDSS), and Unsafe Density (UD);
  \item \textbf{Deceleration-based indicators:} Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index(CPI), and Criticality Index Function (CIF).
\end{enumerate}

A more recent paper \cite{wishart2020driving} by the safety metric team of the Institute of Automated Mobility (IAM), whose project leader is the co-author of our paper, provides a comprehensive set of operational safety metrics following an extensive literature review. The objective was to develop a set of metrics for both human-driven and AVs that includes existing, adapted, and novel metrics. In a follow-up paper\cite{elli2021evaluation}, the IAM proposed a taxonomy for operational safety metrics that is explored and expanded upon here. The IAM work is also a component of an Information Report being developed by the SAE Verification and Validation (V\&V) Task Force under the On-Road Automated Driving (ORAD) Committee\cite{OSM2020}. The taxonomy will be introduced first, and then selected operational safety metrics will be discussed (including the metrics from \cite{mahmud2017application} listed above).

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/taxonomy_2.jpg}}
\caption{Operational safety metrics taxonomy proposed by the IAM.}
\label{fig:taxonomy}
\end{center}
\end{figure}





The expanded taxonomy introduced here is shown in Figure.\ref{fig:taxonomy}. The highest taxonomic rank in the proposed taxonomy hierarchy consists of three types that are based, essentially, on the data source, which includes the level of access required of ADS data. This access to proprietary data could be challenging, depending on the implementation of the operational safety metric; it should be noted that “lighter” metrics require more cooperation with the AV developer. The three types are (example metrics are given for each, and are described in more detail later in the section):
\begin{enumerate}
\item \textbf{Black Box Metric:} A metric that allows measurement of data that can be obtained without requiring any access to ADS data. This could be from an on-board or off-board source. ADS data may enhance the accuracy and precision of the measurement(s).
EXAMPLE: Proper Response Action (PRA).

\item \textbf{Grey Box Metric:} A metric that allows measurement of data that can only be obtained with limited access to ADS data.
EXAMPLE: ADS DDT Execution (ADE).

\item \textbf{White Box Metric:} A metric that allows measurement of data that can only be obtained with significant access to ADS data.
EXAMPLE: Perception Precision (PP).
\end{enumerate}

The second rank in the taxonomic hierarchy is the classification rank, which consists of the following (again, an example metric that is described later in the section is included):
\begin{enumerate}
\item\textbf{Safety Envelope Metric:} A metric that allows for measurement of the subject vehicle’s maintenance of a safe boundary around itself. This includes situations that may not be within the subject vehicle’s control.
		EXAMPLE: Rear End Collision Incident (RECI).
\item\textbf{Behavioral Metric:} A metric that allows for measurement of an improper behavior of the subject vehicle.
EXAMPLE: Aggressive Driving (AD).
	
\item\textbf{Component Metric:} A metric that allows for measurement of the proper function of ADS components.
EXAMPLE: Event Data Recorder Compliance (EDRC).
	
\item\textbf{Sensing Metric:} A metric that allows for measurement of the ability of the ADS sensors to receive adequate information from the AV environment.
EXAMPLE: Camera Resolution (CR).
	
\item\textbf{Perception Metric:} A metric that allows for measurement of the ability of the ADS to interpret information about the AV environment obtained by the ADS sensors.
EXAMPLE: Human Traffic Control Detection Error Rate (HTCDER).
	
\item\textbf{Planning Metric:} A metric that allows for measurement of the ability of the ADS to plan an appropriate route through the AV environment.
EXAMPLE: Object Avoidance Plan Error (OAPE).
	
\item\textbf{Control Metric:} A metric that allows for measurement of the ability of the AV to execute the planned route devised by the ADS.
EXAMPLE: Actuation Error (AE).

\end{enumerate}

It is important to note that not all classification rank types link to data source rank types in the current version. For example, the Component Metric is not linked to the Black Box Metric because data at the component level is deemed to be more access to (potentially proprietary) data than is allowed for the Black Box Metric.

The metrics currently being considered for inclusion in the SAE J3237 Information Report\footnote{This SAE standards document is currently in development and the operational safety metrics list could be modified, expanded, or contracted. In particular, additional White Box metrics are currently being considered.} include in Table \ref{tab:taxonomy}. The IAM has focused on Black Box Metrics and Grey Box Metrics as part of the comprehensive set introduced in \cite{mahmud2017application}.\\
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{0.8\textwidth}{!}{
\centering%
\begin{tabular}{|l|c|c|}
\hline\rowcolor{gray} 
\multicolumn{1}{|c|}{\textbf{Metric Name}}               & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ Source \\ Taxonomy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classification\\  Taxonomy\end{tabular}} \\ \hline
Minimum Safe Distance Violation (MSDV)                   & Black                                                                       & Safety Envelope                                                             \\
Proper Response Action (PRA)                             & Black                                                                       & Safety Envelope                                                             \\
Minimum Safe Distance Factor (MSDF)                      & Black                                                                       & Safety Envelope                                                             \\
Time-to-Collision (TTC)                                  & Black                                                                       & Safety Envelope                                                             \\
Modified Time-to-Collision (MTTC)                        & Black                                                                       & Safety Envelope                                                             \\
Time Headway (TH)                                        & Black                                                                       & Safety Envelope                                                             \\
Instantaneous Safety Metric (ISM)                        & Black                                                                       & Safety Envelope                                                             \\
Collision Avoidance Capability (CAC)                     & Black                                                                       & Safety Envelope                                                             \\
Minimum Safe Distance Infringement (MSDI)                & Black                                                                       & Safety Envelope                                                             \\
Post-Encroachment Time (PET)                             & Black                                                                       & Safety Envelope                                                             \\
Not-at-Fault Collision Incident (NAFCI)                  & Black                                                                       & Safety Envelope                                                             \\
Rear-End Collision Incident (RECI)                       & Black                                                                       & Safety Envelope                                                             \\
Deceleration Rate to Avoid the Crash (DRAC)              & Black                                                                       & Safety Envelope                                                             \\
Difference of Space Distance and Stopping Distance (DSS) & Black                                                                       & Safety Envelope                                                             \\
Maximum Speed (MaxS)                                     & Black                                                                       & Behavioral                                                                  \\
Delta Velocity ($\Delta$V)                                      & Black                                                                       & Behavioral                                                                  \\
Traffic Law Violation (TLV)                        & Black                                                                       & Behavioral                                                                  \\
Evasive Action (EA)                                      & Black                                                                       & Behavioral                                                                  \\
Aggressive Driving (AD)                                  & Black                                                                       & Behavioral                                                                  \\
Collision Incident (CI)                                  & Black                                                                       & Behavioral                                                                  \\ \hline
ADS DDT Execution (ADE)                                  & Grey                                                                        & Control                                                                     \\
Achieved Behavioral Competency (ABC)                     & Grey                                                                        & Planning                                                                  \\
Human Traffic Control Perception Error Rate (HTCDER)     & Grey                                                                        & Perception                                                                  \\
Human Traffic Control Violation Rate (HTCVR)             & Grey                                                                        & Behavioral                                                                  \\
Minimum Safe Distance Calculation Error (MSDCE)          & Grey                                                                        & Perception                                                                  \\
Safety-Related Component Failure Perception (SRCFD)      & Grey                                                                        & Component                                                                   \\
Event Data Recorder Compliance (EDRC)                    & Grey                                                                        & Component                                                                   \\ \hline
Perception Precision (PP)                                & White                                                                       & Perception                                                                  \\
Perception Perception Rate (PDR)                         & White                                                                       & Perception                                                                  \\
Perception Weighted Harmonic Mean (PWHM)                 & White                                                                       & Perception                                                                  \\
Perception False Positive Rate (PFPR)                    & White                                                                       & Perception                                                                  \\
Perception False Negative Rate (PFNR)                    & White                                                                       & Perception                                                                  \\
Anomaly Perception Behavior (ADB)                        & White                                                                       & Perception                                                                  \\
Multiple Object Perception Error Rate (MODER)            & White                                                                       & Perception                                                                  \\
Localization Error (LE)                                  & White                                                                       & Perception                                                                  \\
Multiple Object Tracking Precision (MOTP)                & White                                                                       & Perception                                                                  \\
Data Conflict Perception Rate (DCDR)                     & White                                                                       & Perception                                                                  \\
Intersection over Union (IoU)                            & White                                                                       & Perception                                                                  \\
Actuation Error (AE)                                     & White                                                                       & Control                                                                   \\
Software Execution Error (SEE)                           & White                                                                       & Component                                                                   \\
Object Avoidance Plan Error (OAPE)                       & White                                                                       & Planning       \\\hline                                                            
\end{tabular}%
}
\caption{Current SAE J3237 Information Report operational safety metrics.}
\label{tab:taxonomy}
\end{table*}
\indent We also mention the approach an observer system takes to monitor video and extract safety metrics. The observer system also called system in the rest of this paper for convenience, is a terrestrial or aerial monitoring system that collects traffic video for processing from an external observer’s point of view. A list of these metrics, along with their brief descriptions, is presented in Table \ref{tab:metrics}. 

Our main references include \cite{gettman2003surrogate}, \cite{mahmud2017application} and \cite{wishart2020driving}. 
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric}     & \textbf{Definition} & \textbf{Features}                                                                                                                         \\ \hline
MaxS       & $\max v$         & A simple but effective measure of the severity of a collision.                                                                   \\ \hline
$\Delta v$    & $\Delta v$          & An effective indicator of the severity of a collision.                                                                           \\ \hline
TTC &
  $TTC =\frac{X_L-X_F}{v_F-v_L}$ &
  \begin{tabular}[c]{@{}l@{}}Provides more information than PET; assumes that involved vehicles are at a constant speed;\\ cannot reflect the severity.\end{tabular} \\ \hline
PET &
  $PET =t_2-t_1$ &
  \begin{tabular}[c]{@{}l@{}}Can be easily captured and computed; suitable for assessing intersecting conflicts; \\ only suitable for the cases of transversal trajectories;\\ cannot reflect the severity.\end{tabular} \\ \hline
Initial DR & $DR_{t=0}$          & A basic indicator; cannot consider the following vehicle's acceleration/deceleration.                                                        \\ \hline
DRAC       &$TTC =\frac{(v_F-v_L)^2}{X_L-X_F}$         & \begin{tabular}[c]{@{}l@{}}No need to directly observe the deceleration rate; \\ does not work for lateral movement\end{tabular}      \\ \hline
CPI        & $CPI_i=\frac{\sum_{t=t_i}^{tf_i}P(DRAC_{i,t})\geq MADR\Delta t\cdot b}{T_i}$          & Considers more factors such as traffic and road conditions compared to DRAC;                                                         \\ \hline
PSD        &\begin{tabular}[c]{@{}l@{}}$PSD =\frac{RD}{MSD}$;\\ $ PSD =\frac{v^2}{2MADR} $ \end{tabular}      & \begin{tabular}[c]{@{}l@{}}Works for a conflict with a single vehicle involved; \\ \rarely used for specific safety problems.\end{tabular} \\ \hline
UD &
  $UD=\frac{\sum_{S=1}^{S_t}\sum_{V=1}^{V_t}unsafety_{V,S}\cdot d}{TL}$ &
  \begin{tabular}[c]{@{}l@{}} Delivers more accurate information than typical micro-simulation outputs;\\ allows comparison between simulation scenarios or links;\\ some parameters are difficult to capture automatically;\\ only applicable to identical trajectories.\end{tabular} \\ \hline
  
  MSDV &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle violate safety boundary of another.\\ Safety boundary: $d_{min}^{long,same}$(Eq.\ref{eq:d_long_same}) $d_{min}^{long,opp}$(Eq.\ref{eq:d_long_opp}) and $d_{min}^{lat}$(Eq.\ref{eq:d_lat})\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Provides how to calculate the quantified risky distances;\\ a basis of many assessment methods.\end{tabular} \\ \hline
PRA &
  \begin{tabular}[c]{@{}l@{}}An action to recover when\\ $d_{min}^{long},d_{min}^{lat}$ and the safe range of $a^{lat}$,$a^{long}$ are violated\end{tabular} &
  Adds more information beyond MSDV. \\ \hline
MSDF &
  \begin{tabular}[c]{@{}l@{}}$MSDF^{lat} = \frac{d^{lat}}{d^{lat}_{min}}$\\ $MSDF^{long} = \frac{d^{long}}{d^{long}_{min}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Can indicate the degree of defensive driving style;\\ a higher $MSDF$ may not means higher safety.\end{tabular} \\ \hline
MSDCE &
  $MSDCE = \sqrt{\frac{\vert d^{long}_{gt,min} - d^{long}_{min}\vert }{d^{long}_{gt,min}}+\frac{\vert d^{lat}_{gt,min} - d^{lat}_{min}\vert }{d^{lat}_{gt,min}}}$ &
  Indicate the ADS ability to determine the safety distances. \\ \hline
CI &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle is involved in a collision.\\ Active when $d^{lat}$ and $d^{long}$ are equal to 0.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Capture instances of collisions as a metric;\\ the severity of the collision can be defined by KABCO scale\cite{herbel2010highway}:\\
  K(Fatal Injury), A(Incapacitating Injury), B (Non-Incapacitating Injury),\\ C(Possible Injury), O(No Injury).\end{tabular} \\ \hline
TLV &
  Indicate the subject vehicle that violates a traffic law &
  \begin{tabular}[c]{@{}l@{}}Emphasizes that an ADS vehicle must follow existing laws;\\ exceptions are made, for example, when road closures \\ require temporary violations of driving exclusively inside a traffic lane.\end{tabular} \\ \hline
ABC &
  Indicate the subject vehicle can execute a specific behavior correctly. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics.\end{tabular} \\ \hline
ADSA &
  Indicate the ADS is active when executing behaviors. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics;has some dispute in California\cite{hawkins2019california}.\end{tabular} \\ \hline
HTCDER &
  $HTCDER = \frac{GTI-CDI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
HTCVR &
  $HTCVR = \frac{CDI-CCI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
  
AD &
  \begin{tabular}[c]{@{}l@{}}Indicate the maneuvers (longitudinal/lateral accelerations) \\ of a subject vehicle exceeds specified thresholds.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The thresholds vary by jurisdiction and culture;\\ AD is only involved the subject vehicle;\\ implies the inherent and potential risks of natural driving behaviors;\\ should be included when evaluating ADS.\end{tabular} \\ \hline  
  
  
\end{tabular}%
}
\caption{%Some broadly-used safety metrics along with their key properties.\xc{
Summary of operational safety metrics along with their key properties.}
\label{tab:metrics}
\end{table*}


\subsection{Summary of Basic Operational Safety Metrics}

~~~\textbf{Maximum Speed (MaxS)}, when associated with a collision, denotes the maximum speed of the involved vehicles before the crash starts until the full stop (e.g., between time points $t_1$ and $t_4$ in Fig.\ref{fig:safety metircs} 
%\arr{update all time epochs according to the new figures: we have no t5 in the new figure}). 
MaxS is a simple but effective measure directly related to the severity of the collision.


\textbf{Differential Speed ($\Delta s$)} is defined as the relative speed between the involved vehicles. It occurs at $t_2$ in Fig.\ref{fig:safety metircs}.
The system needs to calculate the speed of the involved vehicles (using methods like DL-based object tracking with or without explicitly extracting the motion trajectories) to determine MaxS and $Delta s$.
\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/mymetric2.png}}
\caption{The space-speed pair diagram of a rear-end collision. $t_1$ is the time epoch the leading vehicle begins to decelerate (encroachment begin). $t_2$ is the epoch the following vehicle begins to decelerate. $t_1$-$t_2$ is the reaction time of the driver of the following vehicle. $t_3$ is the projected arrival moment of the following vehicle (under no deceleration). $t_4$ is the actual collision moment.}
\label{fig:safety metircs}
\end{center}
\end{figure}

\textbf{Time to Collision (TTC)} is a commonly used surrogate measure to define the time of an upcoming rear-end collision between two vehicles, if they continue their current speed ($t_2$-$t_3$  in Fig. \ref{fig:safety metircs}). The system needs to observe the relative position and calculate the relative velocity of the two involved vehicles. 
TTC is computed as:
\begin{align}
\label{eq:TTC}
    TTC =\frac{X_L-X_F}{v_F-v_L},
\end{align}
where $X_i$ denotes the position, $v_i$ denotes the velocity, and the indexes $L$ and $F$, respectively, denote the leading and following vehicles. The collision occurs only if $v_F\geq v_L$. Usually, we have $v_L \geq 0$ assuming that the cars move in the same direction. $v_L \leq 0$ represents a vehicle approaching from the front. The severity of an encounter can be determined by the minimum TTC (TTCmin). 
Although very useful in investigating crashes, this metric has some limitations. First, TTC assumes that involved vehicles are moving at constant speeds, which ignores the potential dangers caused by acceleration or deceleration. Secondly, it assumes that the cars drive in the same direction and not appropriate for side crashes. 




\textbf{Post-Encroachment Time (PET)} is defined as the time span between the encroached vehicle leaving and the other vehicle with the right-of-way arriving at the conflict point. The system needs to observe the relative time of the involved vehicles and estimate the conflict point. 
PET in Fig.\ref{fig:PET} is computed as:
\begin{align}
\label{eq:PET}
    PET =t_b-t_a,  
\end{align}
where $t_a$ and $t_b$ represent the arrival time of the two involved vehicles. 
PET can be easily captured and computed by the system. However, it is suitable for intersection conflicts with transversal trajectories, but it does not fully reflect the severity of the crash. 

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/PET1.png}}
\caption{The schematic diagram of PET.}
\label{fig:PET}
\end{center}
\end{figure}



\textbf{Initial Deceleration Rate (Initial DR)} quantifies the avoidance behavior taken by a vehicle to avoid a collision. More specifically, Initial DR (the second derivative of Curve B at time point $t_2$ in Fig.\ref{fig:safety metircs}) is defined as the deceleration rate $a_0$ at the beginning of the decelerating state. Deceleration rate is an appreciated variable to assess the potential severity of a conflict. Other variants of this metric family include Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index (CPI), and Criticality Index Function (CIF). 

\textbf{Deceleration Rate to Avoid a Crash (DRAC)} is defined as the minimum deceleration rate of the following vehicle to avoid a crash to the leading vehicle. 
To characterize this metric, the observer system should keep track of the relative positions and the relative velocities of the two vehicles. Note that DRAC fails to evaluate lateral movements and is applicable only to scenarios where both cars are on the same lane. Mathematically, DRAC is defined as 
\begin{align}
\label{eq:DRAC}
    DRAC =\frac{(v_F-v_L)^2}{X_L-X_F}. 
\end{align}


\textbf{Crash Potential Index (CPI)} is defined as the probability of DRAC exceeding the Maximum Available Deceleration Rate (MADR) at any moment. 
%\arr{Clarify: at any moment? or at the current moment?}\xc{Like the equation shown, the moment means the observation time step. CPI is considered the total time interval }. 
MADR depends on the type of the vehicle as well as the environmental conditions. The system needs to calculate MADR of the target vehicles and instantaneous track time-variant deceleration to obtain the %for safety analysis and 
crash likelihood. CPI is defined as 
\begin{align}
    CPI_i=\frac{\sum_{t=t_i}^{tf_i}P(DRAC_{i,t})\geq MADR ~\Delta t\cdot b}{T_i},
\end{align}
where $t_i$ and $tf_i$ are the initial and final time intervals of vehicle $i$, respectively, $T_i$ denotes the total travel time of vehicle $i$, $\Delta t$ is the observation time step, and $b$ is a binary state variable with $b=1$ for active state and $b=0$ for inactive state. Compared with DRAC, CPI considers more factors such as the traffic and road conditions, but it is not yet suitable for assessing lateral movements.




%Wrong notation: \textbf{Proportion of Stopping Distance (PSD)} is defined as the ratio of the remaining distance (RD) from the current position to the potential collision point to the acceptable minimum stopping distance (MSD). 
\textbf{Proportion of Stopping Distance (PSD)} is defined as the ratio of the Remaining Distance (RD) from the current position to the potential collision point to the acceptable Minimum Stopping Distance (MSD).
It can be stated as
\begin{align}
\label{eq:PSD}
    PSD =\frac{RD}{MSD}.
\end{align}



%Noting that here, MSD is under the assumption of maximum deceleration, we can write MSD as:
If MSD is considered under maximum deceleration, then PSD becomes:
\begin{align}
\label{eq:MSD}
    PSD =\frac{v^2}{2 MADR}.
\end{align}

PSD is an easily observable indicator and is one of the few metrics that can be used for a conflict involving a single vehicle (e.g., crashing into a stationary obstacle like a tree). PSD is defined for evasive actions and usable only for specific safety problems.




\textbf{Unsafe Density (UD)} is defined as the severity of the potential crash when the leading vehicle is within the achievable maximum DR. This metric is introduced in \cite{torday2003indicator}. When multiple cars involved, this metric considers all cars in a link, while the similar metric of UnSafety (UNS) considers only two of the cars from the link to calculate the $UNS$ of car $v$ at time step $s$, denoted by $UNS_{v,s}$. 

According to \cite{torday2003indicator}, the severity of a read-end crash is proportional to $\Delta v$, and $v_F$. %, and but $R_d$ can be obtained, so multiply the ratio $R_d$. 
More specifically, UNS is defined as:
\begin{align}
    UNS = \Delta v\cdot v_F\cdot R_d,
\end{align}
where $R_d$ denotes the ratio between the deceleration of the leading vehicle and its maximum deceleration capacity, namely
\begin{equation}
    R_d=
\begin{cases}
b/b_{max}& \text{b<0}\\
0& \text{else}
\end{cases}.
\end{equation}
Then, UD can be written as:
\begin{align}
    UD=\frac{\sum_{S=1}^{S_t}\sum_{V=1}^{V_t} UNS_{V,S}\cdot d}{TL},
\end{align}
where $S_t$ denotes the number of simulation steps within the aggregation period, $V_t$ denotes the number of vehicles in the link, $d$ denotes the time span between the two simulation steps, $T$ denotes the aggregation period, and $L$ denotes the section length for which the metrics are evaluated. 

UD provides more accurate information than typical micro-simulation outputs and allows comparison between the simulation scenarios or links. In a transportation network, each intersection is considered as a node, and the traffic flow between the nodes is represented by a link. 
%For limitation, some parameters of UD are difficult to be captured automatically, and it is only applicable for identical trajectory.
The two limitations of the UD parameter include (i) the difficulty of quantifying its constituent parameters and (ii) its applicability only to identical trajectories, namely when two cars move in the same direction, and the type of the potential crash is rear-end collision.

\subsection{Operational safety metric for ADS proposed by the IAM} 
%revised by Razi
Here, we review part of the recently proposed metrics by the IAM \cite{wishart2020driving}. These metrics are developed by a team whose leader is a co-author of this paper. 

\textbf{Minimum Safe Distance Violation (MSDV)} is defined to indicate that the subject vehicle violates the safety envelope of another entity (often is another vehicle). When the subject vehicle (subscript 1) is following behind another entity (subscript 2) and both of them are moving in the same direction. The longitudinal boundary can be defined as:
\begin{align}\label{eq:d_long_same}
    d_{min}^{long,same} &= v_1^{long}\rho_1+\frac{1}{2}a_{1,max,acc}^{long}\rho_1^2\\\nonumber
    &+ \frac{(v_1^{long}+a_{1,max,acc}^{long}\rho_1)^2}{2a_{2,min,dec}^{long}}\\\nonumber
    &-\frac{(v_2^{long})^2}{2a_{2,max,dec}^{long}},
\end{align}
where $v_i^{long/lat}$ denotes the current longitudinal/lateral velocity of  vehicle $i$, $a_{i,max/min,acc/dec}^{long/lat}$ denotes the longitudinal/lateral maximum/minimum acceleration/deceleration of vehicle $i$, and $\rho_i$ denotes the response time of vehicle $i$. 
When two involved vehicles are moving in opposite directions towards each other, the longitudinal boundary can be defined as: 
\begin{align}\label{eq:d_long_opp}
    d_{min}^{long,opp} =& v_1^{long}\rho_1+\frac{1}{2}a_{1,max,acc}^{long}\rho_1^2\\ \nonumber
    +& \frac{(v_1^{long}+a_{1,max,acc}^{long}\rho_1)^2}{2a_{1,min,dec}^{long}}\\ \nonumber
    +& \vert v_2^{long}\vert\rho_2+\frac{1}{2}a_{2,max,acc}^{long}\rho_2^2\\\nonumber
    +& \frac{(\vert v_2^{long}\vert+a_{2,max,acc}^{long}\rho_2)^2}{2a_{2,min,dec}^{long}}
\end{align}
The lateral boundary can be defined as:
\begin{align}\label{eq:d_lat}
    d_{min}^{lat} = \mu+ & v_1^{lat}\rho_1+\frac{1}{2}a_{1,max,acc}^{lat}\rho_1^2\\\nonumber
    +& \frac{(v_1^{lat}+a_{1,max,acc}^{lat}\rho_1)^2}{2a_{1,min,dec}^{lat}} \\\nonumber
    - & [v_2^{lat}\rho_2-\frac{1}{2}a^{lat}_{2,max,acc}\rho_2^2\\\nonumber
    -& \frac{(v_2^{lat}-\rho_2 a_{2,max,acc}^{lat})^2}{2a_{2,min,dec}^{lat}} ],
\end{align}
where $\mu$ is the lateral fluctuation margin. 
Noting that if the calculated result of $d_{min}^{long,same}$ or $d_{min}^{lat}$ is negative, it should be rounded up to 0. 
While the two boundaries are violated by the subject vehicle, MSDV is active ($MSDV=1$), meaning that %the binary status of the metric is equal to 1), which means 
an avoidable accident may occur. This metric characterizes the quantified risky distances as the basis of many assessment methods.

\textbf{Proper Response Action (PRA)} is defined to indicate a proper action taken by the subject vehicle to recover itself when safety boundaries ($d_{min}^{long},d_{min}^{lat}$ and the safe range of $a^{lat}$,$a^{long}$) are violated. It adds more information beyond MSDV to evaluate the driving safety of the subject vehicle.  

\textbf{Minimum Safe Distance Factor (MSDF)} is defined as the ratio between the current distance[s] to the calculated safe boundaries from the surrounding entity.
It can be found as:
\begin{align}
    &MSDF^{lat}& = \frac{d^{lat}}{d^{lat}_{min}}, &  MSDF^{long}& = \frac{d^{long}}{d^{long}_{min}},
\end{align}
where $d^{lat}$ and $d^{long}$ denote the measured distances. $MSDF\geq 1$ indicates the degree of defensive driving style. Note that a higher $MSDF$ may not mean a higher safety, necessarily.

\textbf{Minimum Safe Distance Calculation Error (MSDCE)} is defined as the difference between the calculated results by ADS from the ground truth. It can be formulated as:
\begin{align}
    MSDCE = \sqrt{\frac{\vert d^{long}_{gt,min} - d^{long}_{min}\vert }{d^{long}_{gt,min}}+\frac{\vert d^{lat}_{gt,min} - d^{lat}_{min}\vert }{d^{lat}_{gt,min}}}
\end{align}

This metric is derived from the MSDV, which indicates the ADS ability to determine the safety distances.

\textbf{Collision Incident (CI)} is defined to indicate the subject vehicle is involved in a collision determined by the reasonably related data. CI is active when $d^{lat}$ and $d^{long}$ are equal to 0. Also, the severity of the collision can be defined by KABCO scale\cite{herbel2010highway} with K(Fatal Injury), A(Incapacitating Injury), B (Non-Incapacitating Injury), C(Possible Injury), O(No Injury). 

\textbf{Traffic Law Violation (TLV)} is defined to indicate the subject vehicle that violates a traffic law which would result in an infraction or citation. Violating these laws sets TLV active. This metric emphasizes that an ADS-vehicle must follow existing laws, and an active TLV may lead to severe safety issues. It should be noted that exceptions to a TLV are made, for example, when road closures require temporary violations of driving exclusively inside a traffic lane.

\textbf{Achieved Behavioral Competency (ABC)} is defined to indicate the subject vehicle can execute a specific behavior correctly. This metric indicates the safety of ADS and is included in the preliminary list of ADS vehicles' metrics.

\textbf{ADS Active (ADSA)} is defined to indicate that the ADS is active when executing behaviors. This metric represents the safety of ADS and is included in the preliminary list of ADS vehicles' metrics. The metric has some dispute in California\cite{hawkins2019california}.

\textbf{Human Traffic Control Detection Error Rate (HTCDER)} is defined as the capability to detect instructions from a Human Traffic Control (HTC) actor correctly. It is calculated as:
\begin{align}
    HTCDER = \frac{GTI-CDI}{CDI},
\end{align}
where $GTI$ is the number of ground truth instructions, and $CDI$ is the number of correctly detected instructions. This metric is one of the HTC measurements to evaluate the safety of the subject vehicle. Note that the manual instructions by officers should still be considered in this metric.

\textbf{Human Traffic Control Violation Rate (HTCVR)} is defined as the capability of a subject vehicle to follow the received instructions successfully. It is formulated as:
\begin{align}
    HTCVR = \frac{CDI-CCI}{CDI},
\end{align}
where $CCI$ is the number of correctly compiled instructions. %This metric is another HTC measurement and has similar cases to HTCDER. 

\textbf{Aggressive Driving (AD)} is defined to indicate the maneuvers (longitudinal/lateral accelerations) of a subject vehicle exceeding specified thresholds. When exceeding ($a\geq a_T$), the metric is set active. The thresholds vary by jurisdiction and culture. This metric involves only the subject vehicle and implies the inherent and potential risks of natural driving behaviors. When evaluating the safety of ADS, this metric should be included. 


\section{Proposed Metrics for Network-level Analysis}

It is clear from the discussion above that most of the metrics are defined for scenarios where only two vehicles are involved. This represents a micro-scale perspective to the safety problem while ignoring the network-level metrics that may contribute to the overall traffic safety. For instance, the composition of traffic (e.g., the ratio of trucks to all vehicles) can contribute to the frequency and severity of collisions. In this paper, we take this approach and offer a set of new metrics that can be used for the overall and long-term safety assessment of traffic flow, especially on %cities and 
highways. These are sample metrics, and we do not claim they are comprehensive by any means. Indeed, we believe that this area needs further investigation. The summary of these metrics is provided in Table.\ref{tab:newmetric}. 


\textbf{Individual Velocity Variation Rate (IVVR)} is defined as the variation of velocities for each vehicle in a specific zone or time interval. We define it as
\begin{align}
    IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}
\end{align}
where $v_i^{max},v_i^{min},v_i^{av}$ are the minimum, maximum, and average velocities of vehicle $i$. The higher values of this metric means that on average each vehicle changes its speed more often by accelerating and decelerating. This can be due to the road profile, density of intersections and exits, or road conditions. 


\textbf{Overall Velocity Variation Rate (OVVR)} is defined as the variation of average velocities among vehicles in a specific zone or time interval. OVVR is defined as 
\begin{align}
    OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}},
\end{align}
where $v_i^{av}$ is the average velocity of vehicle $i$, and $v^{av}=\sum_{i=1}^N{v_i^{av}}/N$ is the average velocity of all vehicles. Similar to IVVR, this metric can be associated with crash rate in specific highway sections.

\textbf{Over Speeding Rate (OSR)} is defined as the rate of over-speeding by vehicles as follows:
\begin{align}
    OSR =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max} > v_L),
\end{align}

\begin{align}
    OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i),
\end{align}
%\xc{Modified OSR $OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$. 
%where $Threshold_i>1$ (e.g.,  Levl 1:$Threshold_1=1.1$, Level2:$Threshold_2=1.2$ ... ) indicates the different level of over-speeding }
where $Threshold_i$ is used to capture different levels of over-speeding.
Here, $v_L$ is the speed limit, and $I(x>y)$ is the indicator function with $I(x>y)=1$ for $x>y$ and $I(x>y)=0$ otherwise.  
Speed limits are typically set based on a standardized set of guidelines and national manuals, taking into account road geometry features such as the radii of curves, sight distance, and weather conditions. A high OSR, when associated with a high crash rate, may indicate the need for taking more warning and prevention measures to avoid over-speeding, noting that over-speeding can be an important contributor to crashes. On the other hand, high OSR, when it does not correlate with a high accident rate, can indicate the need for revising the set speed limits without compromising traffic safety. 

The aforementioned traffic metrics can be characterized by processing the roadside cameras or by crowd-sourcing and accumulating information provided by vehicles' dash cameras.

\textbf{Traffic Composition Indicator (TCI)} is defined to gauge the diversity of vehicle types in specific road sections.  
For instance, it is known that a higher density of trucks on roads can correlate with the frequency and severity of road accidents; hence trucks are prohibited in some road sections in highly-populated areas \cite{meyers1981comparison}. This can be due to trucks' larger deceleration inertia, more frequent break failures, and lower maneuverability levels. In general, if vehicles classified into classes $c=1,2,3,\dots,C$, then the traffic composition can be defined as
\begin{align}
    TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2},\\
\end{align}
where $N_c$ is the number of vehicles in class $c$, and the metric is defined similarly to the Jain fairness index. This metric ranges from $1/C$ for the most unbalanced composition to $1$ for an equal number of vehicles from each type. If one is interested in evaluating the rate of a specific class like trucks to all vehicles, the following metric can be used:
\begin{align}
     f_c = \frac{N_c}{\sum_{i=1}^C N_i}.
\end{align}

When classifying cars into two classes $c=1$ for trucks and $c=2$ for non-trucks, these two metrics are related as 
\begin{align}
     TCI = \frac{1}{2(1-2 f_1 f_2)}.
\end{align}

Lower $TCI$ values mean that most cars are of the same type with lower risks. This metric can be estimated by processing roadside videos but requires high-complexity learning methods for vehicle detection and classification. 
 
\textbf{Normalized Traffic Density (NTC)} is defined as the density of vehicles on road sections as 
%  \begin{align}
%      NTC = \frac{N_v}{N_l*L},
%  \end{align}
 
  \begin{align}
     NTC = \frac{\sum \exp{l_i/\bar{l}}}{N_l*L},
 \end{align}
%\xc{$NTC = \frac{\sum l_i/\bar{l}}{N_l*L},
where  $l_i$ is the length of a vehicle, $\bar{l}$ is the average of all vehicles' length. We normalize the vehicle by its length to capture the effect of vehicle's size. %later we cn check, I am not sure it is necessary to make it this complex?

Here, 
%$N_v$ is the number of vehicles, 
$N_l$ is the number of lanes, and $L$ is the length of the road section. This parameter can be easily captured by video processing and vehicle recognition. Higher NTC values are expected to be associated with higher crash rates, and may raise the request for traffic load balance strategies.  
 
\textbf{Traffic Recovery Time (TRT)} is defined as the time required for traffic flow recovery after accidents. 
The system of vehicular flow can be considered as a non-equilibrium system of interacting particles \cite{sugiyama2008traffic}, and the instability of a flow-free state is induced by the collective effects of the increase of fluctuations. 
It is known that any traffic event can suddenly lead to a jamming state, and TRT reflects the time span from an event epoch to the status change to free flow. This time is expected to be much shorter than the interval between the consecutive events for flow stability. TRT can be defined as:
\begin{align}
    TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|,
\end{align}
where $N_e$ is the number of events in the monitoring interval, and $t_b(i)$ and $t_r(i)$, respectively, denote the event start epoch, and the flow recovery epoch for event $i$. These parameters can be easily captured by roadside videos or fusing information obtained from dash cameras. 
%\arr{update the table accordingly}

The summary of the proposed network-level safety metrics is presented in Table \ref{tab:newmetric}. We believe that this list is not comprehensive by any means and can initiate efforts to develop a more comprehensive list of network-level safety metrics. 




\begin{comment}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htbp]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Metric &
  Defination &
  Features \\ \hline
IVVR &
  $IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects the instability of traffic flow by car speed variations and crash rate;\\ Can partially offer network re-design suggestions;\end{tabular} \\ \hline
OVVR &
  $OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}}$ &
  \begin{tabular}[c]{@{}l@{}}Overall speed variation of vehicles; \\Defined similar to IVVR for overall traffic speed variation;\\ Not easily affected by outliers; \end{tabular}\\ \hline
OSR &
  $OSR =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max} > v_L)$ &
  \begin{tabular}[c]{@{}l@{}}Indication of speed limit violations; Can offer suggestions for network design;\end{tabular} \\ \hline
TCI &
  \begin{tabular}[c]{@{}l@{}}$TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2}$\\ $f_c = \frac{N_c}{\sum_{c=1}^C N_c}$\\ $TCI = \frac{1}{2(1-2 f_1 f_2)}$, two classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Flow composition indicator;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
NTC &
  $NTC = \frac{\sum l_i/\bar{l}}{N_l*L}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects traffic density;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
TRT &
  $TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|$ &
  \begin{tabular}[c]{@{}l@{}}
  A simple and reasonable way to evaluate severity of the accidents;\\
  Can also take traffic stability into consideration\end{tabular}\\ \hline
\end{tabular}%
}
\caption{A set of proposed network-level safety metrics. }
\label{tab:newmetric}
\end{table}

\end{comment}


\begin{table*}[htbp]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric} &
  \textbf{Definition} &
  \textbf{Features} \\ \hline
IVVR &
  $IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects the instability of traffic flow by car speed variations and crash rate;\\ Can partially offer network re-design suggestions\end{tabular} \\ \hline
OVVR &
  $OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}}$ &
  \begin{tabular}[c]{@{}l@{}}Overall speed variation of vehicles; \\Defined similar to IVVR for overall traffic speed variation;\\ Not easily affected by outliers \end{tabular}\\ \hline
OSR &
  $ OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$ &
  \begin{tabular}[c]{@{}l@{}}Indication of speed limit violations; Can offer suggestions for network design\end{tabular} \\ \hline
TCI &
  \begin{tabular}[c]{@{}l@{}}$TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2}$\\ $f_c = \frac{N_c}{\sum_{c=1}^C N_c}$\\ $TCI = \frac{1}{2(1-2 f_1 f_2)}$, two classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Flow composition indicator;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
NTC &
  $NTC = \frac{\sum \exp{l_i}/\bar{l}}{N_l*L}$ &
  \begin{tabular}[c]{@{}l@{}}Consider vehicle shape;\\ Reflects traffic density;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
TRT &
  $TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|$ &
  \begin{tabular}[c]{@{}l@{}}
  A simple and reasonable way to evaluate severity of the accidents;\\
  Can also take traffic stability into consideration\end{tabular}\\ \hline
\end{tabular}%
}
\caption{A set of proposed network-level safety metrics.} %\xc{modified}}
\label{tab:newmetric}
\end{table*}
%TRT:\ar{of what? potential accidents.} \arr{Is not it more related to the overall stability of traffic in case of crashes? because it does not say what is the risk, rather it says how long it takes to recover and be back to normal conditions after an accident.}
%\xc{TRT: What I think is TRT is more related to the effect brought by crashes, which can be explained by both severity and traffic stability}





==> sensors.tex <==
\section{Data Acquisition}   \label{sec:hardware}

In this section, we investigate the role of data acquisition in developing safety-related algorithms. First, we review data modalities and hardware used for information acquisition. Next, we list the most commonly used datasets for testing the developed algorithms. 


\subsection{Sensor and Data Acquisition Equipment}

Most traffic analysis platforms rely on data collected by different types of sensors, including cameras, Global Positioning Systems (GPS), Radio Detection And Ranging (Radar), and Light Detection and Ranging (LiDAR). These sensors (except GPS) can be used in vehicles or on external observer systems such as roadside infrastructures, drone-based aerial platforms, etc. 
The following is a short description of sensors followed by a summary provided in Table \ref{tab:sensors}.


\textbf{Video Cameras} are the most widely used means of information collection. Modern cars are heavily equipped with cameras in various parts to capture imagery for processing. Using thermographic cameras for night vision has become more common than ever. 
Camera feeds can be used by the driver (e.g., backup camera) to minimize safety risks, or by the control computer in an AV for automated driving. The imagery can also be used by more advanced AI platforms for driver's cognition assessment in real-time mode (e.g., driver drowsiness assessment \cite{affectiva}, and distraction awareness \cite{mejia_2020}). Volume collections of imagery can be stored for further analysis for transportation infrastructure revisions.

\textbf{GPS} systems provide an accurate position of the vehicle by communicating to GPS satellites. 
The accuracy of GPS depends on different factors, including satellite geometry, signal blockage, atmospheric conditions, and receiver design features/quality. The global average User Range Error (URE) of GPS can be as low as 2.3 ft\cite{gpsIMAGE}. With recent advances in 5G wireless networking, even preciser positioning is available for vehicles. For instance, Verizon launched its Hyper Precise Location using Real-Time Kinematics (RTK), with an unprecedented accuracy of 1-2 centimeters\cite{radio_resource_2028}.
% \arr{add REF: like below.}\xc{done} %https://www.rrmediagroup.com/News/NewsDetails/NewsID/19972#:~:text=By%20creating%20a%20vehicle%2Dto,and%20warn%20vehicles%20of%20impending
%\arr{add REF like GPS.gov, etc.}


\textbf{Radar} operates based on Doppler frequency shift in the reflected wave \cite{munoz2008traffic}. Radar units are often installed on modern cars, roadside poles, police vehicles, and portable speedometer guns to measure the absolute or the relative speed of other vehicles. Radars are low-cost and relatively robust devices appropriate for different weather conditions and illumination intensities. Some radar units may have a narrow Field of View (FoV) but are capable of long-range detection \cite{shirazi2016looking}. A traditional radar is a single source-detector, which does not have the spatial resolution required for precise scene/environment description; however, in recent years, imaging radars have been developed by adopting multiple-input, multiple-output (MIMO), and radar-on-chip technologies. Although such advanced technology is still expensive, attempts are made to reduce the cost of broader adoption\cite{bilik2019rise}.

\textbf{LiDAR} uses laser beam reflection to enable accurate positioning down to centimeter's scale \cite{tan2016weakly}. The 3D scanning of multiple laser beams provides a 3D point cloud image (3D map) of the surrounding obstacles with accuracy much higher than regular radars \cite{ma2018mobile}. LiDARs send out a near-infrared laser beam and detect reflections from the object; thus, it can still operate in dark conditions, in contrast to visual sensors. Its use is less common than radars for a few reasons, including its higher cost, relatively sparse spatial resolution, especially for a limited number of scanning laser beams, extremely narrow FoV, and computational complexity of $360^\circ$ scanning, noting that low-complexity point cloud methods are still under development. Solid-state LiDARs have been developed to reduce the cost, while enhancing the spatial resolution\cite{erichsen2020semantic}.


\textbf{Drones} are commonly used nowadays to implement aerial monitoring systems. Most external observer systems utilize sensors in roadside infrastructures. However, the use of drones, also known as Unmanned Aerial Vehicles (UAVs), is gaining more attention in different applications to enable fast, low-cost, and on-demand monitoring \cite{khan2017uav}, and traffic analysis is not an exception. Particularly, drones can provide top-view and clearer occlusion-free images of the traffic flow when needed \cite{ke2018real}. A network of cooperative drones can collectively cover relatively large areas \cite{barmpounakis2020new}. Modern drones may be equipped with advanced sensing platforms, high-resolution cameras, and more importantly advanced features such as learning-based image processing, AI-based autonomous control, collision avoidance and auto lading, auto-calibration, real-time transmission, object tracking, and image restoration. The key challenges of drones are their limited payload, flight time, and communication range under study by several research teams. Aerial images pose new challenges to the research community, such as tackling image stabilization, small object recognition, and developing lightweight ML algorithms customized for top-view images. 

\textbf{Other Sensors:} 
In addition to the aforementioned broadly-used sensors, there exist some custom-built advanced sensors that can be used for traffic monitoring and driving safety analysis. Passive Infrared sensors\cite{ahmed1994active}, Inductive Loops\cite{mimbela2007summary}, and Piezoelectric sensors\cite{zhang2015new} can enable measuring basic flow parameters such as vehicle count, speed, and flow volume, noting that Piezoelectric sensors are still used for weigh-in-motion measurement. Environmental Sensor Stations (ESS)\cite{ESS} on the roadway can collect atmospheric data, including air temperature and humidity, visibility distance, wind speed, wind direction, etc., as side parameters to be used for traffic analysis. 


